Deep Learning based Vulnerability Detection: Are We There Yet?

Automated detection of software vulnerabilities is a fundamental problem in software security. Existing program analysis techniques either suffer from high false positives or false negatives. Recent progress in Deep Learning (DL) has resulted in a surge of interest in applying DL for automated vulnerability detection. Several recent studies have demonstrated promising results achieving an accuracy of up to 95% at detecting vulnerabilities. In this paper, we ask, "how well do the state-of-the-art DL-based techniques perform in a real-world vulnerability prediction scenario?". To our surprise, we find that their performance drops by more than 50%. A systematic investigation of what causes such precipitous performance drop reveals that existing DL-based vulnerability prediction approaches suffer from challenges with the training data (e.g., data duplication, unrealistic distribution of vulnerable classes, etc.) and with the model choices (e.g., simple token-based models). As a result, these approaches often do not learn features related to the actual cause of the vulnerabilities. Instead, they learn unrelated artifacts from the dataset (e.g., specific variable/function names, etc.). Leveraging these empirical findings, we demonstrate how a more principled approach to data collection and model design, based on realistic settings of vulnerability prediction, can lead to better solutions. The resulting tools perform significantly better than the studied baseline: up to 33.57% boost in precision and 128.38% boost in recall compared to the best performing model in the literature. Overall, this paper elucidates existing DL-based vulnerability prediction systems' potential issues and draws a roadmap for future DL-based vulnerability prediction research. In that spirit, we make available all the artifacts supporting our results: https://git.io/Jf6IA.

==> README <==
This package provides a class for typesetting publications of 
Association for Computing Machinery.

Your TeX distribution probably includes the latest released version of
this package.  If you decide to install it yourself, please see
Installation section of the User's Guide.

Changes

version 1.08    SIGPLAN reformatting (Matthew Fluet); bug fixes

version 1.09    SIGPLAN: revert caption rules (Matthew Fluet)

version 1.10    Bug fixes

version 1.11    Customization of ACM theorem styles and proof
                environment (Matthew Fluet).

version 1.12    Bug fixes and documentation updates.  
		Footnotes rearranged.
                Option natbib is now mostly superfluous: the class 
		makes a guess based on the format chosen.

version 1.13    Formatting changes: headers, folios etc.
		Bibliography changes.

version 1.14    Warn about undefined citation styles; move definitions
                of acmauthoryear and acmnumeric citation styles before
                use.

version 1.15    New structured affiliation command.
                New commands for acknowledgements.

version 1.16    Formatting changes for headers and footers.

version 1.17    Formatting changes for margins and lists.  Bug fixes.

version 1.18    Natbib is now the default for all versions.  A unified bib
		file is used for all styles.  Better treatment
		of multiple affiliations.

version 1.19    Include 'Abstract', 'Acknowledgements', and 'References'
                in PDF bookmarks.

version 1.20    Bug fixes, documentation updates

version 1.21    Bibliography changes: added arXiv, some cleanup

version 1.22    Bibliography changes for Aptara backend;  should be 
		invisible for the users.

version 1.23    Added PACM PL journal option.

version 1.24    Added IMWUT journal option.

version 1.25    Updated PACMPL journal option.

version 1.26    Bug fixes

version 1.27    Bug fixes

version 1.28    Bug fixes: natbib=false now behaves correctly.

version 1.29	Documentation changes.  Head height increased from 12pt to 13pt.
		Removed spurious indent at start of abstract.
		Improved kerning in CCS description list.

version 1.30    Bibtex style now recognizes https:// in doi.
	        Added \frenchspacing.
		\department now has an optional hierarchy level.
		Switched to T1 encoding
		Updated IMWUT and PACMPL

version 1.31    Changed default year and month to the current ones
		(thanks to Matteo Riondato)
		Table of contents now works
		Marginalia now work in all formats
		New command \additionalaffiliation
		Documentation changes

version 1.32    New DOI formatting.
		Format siggraph is now obsolete, and sigconf
		is used instead.
		New proceedings title: POMACS.

version 1.33    New option `timestamp' (Michael D. Adams)
		New option `authordraft'
                Documentation updates
		Bug fixes
		We now use Type 1 versions of Libertine fonts even with XeTeX.
		New hook acmart-preload-hook.tex (wizards only!)
		Added new options `obeypunctuation' for \affiliation command
		Added SubmissionID
		Added right line count ruler for two-column formats
		Added workaround for Adobe Acrobat bugs in selection
		Added eid field to the bibliography
		
version 1.34    Deleted DOI from doi numbers
		Changed bibstrip formatting
		The command \terms is now obsolete
		The rulers in review mode now have continuous numbering

version 1.35    Author-year bib style now uses square brackets.
		Changed defaults for TOG sample
		Price is suppressed for usgov and rightsretained modes.
		Bugs fixed

==> RQ_answers/Tables/RQ3_ablation.tex <==
\begin{figure*}[!htb]
    \centering
        \begin{subfigure}{0.30\linewidth}
        \includegraphics[width=\linewidth]{RQ_answers/Box_plots/verum-precision.pdf}
        \caption{\small Contribution of GGNN}
        \label{fig:ggnn_abl}
        \end{subfigure}
        \begin{subfigure}{0.30\linewidth}
        \includegraphics[width=\linewidth]{RQ_answers/Box_plots/verum-recall.pdf}
        \caption{\small Recall}
        \label{fig:verun_rc_bp}
        \end{subfigure}
        \begin{subfigure}{0.30\linewidth}
        \includegraphics[width=\linewidth]{RQ_answers/Box_plots/verum-f1.pdf}
        \caption{\small F1-score}
        \label{fig:verun_f1_bp}
        \end{subfigure}
        \caption{\small {Performance spectrum of \realdata.}}
        \label{fig:verun_bp}
\end{figure*}


==> RQ_answers/Tables/code_heatmaps.tex <==
\begin{figure}
\centering
\begin{subfigure}{0.95\linewidth}
\scriptsize
\tt
\begin{tabular}{|r p{0.89\linewidth}|}
\hline
1  & \ltwo{link\_layer\_show(\textbf{struct} ib\_port {*}p, } \\
2  & ~~~~~~~\lone{\textbf{struct} port\_attribute {*}unused, \textbf{char} * buf)\{}\\
3  & ~~~\lone{\textbf{switch} }\lthree{(rdma\_port\_get\_link\_layer(}\\
4  & ~~~~~~~~~~~~~~~\lthree{p->ibdev, p->port\_num))}\lfive{ \{}\\
5  & ~~~~~~\lfive{\textbf{case} }\lfour{IB\_LINK\_LAYER\_INFINIBAND:}\\
6  & ~~~~~~~~~\lfour{\textbf{return} \blue{sprintf(buf, "\%s$\backslash$n", "InfiniBand")};}\\
7  & ~~~~~~\lfive{\textbf{case} IB\_LINK\_LAYER\_ETHERNET:}\\
8  & ~~~~~~~~~\lfive{\textbf{return} \blue{sprintf(buf, "\%s$\backslash$n", "Ethernet")};}\\
9  & ~~~~~~\lfive{\textbf{default}:}\\
10 & ~~~~~~~~~\lfive{\textbf{return} \blue{sprintf(buf, "\%s$\backslash$n", "Unknown")};}\\
11 & ~~~\lfive{\}}\\
12 & \lfive{\}}\\
\hline
\end{tabular}
\caption{{\small Vulnerable code example in \draper \cite{russell2018automated} dataset correctly predicted by a token-based Russel~\etal's method.}}
\label{fig:lemna_draper}
\end{subfigure}
\vspace{5mm}
    
\begin{subfigure}{0.95\linewidth}
\scriptsize
\tt
\begin{tabular}{|r p{0.89\linewidth}|}
\hline
1 & \textbf{static int} mov\_read\_dvc1(\lfour{MOVContext *c},  \\
2 & ~~~~~~~~\lfour{AVIOContext *pb}, \lthree{MOVAtom atom}) \{ \\
3 & ~~~~\lone{AVStream *st};  \\
4 & ~~~~\lfour{\textbf{uint8\_t} profile\_level}; \\
5 & ~~~~\textbf{if} (\lthree{c->fc->nb\_streams < 1}) \\ 
6 & ~~~~~~~~\lfour{\textbf{return} 0}; \\
7 & ~~~~\ltwo{st = c->fc->streams[c->fc->nb\_streams-1]}; \\
8 & ~~~~\textbf{if} (\lfour{atom.size $>=$ (1$<<$28) || atom.size $<$ 7}) \\
9 & ~~~~~~~~\lfour{\textbf{return} AVERROR\_INVALIDDATA}; \\
10 & ~~~~\lfour{profile\_level = avio\_r8(pb)}; \\
11 & ~~~~\textbf{if} (\lfour{(profile\_level \& 0xf0) $!=$ 0xc0}) \\
12 & ~~~~~~~~\lthree{\textbf{return} 0}; \\
...   & ~~~~...\\
% 13 & ~~~~\lfour{av\_free(st->codec->extradata)}; \\
% 14 & ~~~~\lfour{st->codec->extradata = av\_mallocz(}\\
% 15 & ~~~~\lfour{atom.size - 7 + FF\_INPUT\_BUFFER\_PADDING\_SIZE)}; \\
% 16 & ~~~~\textbf{if} (\lfive{$!$st->codec->extradata}) \\
% 17 & ~~~~~~~~\lfive{\textbf{return} AVERROR(ENOMEM)}; \\
18 & ~~~~\lfour{st->codec->extradata\_size = atom.size - 7}; \\
19 & ~~~~\ltwo{avio\_seek(pb, 6, SEEK\_CUR)}; \\
20 & ~~~~\lfour{\blue{{avio\_read(}}}\\
21 & ~~~~~~~~\lfour{\blue{{pb, st->codec->extradata,}}}\\
22 & ~~~~~~~~~~~~\lfour{\blue{{st->codec->extradata\_size)}}};\\ 
23 & ~~~~\lfour{\textbf{return} 0}; \\
24 & \}\\ 
\hline
\end{tabular}
\caption{{\small Vulnerable example from \devigndata~\cite{zhou2019devign} dataset correctly predicted by graph-based \tool model. Other methods could not predict the vulnerability in this example.}}
\label{fig:lemna_ggnn}
\end{subfigure}
\vspace{5mm}

\caption{Contribution of different code component in correctly  classifying the corresponding method as vulnerable by different models. \lone{Red-shaded} code elements have highest contribution, while  \lfive{Green-shaded} elements have the least. 
\blue{Blue} colored code are the source of vulnerabilities.}
\label{fig:code_heatmap}
\end{figure}

==> RQ_answers/Tables/rq1_range_plots.tex <==
\begin{table}[!htb]
    \centering
    \footnotesize
    \caption{\small \textbf{Comparisons of all available baselines in \realdata.}}
    \begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
        \hlineB{2}
        \textbf{Rank} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \bigstrut\\
        \hlineB{2}
          \hline
          1 &    \tool &    41.25  &  2.28 & \quart{73}{6}{77}{233} \bigstrut\\
          \hline
          2 &       SySeVR &    30.25  &  2.35 & \quart{45}{7}{47}{233} \bigstrut\\
          2 &     GGNN &    29.87  &  4.34 & \quart{42}{11}{46}{233} \bigstrut\\
          \hline
          3 &        VulDeePecker &    15.70  &  6.41 & \quart{0}{17}{8}{233} \bigstrut\\
          3 & Russel et. al. &    15.24  &  2.74 & \quart{2}{7}{7}{233} \bigstrut\\
        \hline
        \hlineB{2}
    \end{tabular}
   
    \label{tab:full_comparison_verum}
\end{table}


\begin{table}[!htb]
    \centering
    \footnotesize
    \caption{\small \textbf{Comparisons of all available baselines in \devigndata (F-1 score).}}
    \begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
        \hlineB{2}
        \textbf{Rank} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \bigstrut\\
        \hlineB{2}
          1 &   \tool &    64.42  &  1.33 & \quart{76}{3}{78}{161} \bigstrut\\
        \hline
          2 &         GGNN &    57.18  &  2.58 & \quart{58}{6}{61}{161} \bigstrut\\
        \hline
          3 &     SySeVR &    56.03  &  3.20 & \quart{53}{7}{58}{161} \bigstrut\\
        \hline
          4 & Russel et. al. &    45.62  &  1.33 & \quart{32}{4}{34}{161} \bigstrut\\
        \hline
          5 &      VulDeePecker &    35.20  &  8.82 & \quart{0}{20}{9}{161} \bigstrut\\
        \hline
        \hlineB{2}
    \end{tabular}
    \label{tab:full_comparison_devign}
\end{table}


==> RQ_answers/rq1.tex <==
% \subsection{Limitations of existing datasets (RQ1)}
% \label{sect:rq1}

% % \noindent{\textbf{RQ1: \textit{What are the limitations of existing datasets?}}}

% \begin{figure}[!tpb]
%     \input{Tables/lemna_example_1_integer_overflow}
%     \vspace{5mm}
%     \input{Tables/lemna_example_2_memory_overflow}
%     \vspace{5mm}
%     \input{Tables/lemna_example_3_draper_G_D}
%     % \vspace{5mm}
%     \caption{\small \textbf{Code examples visualization with Lemna~\cite{guo2018lemna}. All of these code examples are predicted as vulnerable by respective models. \cref{fig:lemna_int_overflow} and \cref{fig:lemna_memory_overflow} are code slices from NVD+SARD dataset and SySeVR predicted those as vulnerable. \cref{fig:lemna_draper} is also predicted as vulnerable by Russel~\etal's CNN+RF~\cite{russell2018automated} model. \lone{Red} colored tokens contributed the most in respective predictions. \lfive{Green} colored tokens contributed the least.}}
%     \label{fig:lemna_examples}
% \end{figure}

% % \noindent\textbf{}


% \motivation We begin with a close inspection of the widely used \vp datasets. Specifically, we investigate the properties of those datasets and the features that are learned by existing DL models trained on those datasets. VulDeePecker~\cite{li2016vulpecker} and SySeVR~\cite{li2018sysevr} offer vulnerability prediction models trained on a mixture of vulnerable examples from NVD~\cite{booth2013national} and SARD~\cite{SARD} datasets; Russell~\etal~\cite{russell2018automated} offers a vulnerability prediction model trained on \draper data which are annotated with a static-analysis tool (see~\tab{existing_approach_design_choices}). 

% % We first intend to understand what features do different models learn when trained on these datasets. Although 
% \approach It is difficult, if not impossible, to fully explain what DL models learn~\cite{frosst2017distilling}. However, recent techniques such as Lemna~\cite{guo2018lemna} have shown much success in providing useful explanations. Lemna estimates the local decision boundary around a data point using an auxiliary explainable linear model. Given a sequence of tokens as input, Lemna generates a weight corresponding to the contribution of every token in the models' prediction.

% Specifically, given an example data point $(x_i,\;y_i),\;i\in \{1,\ldots,N\}$ where $x_i$ is the input and $y_i$ is the predicted label by \vp model, Lemna draws samples around $x_i$ to obtain $L$ synthetic input sequences $z_{i,j},\;j\in \{1,\ldots,L\}$ and its prediction labels $w_{i,j},\;j\in \{1,\ldots,L\}$. Lemna then learns a linear regression model from the original data point along with the sampled data points. Each of the token $x_i^t$ is assigned a value $\omega_i^t$ representing the contribution of that token for prediction. Higher value of $\omega_i^t$ would indicate larger contribution of token $x_i^t$ in predicting for $y_i$. For a detailed discussion, see~\cite{guo2018lemna}. We use the heatmap generated by Lemna to visualize the contribution of different tokens in an input code snippet for predicting the existence of vulnerability. 

% To further analyze the characteristics of existing datasets, we investigate amount of duplication in the datasets. There are several ways duplication can be introduced by the preprocessing techniques used by the DLVP method -- \eg. same slice can be extracted from different entry points, different code can have same token sequence due to the abstract tokenization adopted by the approaches\footnote{For details about the slicing and tokenization, we refer to \Cref{subsec:background_overview} and respective papers~\cite{ li2018sysevr, russell2018automated, li2016vulpecker}}. 

% \observations \Cref{fig:lemna_examples} shows three examples of vulnerable code snippets.~\Cref{fig:lemna_int_overflow}, and~\Cref{fig:lemna_memory_overflow} are from NVD and SARD datasets and used by VulDeePecker~\cite{li2018vuldeepecker}, and SySeVR~\cite{li2018sysevr} to train their models respectively. Both of those code snippets show code slices extracted from the program, since both VulDeePecker and SySeVR are trained on slices. ~\Cref{fig:lemna_draper} shows a function from \draper~\cite{russell2018automated}, which Russel~\etal~\cite{russell2018automated} used to train their model. Note that, while we show the actual code tokens for analysis purpose, for training we used approach specific tokenization.

% Each token in~\fig{lemna_examples} is highlighted with a color corresponding to the token's contribution to the prediction. Most important tokens are highlighted in \lone{red} and the least important tokens are colored \lfive{green}. We make the following observations:

% \smallskip
% \noindent\textit{NVD + SARD dataset.}~Examples shown in \Cref{fig:lemna_int_overflow} and \Cref{fig:lemna_memory_overflow} are predicted correctly by SySeVR. But from the heatmap, the most important token sequences used for the prediction are not related to the tokens pertaining to the actual vulnerability. 


% ~\Cref{fig:lemna_int_overflow} demonstrates an integer overflow vulnerability (CWE-190) where multiplying two integers (or a floating point variable) might result in an overflow. The actual vulnerability in this case lies in line 7, however \lone{\tt \textbf{void}} \lone{\tt CWE190\_Integer\_Overflow\_Unsigned\_int...()} contributes the most to SySeVR's Deep Learning model followed by \ltwo{\tt \textbf{unsigned int} data} and \ltwo{data = 0;}. 


% \Cref{fig:lemna_memory_overflow} shows a similar example for Uncontrolled Memory Vulnerability (CWE-789), where size of the memory allocated comes from a user input or the output of an API call. Without explicit sanitization, it can cause an uncontrolled memory allocation leading to a crash. Even though the main reason for the vulnerability in this example lies in lines 5, 9, and 10, however \lone{\tt \textbf{void} CWE789\_Uncontrolled\_Mem\_Alloc... ()} contributes the most in SySeVR's Prediction, followed by \ltwo{\tt \textbf{size\_t} data ;} and \ltwo{\tt data = 0;}.

% \smallskip
% \noindent\textit{\draper dataset.}~The example shown in \Cref{fig:lemna_draper} is predicted correctly as vulnerable by Russel~\etal's method. The plausible reason for this code to be vulnerable is the use of {\tt sprintf} function in line 6, 8, and 10. The length of {\tt buf} is not checked before writing to it through the {\tt sprintf} function. The CNN+RF model proposed by Russel~\etal~\cite{russell2018automated} picked up \lone{\tt \textbf{struct} port\_attribute} \lone{\tt *unused, \textbf{char} * buf)\{ \textbf{switch}} as the highest contributing token sequence. Similar to previous two examples, neither highest, nor the second highest contributing token sequences are related to the vulnerability.

% \input{RQ_answers/Tables/rq1_duplicate_results}


% Table~\ref{tab:duplicate} shows the percentage of duplicate samples generated by different DLVP methods. For NVD and SARD datasets, the preprocessing technique from VulDeePecker results in $\mathbf{\sim75\%}$ duplicate examples (leaving only $\sim$25\% unique examples). $\mathbf{\sim50\%}$ of the examples are duplicated for NVD and SARD datasets when preprocessing technique from SySeVR is used. In Juliet and \draper datasets, Russell~\etal.'s method produces $57\%$ and $2.98\%$ duplicate examples, respectively. Ideally, a DL based model should be trained and tested on a dataset where 100\% of the examples are unique.  Duplication tends to artificially inflate the overall performance of the method~\cite{allamanis2019adverse}. 

% We note that dataset used to train VulDeePecker and SySeVR\footnote{NVD + SARD dataset, mostly examples from SARD} were not originally intended to be used for vulnerability prediction task. These datasets were designed to elicit false negatives/false positives in static analyzers and also for human reference (in the form of CWEs). Therefore, they offer a simplified representation of the real vulnerability. Unlike these datasets, the \draper dataset was collected by Russell~\etal~\cite{russell2018automated} from the real world projects on GitHub and some examples from the Debian distribution. However, the annotations for \draper were made using a collection of static analyzers, therefore, it is difficult to know how noisy the dataset is \ie how many of these annotated vulnerabilities are False Positives. We conjecture that, the simplicity and the noise in the datasets are forcing models to learn irrelevant features from the datasets. 


% % \noindent\textbf{Approach.}~

% % this informs us of how much of the training and testing samples are exactly the same after the code has been preprocessed. 





% \begin{result}
% Existing (semi-)synthetic datasets are too simple~\bray{I don't think we demostrate simplicity} and homogeneous to be representative of the intricacies of real-world vulnerabilities. Essentially, the existing models trained on the synthetic datasets are learning trivial and shallow features that are not related to the core logic of the vulnerabilities.
% \end{result}

% As outlined in~\Cref{tab:existing_approach_design_choices}, existing approaches applied their model in finding vulnerabilities in real world projects and reported some success. Similar to that experimental settings, we also tested those method trained on those datasets for finding vulnerabilities in \realdata and \devigndata. Without much of a surprise, we found that they perform poorly. Full results of this experiment are described in \Cref{appnd:pretrain_results} for interested readers. 
% \bray{summarize the results in one line}

% Since (semi-)synthetic datasets do not fully represent real world vulnerabilities, for the rest of this paper focus on using real world data. We investigate how existing techniques perform while learning from real world data, what the limitation of existing techniques are when they learn from real world data, and how \tool overcome those limitations. 
% % Now we move onto investigating 
% % Now that we discovered some interesting properties of existing (semi-)synthetic datasets, we also tested respective models trained on those dataset 

% % \input{RQ_answers/Tables/rq2_result}


==> RQ_answers/rq1_new.tex <==
\subsection{Effectiveness of existing \vp approaches (RQ1)}
\label{sect:rq1}
\motivation The goal of any \dlvp approaches is to be able to predict vulnerabilities in the real-world. The datasets that the existing models are trained on contain synthetic examples that are representative of real-world vulnerabilities. Therefore, we ought to, in theory, be able to use these models to detect vulnerabilities in the real-world. There are two possible scenarios under which these models may be used: 

\noindent$\circ$~ \textit{Scenario-A~(pre-trained models)}:~We may reuse the existing pre-trained models to predict for vulnerabilities that appear in the real-world datasets, or 

\noindent$\circ$~ \textit{Scenario-B~(re-trained models)}:~We may rebuild the existing models first by training them on the real-world datasets and then we may use those models to detect the vulnerabilities. In this research question, we investigate the effectiveness of each of these strategies. 

\approach To answer this research question, we study the approaches listed in~\tab{existing_approach_design_choices}. Specifically, we undertake the following steps:
\bi
\item For \textit{Scenario-A}, in order to determine if existing pre-trained models can be used to detect real-world vulnerabilities, we first train VulDeePecker~\cite{li2016vulpecker} and SySeVR~\cite{li2018sysevr} on datasets used in their corresponding approaches, \ie, examples from NVD~\cite{booth2013national} and SARD~\cite{SARD} datasets. Likewise, for Russell~\etal~\cite{russell2018automated} train their model on the \draper dataset. Next, we use those pre-trained models to detect vulnerabilities in real-world datasets (\ie, on \devigndata and \tool dataset).
\item For \textit{Scenario-B}, in order to assess the performance of existing approaches when they are re-trained afresh on real-world datasets, we use one portion of the \devigndata and \tool dataset to first train VulDeePecker, SySeVR, and Russell~\etal's models. Then, we use those models to predict for vulnerabilities in the remainder of the \devigndata and \tool. We repeat the process 30 times, each time we training and test portions of the dataset are different.
\ei

\observations~\tab{pretrained} tabulates the performance of existing pre-trained models on predicting vulnerabilities in real-world data from \devigndata and \tool dataset. We observe a precipitous drop in performance when pre-trained models are used for real-world vulnerability prediction. 

In \realdata, VulDeePecker achieves an F1-score of \textit{only} $\mathit{12.08}\%$ and in \devigndata VulDeePecker achieves an F1-score of $\mathit{14.33}\%$, while in the baseline case (\ie, rows labeled `Baseline') which used semi-synthetic data (NVD/SARD) for testing, the F1-score of VulDeePecker was as high as $\mathit{85.4\%}$. 

Using pre-trained SySeVR models exhibit a similar trend as that of VulDeePecker. In \realdata, SySeVR achieved an F1-score of \textit{only} $\mathit{10.27}\%$ and in \devigndata SySeVR achieved an F1-score $\mathit{16.85}\%$, this was significantly lower than the F1-score of $\mathit{85.2\%}$ that was reported on baseline case which used semi-synthetic data for testing.

As with the previous two models, we observe a notable reduction in predictive performance of Russell~\etal's model when applied to real-world datasets. In the case of \devigndata, DL model from Russell~\etal's method produced an F1-score of $\mathit{46.77\%}$ on \devigndata compared to the baseline of $\mathit{56.6\%}$. In \realdata, the F1-score was only $\mathit{23.67\%}$.

Since the pre-trained models from any of the existing approaches failed to convincingly predict vulnerabilities in the real-world, we rebuild the existing models afresh by training on real-world data from \devigndata and \tool data. \tab{retrained} tabulates our findings for re-trained models. 

We observe limited performance improvements. In \tool dataset, both Russell~\etal and VulDeePecker achieve an F1-score of roughly $\mathit{15\%}$ (in contrast to their baseline performances of $\mathit{85\%}$ of their respective datasets). SySeVR achieved an F1-score of $\mathit{30\%}$ on \tool dataset. This was still considerably lower than the baseline F1-score of $\mathit{85\%}$. We observed similar trends in \devigndata. 



\begin{result}
Existing approaches fail to generalize to real-world vulnerability prediction. When existing pretrained \vp models are used for real-world vulnerability prediction, we observe F1-scores \textit{as low as} $10\%$ (almost $70\%$ less than the corresponding baseline). When existing models are build afresh by training on real-world data, we obtain slightly better performance of \textit{at most} $\mathit{56\%}$ which is still almost $\mathit{30\%}$ less than the baseline.
\end{result}

% As outlined in~\Cref{tab:existing_approach_design_choices}, existing approaches applied their model in finding vulnerabilities in real world projects and reported some success. Similar to that experimental settings, we also tested those method trained on those datasets for finding vulnerabilities in \realdata and \devigndata. Without much of a surprise, we found that they perform poorly. Full results of this experiment are described in \Cref{appnd:pretrain_results} for interested readers. 
% \bray{summarize the results in one line}

% Since (semi-)synthetic datasets do not fully represent real world vulnerabilities, for the rest of this paper focus on using real world data. We investigate how existing techniques perform while learning from real world data, what the limitation of existing techniques are when they learn from real world data, and how \tool overcome those limitations. 
% Now we move onto investigating 
% Now that we discovered some interesting properties of existing (semi-)synthetic datasets, we also tested respective models trained on those dataset 



==> RQ_answers/rq2.tex <==
% !TEX root = ../fse_results.tex

\subsection{Limitations of existing \vp approaches (RQ2)}
\label{sect:rq2}


% \input{RQ_answers/Tables/rq1_boxplots}

% \noindent\textbf{RQ2:}~\textit{How effectively and accurately \tool can detect real world vulnerabilities?}


\motivation In this research question, we evaluate the effectiveness of \tool to detect real world vulnerabilities. While comparing with existing baselines, we empirically compare and contrast different techniques with \tool.

\approach To compare the performance, we adopt three \vp baseline techniques (\ie VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and Russel~\etal~\cite{russell2018automated}) proposed in existing literature and train those on two real world datasets (\realdata and \devigndata). For VulDeePecker, we extracted the code slices from API calls (backward slice only as reported by VulDeePecker) in the code. For SySeVR, along with API call slice, we also extract the slices from Array Index, Arithmetic expression, and Pointer Usage. Slicing results in numerous duplicates. For instance, in the same line if an API is called with a pointer access, we will have two different slices (one from API slice, one from pointer slice). We de-duplicate such repetition of slices. Note that, with VulDeePecker and SySeVR, we could not extract slices for all the examples in the dataset two dataset(\ie \realdata, and \devigndata). For the examples where slices could not be extracted, we classify them as non-vulnerable. If at least one slice from an example is classified as vulnerable by the model, we classify that example as vulnerable. For all three of these techniques, we use the tokenization method reported by the respective reports. In addition, we adopt another graph neural network based baseline, Devign, proposed by Zhou \etal~\cite{zhou2019devign}. We note that Zhou~\etal did not make their implementation and hyper-parameter details are not publicly available, we therefore re-implemented Devign. 


\observations Table~\ref{tab:all_method_comparison_real_world_datasets} shows the result of different approaches in predicting vulnerability in real world. Here we report the accuracy, precision, recall, and F1 score in each case. These performance measures are median on scores across 30 runs. We also show the inter-quartile range (IQR) to understand the spread of performances across the median. The median and IQR for the F1-score is visualized as a candlestick plot in the last column in~\cref{tab:all_method_comparison_real_world_datasets}.

% \input{RQ_answers/Tables/rq1_range_plots}
\noindent$\circ$~ \textit{\realdata.}~\tool performs best in terms of F1-score and recall. The median recall is $51.85\%$ higher and median F1-score is $36.36\%$ higher than the next best baseline (SySeVR). While \devign produces the best precision, \devign's median recall $56.21\%$ less than that of \tool. This indicates while \devign results in slightly lower number of false positives (better precision) at the cost of a large number of false negatives (lower recall). Overall, \tool's median F1-score is $38.09\%$ higher than \devign. 


% \Cref{fig:verun_bp} shows contrasting visual representation of the spread of different performance metrics. We observe that \tool yields statistically significant better f1-score compared to other baselines.
\noindent$\circ$~ \textit{\devigndata.} In this dataset, \tool performs best with respect to all performance metrics. \tool's median accuracy, precision, recall, and F1-scores are 5.01\%, 5.19\%, 13.11\%, and 12.64\% higher respectively than the next best baseline.
% ~\Cref{fig:devign_bp} shows visual representation of spread of precision, recall, and f1-score for the approaches across 30 runs. In terms of F1-score, \tool is best among those approaches with statistical significance.  

We conjecture that the consideration of the code semantics results in the improved performance of the semantics-based models over those of syntax-based model. In Russel~\etal's approach, code fractions that are syntactically related might be interspersed with numerous semantically and syntactically irrelevant code fragments. When slices are extracted in VulDeePecker and SySeVR, all irrelevant code fragments are stripped away from the slice. Thus, from a DL model's perspective, it is easier to reason about slice than to reason about the whole code presented to it as a series of tokens. In contrast to the slice based models, when complete code property graph is presented to the model, it can reason about much richer information in the graph thus results in more effective \vp.

% Graph models are in general better than semantics models since models built on graphs have richer information available to reason about. 

% Code semantics is very important while detecting real world vulnerability. Syntax based models do not perform very well in real world \vp task. Models trained on code slices from control and data dependency do have some semantic information to reason about, and thus performs better than syntax based counterparts. 


\begin{result}
\tool performs significantly better than token based and sliced based methods on both real-world datasets. We also show that, \tool's graph embedding model when used in conjunction with re-sampling and representation learning perform noticeably better than vanilla GGNN.
\end{result}

% 

% \red{Saikat: This paragraph reads like a summary, move to the result box} We observe that all those techniques do not achieve the same level of performance in real world dataset as those in (semi)-synthetic datasets. We also find that, to find vulnerability in real world dataset, model should consider the semantics of the code, in contrast to considering code as token sequences.

% \smallskip
% \noindent\textbf{\small RQ2: How do different \dlvp approaches perform when trained on real world data} 




% \result{}

% Next, we focused on the structure of the code. First, we wanted some model based on the syntactic structure of the code. For doing so, we parsed the code into nodes using Joern~\cite{yamaguchi2015automatic}. These node mostly include AST nodes, other nodes include variable definition nodes, CFG nodes etc. We initialize each node with node type and node features. We extract node feature using Word2Vec~\cite{rong2014word2vec}. After getting the representation of every node, we get the graph level representation by summing up all the node in a graph. Hence, every graph is transformed to a real valued vector containing the information about all the node in that graph. Then we classify these vectors using traditional machine learning tools \eg Support Vector Machine (SVM), Logistic Regression (LR), K-Nearest Neighbor(KNN) etc. Note that, any trainable ML model can be used for this experiment, we chose these three as case study model. Also note that, while computing the graph representation in this case, we are not considering the any edges in the graph. Thus this representation is \emph{not} a complete semantic model, since semantic information (through control and data dependency edge) are not present here. 

% Finally, we consider the semantic model. For doing so, we collect the graph with six different type of edges \ie AST, control flow, data flow, data dependency (def-use), DOM and PDOM edges. We initialize the node in the same way as decribe in previous step. We then pass this graph to Gated Graph Neural Network(GGNN)~\cite{li2015gated}.  After generating the final representation of every node in a GGNN, we calculate the graph level representation by summing up all the node information and then pass that graph representation to a Fully Connected Neural Network to classify into vulnerable and non-vulnerable category. 

% In each case, we randomly split the dataset into 80\%-20\% train-test sets. To avoid any biases created by this randomness, we repeat the experiment 30 times.


% This result gives us a \emph{rough estimate} of how different types of model perform in predicting vulnerability. 



% As we can see, Graph + DL (GGNN) model performs best in both \realdata and \devigndata in terms of F1- score. In both the dataset, GGNN gives the highest recall (with statistical significance) meaning that it predicts less number of false negatives. KNN has the highest average value of precision. However, the precision result of KNN are \emph{not} significantly better compared to other method with statistical significance.

% Note that, among the token based models, SySeVR performs very well in both the datasets. However, as we have already mentioned, 66.42\% of the test code in \realdata and 84.08\% in \devigndata are in the scope for SySeVR (\ie at least once slice can be extracted following the 4 slice extraction method proposed by SySeVR). The performance of SySeVR and VulDeePecker in Table~\ref{tab:all_method_comparison_real_world_datasets} are \wrt to the code that are in-scope only for respective technique. 

% \smallskip
% \noindent\textbf{Observation 2.1} Semantic information and reasoning about it, plays a very important role in \vp task. Models that explicitly learn from semantic graph perform better in real world \vp. Having limited semantics information, VulDeePecker and SySeVR learn to do some reasoning about the semantics of the code and hence perform well in cases where appropriate slice can be extracted. In fact, SySeVR works very well in examples that are in its' scope. SySeVR proposed four different types if entry points for extracting slices. 

% In theory, slices can be extracted from any point of the program. However, if we extract slices from every point in the code, number of slices will explode. This problem is similar to the path explosion problem in testing~\cite{boonstoppel2008rwset}. Thus we argue, reasoning on graph as a whole instead of reasoning on individual slices are better choices. 

% Since rest five methods (Russel~\etal~\cite{russell2018automated}, SVM, LR, KNN, and GGNN) work with 100\% of the data, we present a Scott-Knott ranking on the F1 score of different approaches to prove an approach is better with statistical significance.
% \smallskip
% \noindent\textbf{Statistically Sound Comparison.} As described in Section~\ref{subsec:real-world-evaluation}, to prove a technique is better than another, some statistical test is necessary. There are several statistical test available to testing hypotheses with different assumptions and different properties. For instance, t-statistic test assumes that the samples we are testing would follow a gaussian distribution. In our evaluation, we will be comparing performance of multiple approaches. For such case, Scott-Knott method is championed by software engineering researchers~\cite{krishna2018bellwethers, mittas2012ranking}. For a group of samples (in our case performance measures), Scott-Knott, recursively splits the group to establish statistical significance of one group over other using Hypothesis testing. In theory, any hypothesis testing can be used in conjunction to Scott-Knott method. In our evaluation, we followed the A12 test, which has been highly used and championed in Software Engineering research~\cite{krishna2018bellwethers}.

% \input{Tables/rq2_comparison}

% Table~\ref{tab:statistical_comparison} shows the ranking of those five methods, the median performance, and Inter-Quartile Range(IQR) of each of the approaches. As we can see, in both the dataset, GGNN is in the top rank and is not ties with any other method. Here is an interesting finding from this result, even though Russel~\etal has the higher average f1-score than SVM in \realdata, it is not significantly better. Thus, in Table~\ref{table:comparison_chrome_deb_f1}, those two method are tied in third rank. Similarly, in \devigndata, SVM, LR and Russel~\etal are not significantly better than one another.

% \smallskip
% \noindent\textbf{Observation 2.2. Having good result in one run of the experiment, even having good result on average does not prove a method is significantly better than other.}

% Thus we summarize the lessons learned in this research question, 

% \smallskip
% \noindent\textbf{Lesson 2} Graph based models should be used for real world \vp. Further investigation of improved graph based model will unveil better reasoning. While comparing with two approaches, statistical significance test should be performed to rule our the ``luck factor''.



% \begin{table}[]
%     \centering
    
% \end{table}

% \begin{table}[!htb]
%     \centering
    
% \end{table}


% \noindent\textbf{RQ2. Why do current vulnerability prediction models fail in real-world situations?}

% In this RQ, we thoroughly investigate why existing Deep Learning based Vulnerability Detection systems fail to generalize in real world scenario. We investigate the problems with existing approaches from different angles -- first, we investigate the data on which the models pre-trained on; second, we investigate different aspect of the existing approaches. 

% Our first part of investigate research question is 

% \noindent\textbf{Experiment 2.1.2} As we have seen in the previous experiment, the existing datasets are highly repetitive, we investigate on the learned features from those datasets. To understand that better, we intend to examine the activation of the data with respect to its predictions, namely what kind of patterns are triggering the prediction for a piece of code to be vulnerable. As a case study, we examine the trained CNN model. We use the guided back-propagation technique~\cite{springenberg2014striving} to calculate the gradient given its prediction label with respect to the input token embedding. 
% To understand what is actually triggering a prediction, we only take the positive guided-gradients and normalize it. Since each embedding is a vector, to get the activation value per embedding, we sum them over the embedding dimension. The procedure is described in Algorithm~\ref{algo:guided_backprop} in details.

% \begin{algorithm}
% \footnotesize
% \SetAlgoLined
% \KwResult{Activation values $av_{i,j}$ for $i^{th}$ sample's $j^{th}$ token}
%  \textbf{Input} Data $x_i, \forall i \in \{1,\ldots, N\}$ with sequence length $M$ and embedding size $K$\;
%  \textbf{Model} $F(\cdot): \mathbb{R}^{M\times K} \to \mathbb{R}^{2}$\;
%  \For{$i \in \{1,\ldots, N\}$}{
%  $\hat{y_i} = \arg \max F(x_i)$\;
%  $\nabla_i = $ GuidedBackPropagation($F(\cdot), x_i, \hat{y_i}) \in \mathbb{R}^{M\times K}$\;
%  $\nabla_i^{+} = \max(0, \nabla_i) ./ \max(\nabla_i)$\;
%  $av_i = $ RowSum($\nabla_i^{+}$) $\in \mathbb{R}^{M}$
%  }
%  \caption{The procedure for obtaining activation values using guided back-propagation.}
%  \label{algo:guided_backprop}
% \end{algorithm}

% Since we are dealing with sequences, we search for the top sub-sequences that have highest average activation values in between consecutive tokens up to a certain length across the data entries. In this case we set the maximum length to five based on our experiment results. These sub-sequences are  the top features that the CNN model is learning. To investigate the prevalence of those features, we also calculated the top features' prevalence ratio, that is defined as the following.

% The prevalence ratio for $i^{th}$ feature ($f_i$) of $j^{th}$ class ($y=j$):

% \begin{align*}
%     \mathrm{Prevalence_{i, j}} = \frac{\sum_{k:\; y_k = j} \mathrm{Count}_{f_i}(x_k)}{\sum_{k:\; y_k \neq j} \mathrm{Count}_{f_i}(x_k)} \cdot \frac{|\{x_k:\; y_k \neq j\}|}{|\{x_k:\; y_k = j\}|}
% \end{align*}
% $\mathrm{Count_{f_i}(\cdot)}$ counts the number of occurrence of $f_i$ in its input, $|\{x_k:\; y_k = j\}|$ calculates the number of samples that belongs to $j^{th}$ class, similarly $|\{x_k:\; y_k \neq j\}|$ calculates the number of samples that does not belong to $j^{th}$ class.

% In plain English, the higher the prevalence ratio, the more the featured appeared in the specified class.

% \input{Tables/learned_features}

% \noindent \textbf{Result 2.1.2:} It can be observed that the model learnt different features from different datasets. In general, the top features can not be directly linked to any vulnerabilities by simply looking at it except for the features learnt from Github + Debian~\cite{russell2018automated}, which is likely to be related to buffer overflow but it is also plausible to be an artifact due to its high prevalence ratio. 

% The top features learnt from SATE IV Juliet~\cite{okun2013report} are mostly related to referencing variables and identifiers, difficult to see what these features represent but not necessarily meaningless. The features have low prevalence ratio which indicates that they are not learnt based on local patterns.

% \begin{figure}
%     \centering
% \begin{lstlisting}
% init_JSON_config(JSON_config* config)
% {
%     if (config) {
%         memset(config, 0, sizeof(*config));
%         config->depth = JSON_PARSER_STACK_SIZE - 1;
%         config->malloc = malloc;
%         config->free = free;
%     }
% }
% \end{lstlisting}
%     \caption{\small{\textbf{One non-vulnerable code example from Github + Debian~\cite{russell2018automated} dataset that contains the top features (such as {\tt malloc}) and was misclassified as vulnerable.}}}
%     \label{lst:codesample}
% \end{figure}
% \vspace{-6mm}

% Most of the top features learnt from VulDeePecker~\cite{okun2013report} are clearly not related to vulnerabilities, ``5" and ``[ 5" are likely appeared in the original dataset as a part of some Flow Variants. The last feature ``FUNC ( DEC , LITERAL" could be related to vulnerabilities induced by function calling. However, it has two features that have prevalence ratio greater than one, which point out that these two, especially ``- LITERAL ;", might be an artifact. 
% The top features learnt from SySeVR~\cite{li2018sysevr} are similar to the features learnt from VulDeePecker~\cite{li2018vuldeepecker}, mostly related manipulation of variables that are difficult to decipher. However, they have three features with greater than one prevalence ratio, which indicates that the features are likely to be bound locally.

% The top features learnt from Github + Debian~\cite{russell2018automated} are significantly different from the previous, all of them are C/C++ library functions such as {\tt fopen}, {\tt malloc}, {\tt memcpy} and {\tt read}. Notice that these features have much higher prevalence ratio than the previous features, also these functions is highly likely to be related to memory/buffer-based vulnerabilities, we conjure that these features might be caused by its labelling functions that are static analyzers, which are inclined to be artifacts. Listing~\ref{lst:codesample} shows an example to illustrate a typical scenario where these learnt features might misguide the prediction. In this case, the buffer overflow is properly handled and hence it is not a vulnerable code. However, this code snippet is classified as vulnerable by the model. So although the learned features are more reasonable, the system is still far from perfect.

% \noindent \textbf{Observation 2.1.2 :} The code sub-sequences that are learned as top features by existing Deep Learning are not directly related to vulnerability. High prevalence of such features forces models to learn those patterns instead of effectively learning the vulnerability patterns. 

% So far, we have seen that the four synthetic dataset are biased. Now we are curious to see why those model should not work if trained on real world code and real world vulnerability annotations. Thus, the second part of our research question, \textbf{RQ2.2 What are the challenges with the available approaches?}

% \noindent\textbf{Experiment 2.2 } To answer this question, we systematically investigate several aspects -- \eg code pre-processing method, code abstraction methods, type of the models, etc., from the existing approaches. We observe that CNN~\cite{russell2018automated}, BLSTM~\cite{li2018vuldeepecker}, BGRU~\cite{li2018sysevr} all are token based models. In addition, all these approaches use symbolic code pre-processing techniques, where concrete identifier names are replaced by abstract identifiers. To this end, we investigate,
% \textit{What if we use concrete identifier names instead of the abstract?},  
% \textit{What if we consider structural and semantic information of the code?}, and
% \textit{What if we learn structural neural networks for code?}

% We first trained a Word2Vec~\cite{rong2014word2vec} model trained on large corpus of code. 
% To really understand the contribution of concrete identifier names, we design a simple SVM based model on top of the Word2Vec based token embedding. Next, we concatenate the AST node type information with the token embedding and use SVM to understand influence of AST information. Finally, we design a Graph Based Neural Network to detect vulnerability given the flow graph of a program.  

% \textbf{Result 2.2 } Table~\ref{tab:rq2_table} shows accuracy and F1 score on \realdata and Devign dataset. As the results show in both the cases, if we use Word2Vec, even a very simple model line Linear SVM outperforms Deep Learning based CNN + RF models' performance. The F1 score increases from 45.71 to 53.18 in Devign data and from 8.78 to 16.55 in \realdata respectively. This result clearly indicates the code tokens play important role in real-world vulnerability detection task. In addition, if we add AST node type information, the performance increases slightly. Finally, we extract the control and data flow graph from the program function and use Graph Based Neural Network to classify that. Similar graph neural network based technique is recently used by Xhou~\etal~\cite{zhou2019devign}. When a Graph Neural Network is used, the F1 score increases to 61.61 in Devign dataset and 25.97 in \realdata rendering 35\% and 195\% improvement than that of original CNN + RF approach. 

% \noindent\textbf{Observation 2.2 } Concrete names of the code tokens, structural and semantic information play very important role in real life vulnerability detection. Existing models ignored these properties and hence failed to work well in real world scenario. 



% % \begin{itemize}
% %     \item Data Problem
% %     \begin{itemize}
% %         \item Clone
% %         \item Repetitive Features
% %     \end{itemize}
% %     \item Approach Problem
% %     \begin{itemize}
% %         \item Preprocessing
% %         \item Simple model 
% %     \end{itemize}
% % \end{itemize}


% % \noindent \textbf{Data Problem}


==> RQ_answers/rq2_new.tex <==
\begin{figure*}[tpb!]
    \centering
    \begin{subfigure}{0.2\linewidth}
    \centering
    \includegraphics[width=\linewidth]{RQ_answers/tsne_plots/VulDeePecker.pdf}
    \caption{VulDeePecker}
    \label{fig:vuldeepecker-t-sne}
    \end{subfigure}
    \begin{subfigure}{0.2\linewidth}
    \centering
    \includegraphics[width=\linewidth]{RQ_answers/tsne_plots/SySeVR.pdf}
    \caption{SySeVR}
    \label{fig:sysevr-t-sne}
    \end{subfigure}
    \begin{subfigure}{0.2\linewidth}
    \centering
    \includegraphics[width=\linewidth]{RQ_answers/tsne_plots/Russell.pdf}
    \caption{Russell~\etal }
    \label{fig:russell-t-sne}
    \end{subfigure}
    \begin{subfigure}{0.2\linewidth}
    \centering
    \includegraphics[width=.78\linewidth]{RQ_answers/tsne_plots/devign.pdf}
    \caption{Devign}
    \label{fig:russell-t-sne}
    \end{subfigure}
    \caption{t-SNE plots illustrating the separation between vulnerable (denoted by \red{$+$}) and non-vulnerable (denoted by {$\mathbf{\circ}$}) example. Existing methods fail to optimally separate vulnerable and non-vulnerable classes.}
    \label{fig:t-sne-plots}
    \saikat{use a dark and a red color. Also add REVEAL separation here.}
\end{figure*}

\subsection{Key limitations of existing \vp approaches (RQ2)}
\label{sect:rq2}

In RQ1, we showed that existing approaches are not effective in detecting real-world vulnerabilities. 
In this research question, we investigate the reasons why existing approaches are ineffective. We find that the existing approaches suffer from a number of problems.

\input{RQ_answers/Tables/rq1_duplicate_results}
\smallskip

\subsubsection{Duplication}
Preprocessing techniques such as slicing used by VulDeePecker and SySeVR and tokenization used by Russell~\etal introduces a large number of duplicates in both the training and testing data. There are several ways duplication can be introduced by the preprocessing techniques used by the DLVP method -- \eg same slice can be extracted from different entry points, different code can have same token sequence due to the abstract tokenization adopted by the approaches\footnote{For details about the slicing and tokenization, we refer to \Cref{sect:background} and respective papers~\cite{li2018sysevr, russell2018automated, li2016vulpecker}}. 

\tab{duplicate} tabulates the number of duplicates introduced by some of the \vp approaches. We observe that the preprocessing technique employed by SySeVR and VulDeePecker (\ie., slicing followed by tokenization) introduces a significant amount of ($>\mathit{60\%}$) duplicate samples. In addition to the preprocessing technique, the number of duplicates depends also on dataset. Commonly used, (semi-)synthetic datasets such as NVD, SARD, and Juliet are comprised of much simpler code snippets and result in large number of duplicates. Ideally, a DL based model should be trained and tested on a dataset where 100\% of the examples are unique. Duplication tends to artificially inflate the overall performance of the method~\cite{allamanis2019adverse}. Therefore, pre-trained \vp models that introduce significant number of duplicates won't generalize to complex real-world datasets. This partially explains the poor performance of pre-trained models shown in~\tab{pretrained}.

In contrast, real-world datasets such as~\devigndata and \realdata are much more complex and therefore have far fewer duplicates. Real-world data, prior to preprocessing, contain little to no duplicates.
%\bray{give the numbers before preprocessing.}
For instance, SySeVR's pre-processing technique introduces 25.56\% duplicates in \realdata (original dataset had only 0.6\% duplicates). Likewise, SySeVR's pre-processing technique introduces 22.10\% duplicates in \devigndata (whereas the original dataset contains about 0.2\% duplicates). 
%While the number of duplicates introduced in real-world data is lower than (semi-)synthetic data, after de-duplication

%\noindent
\subsubsection{Data Imbalance} The datasets used by existing methods are tabulated in~\tab{existing_approach_design_choices}. We notice that several datasets exhibit a notable imbalance in the fraction of vulnerable and non-vulnerable examples. A model trained on such skewed datasets is susceptible to being considerably biased toward the majority class. Existing methods fail to adequately address the data imbalance during training. This limits the effectiveness of the models exposed to datasets that have a different ratio of vulnerable and non-vulnerable examples. 

\subsubsection{Model Selection}

\subsubsection{Lack of Separability} Existing approaches use pre-processing techniques to translate source code into a numeric feature vector that can be used to train a \vp model. The efficacy of this \vp model depends on how separable the feature vectors of vulnerable examples are from and the feature vectors of  non-vulnerable examples. The greater the separability of the  To visualize the separability of the feature vectors we use t-SNE plots.    


% To compare the performance, we adopt three \vp baseline techniques (\ie VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and Russel~\etal~\cite{russell2018automated}) proposed in existing literature and train those on two real world datasets (\realdata and \devigndata). For VulDeePecker, we extracted the code slices from API calls (backward slice only as reported by VulDeePecker) in the code. For SySeVR, along with API call slice, we also extract the slices from Array Index, Arithmetic expression, and Pointer Usage. Slicing results in numerous duplicates. For instance, in the same line if an API is called with a pointer access, we will have two different slices (one from API slice, one from pointer slice). We de-duplicate such repetition of slices. Note that, with VulDeePecker and SySeVR, we could not extract slices for all the examples in the dataset two dataset(\ie \realdata, and \devigndata). For the examples where slices could not be extracted, we classify them as non-vulnerable. If at least one slice from an example is classified as vulnerable by the model, we classify that example as vulnerable. For all three of these techniques, we use the tokenization method reported by the respective reports. In addition, we adopt another graph neural network based baseline, Devign, proposed by Zhou \etal~\cite{zhou2019devign}. We note that Zhou~\etal did not make their implementation and hyper-parameter details are not publicly available, we therefore re-implemented Devign. 

% We categorize the above approaches in three categories -- (a) Token models, (b) Slice with token models, and (c) Graph model. Russel~\etal~\cite{russell2018automated}'s proposed approach is purely syntax based approach, since they consider the code as a sequence of tokens. Thus, their approach fall into token based modeling category. VulDeePecker~\cite{li2018vuldeepecker} and SySeVR~\cite{li2018sysevr}, in contrast, extract code slices from Control flow and data flow graphs and use token based models to predict vulnerabilities on those slices.These models fall into Slice + Token category. These two approaches consider some form of semantics into account. In case of \devign and \tool, a graph representation of the code is considered in the model. Thus these two methods are categorized as graph based models.

% Table~\ref{tab:all_method_comparison_real_world_datasets} shows the result of different approaches in predicting vulnerability in real world. Here we report the accuracy, precision, recall, and F1 score in each case. These performance measures are median on scores across 30 runs. We also show the inter-quartile range (IQR) to understand the spread of performances across the median. The median and IQR for the F1-score is visualized as a candlestick plot in the last column in~\cref{tab:all_method_comparison_real_world_datasets}.

% \noindent$\circ$~ \textit{\realdata.}~\tool performs best in terms of F1-score and recall. The median recall is $51.85\%$ higher and median F1-score is $36.36\%$ higher than the next best baseline (SySeVR). While \devign produces the best precision, \devign's median recall $56.21\%$ less than that of \tool. This indicates while \devign results in slightly lower number of false positives (better precision) at the cost of a large number of false negatives (lower recall). Overall, \tool's median F1-score is $38.09\%$ higher than \devign. 


% \noindent$\circ$~ \textit{\devigndata.} In this dataset, \tool performs best with respect to all performance metrics. \tool's median accuracy, precision, recall, and F1-scores are 5.01\%, 5.19\%, 13.11\%, and 12.64\% higher respectively than the next best baseline.

% We conjecture that the consideration of the code semantics results in the improved performance of the semantics-based models over those of syntax-based model. In Russel~\etal's approach, code fractions that are syntactically related might be interspersed with numerous semantically and syntactically irrelevant code fragments. When slices are extracted in VulDeePecker and SySeVR, all irrelevant code fragments are stripped away from the slice. Thus, from a DL model's perspective, it is easier to reason about slice than to reason about the whole code presented to it as a series of tokens. In contrast to the slice based models, when complete code property graph is presented to the model, it can reason about much richer information in the graph thus results in more effective \vp.

\begin{result}
\tool performs significantly better than token based and sliced based methods on both real-world datasets. We also show that, \tool's graph embedding model when used in conjunction with re-sampling and representation learning perform noticeably better than vanilla GGNN.
\end{result}


==> RQ_answers/rq3.tex <==
\subsection{Effect of Graph Neural Network (RQ3)}
\label{sect:rq3}
% \noindent\textbf{RQ3:}\textit{ What is the effect of GGNN in \tool’s performance?}


\motivation In this research question, we investigate the impact of GGNN in \tool's pipeline. Recall from~\Cref{fig:intro_fig} and~\Cref{sect:feature_extraction}, \tool refines each vertex feature by assimilating the features of all the neighboring vertices through GGNN (see line 8 from Alg.~\ref{alg:feature_extraction}). We intuit that, as GGNN updates each vertex's feature vector by accumulating all the neighboring vertex's information, every vertex has some extra information not only about itself, but also about the structure of the graph. 

\input{RQ_answers/Tables/rq2_wo_ggnn}
\input{RQ_answers/Tables/rq2_boxplot}

\approach To test the impact of this step, we create a variant of \tool with GGNN disabled. In this setup, we bypass the use GGNN and aggregate the initial vertex features to create the graph features. Further, we create another variant of \tool that uses GGNN, but does not use re-sampling or representation learning. 

\observations\Cref{tab:comparison_wo_ggnn} shows the performance to \tool with and without GGNN. \Cref{fig:ggnn_abl} shows the visual representation of F1-score for both the models in consideration. We observe that, in both \realdata and \devigndata, F1-score increases when we use GGNN in \tool's pipeline. We observe that the improvements offered by the use of GGNN is statistically significant (with a p-value of \red{0.0002 in \realdata, and 0.001 in \devigndata}). Further, when we perform the A12 effect size~\cite{hess2004robust} with 30 independent experiment runs in each case, we found that the the effect size is 81\% for \realdata and 73\% for \devigndata. This means that 81\% of the times \tool performs better with GGNN than it does without GGNN in \realdata and 73\% in \devigndata. Both of those effect sizes are considered large indicating \tool with GGNN's f1-score distribution is better than \tool without GGNN. 

We contend that, since GGNN embeds the neighbors' information in every node, nodes have richer information about the graph. Thus \tool's classification model have more information at its disposal to reason about. The result indicates that when nodes assimilate information from other nodes through graph edge, \vp performance increases. Finding better ways to do such assimilation is out of this project's scope and we leave that for future work.


\begin{result}
GGNN improves \tool's performance when used in the pipeline. The median performance is improved by 5.5\% in \realdata and 1.15\% in \devigndata. In both cases, the improvement is statistically significant with large effect sizes.
\end{result}

==> RQ_answers/rq4.tex <==
\subsection{Effect of Training Data Balancing (RQ4)}
\label{sect:rq4}

% \noindent\textbf{RQ4:} \textit{What  is  the  effect  of  data  balancing  in  \tool’s performance?}

\motivation \tool re-samples the training dataset to create a balance between vulnerable and non-vulnerable examples using SMOTE to reduce bias created by majority non-vulnerable examples. In this research question, we investigate the effect of such training data balancing. 

\input{RQ_answers/Tables/rq3_balancing}
\input{RQ_answers/Tables/rq3_boxplot}


\approach In this research question, we create a baseline by turning off the SMOTE. In that baseline, \tool's model is trained on the imbalanced dataset. Note that, \tool uses SMOTE as off-the shelf data balancing tool. Choice of this data balancing tool is a configurable parameter in \tool's pipeline. Study on the effect of other alternatives is beyond the scope of this project. 

\observations \Cref{tab:comparison_wo_smote} shows the effect of using data re-sampling in \tool's pipeline. \Cref{fig:balance_abl} shows the spread of F1-score \wrt the usage of data re-sampling.  Re-balancing training data improves \tool's performance in general. The improvement increases significantly with the increased imbalance ratio in the training data. When training data is highly imbalanced, the classifier is biased by the majority class. In case of \realdata, the model is biases towards the non-vulnerable class (non-vulnerable examples consists of $\sim$90\% of the dataset), thus in test time it tends to predict everything as non-vulnerable. The effect of this increases false-negative predictions quite significantly reducing the recall. 



\begin{result}
Training data re-balancing improves \tool's performance by 128\% in \realdata and 4.9\% in \devigndata. The effect of data re-balancing is very high when the initial training data is highly imbalanced.
\end{result}

==> RQ_answers/rq4_new.tex <==
\subsubsection{Effect of Graph Neural Network (RQ3)}
\label{sect:rq3}
% \noindent\textbf{RQ3:}\textit{ What is the effect of GGNN in \tool’s performance?}


\motivation In this research question, we investigate the impact of GGNN in \tool's pipeline. Recall from~\Cref{fig:intro_fig} and~\Cref{sect:feature_extraction}, \tool refines each vertex feature by assimilating the features of all the neighboring vertices through GGNN (see line 8 from Alg.~\ref{alg:feature_extraction}). We intuit that, as GGNN updates each vertex's feature vector by accumulating all the neighboring vertex's information, every vertex has some extra information not only about itself, but also about the structure of the graph. 

\input{RQ_answers/Tables/rq2_wo_ggnn}
\input{RQ_answers/Tables/rq2_boxplot}

\approach To test the impact of this step, we create a variant of \tool with GGNN disabled. In this setup, we bypass the use GGNN and aggregate the initial vertex features to create the graph features. Further, we create another variant of \tool that uses GGNN, but does not use re-sampling or representation learning. 

\observations\Cref{tab:comparison_wo_ggnn} shows the performance to \tool with and without GGNN. \Cref{fig:ggnn_abl} shows the visual representation of F1-score for both the models in consideration. We observe that, in both \realdata and \devigndata, F1-score increases when we use GGNN in \tool's pipeline. We observe that the improvements offered by the use of GGNN is statistically significant (with a p-value of \red{0.0002 in \realdata, and 0.001 in \devigndata}). Further, when we perform the A12 effect size~\cite{hess2004robust} with 30 independent experiment runs in each case, we found that the the effect size is 81\% for \realdata and 73\% for \devigndata. This means that 81\% of the times \tool performs better with GGNN than it does without GGNN in \realdata and 73\% in \devigndata. Both of those effect sizes are considered large indicating \tool with GGNN's f1-score distribution is better than \tool without GGNN. 

We contend that, since GGNN embeds the neighbors' information in every node, nodes have richer information about the graph. Thus \tool's classification model have more information at its disposal to reason about. The result indicates that when nodes assimilate information from other nodes through graph edge, \vp performance increases. Finding better ways to do such assimilation is out of this project's scope and we leave that for future work.


\begin{result}
GGNN improves \tool's performance when used in the pipeline. The median performance is improved by 5.5\% in \realdata and 1.15\% in \devigndata. In both cases, the improvement is statistically significant with large effect sizes.
\end{result}

==> RQ_answers/rq5.tex <==
\subsection{Effect of Representation Learning (RQ5)}
\label{sect:rq5}

% \noindent\textbf{RQ5:} \textit{How does \tool perform when other classifiers are used instead of Representation Learning?}


\motivation In this research question, we investigate \tool's chose of model for representation learning. Recall from~\Cref{sect:training}, \tool uses Multi Layer Perceptron (MLP) with triplet loss (see~\Cref{eqn:full_loss}). We investigate use of other models and use of the triplet loss.

\input{RQ_answers/Tables/rq4_models}
\input{RQ_answers/Tables/rq4_boxplot}

\approach Our first obvious baseline is MLP without the triplet loss (MLP$^\dagger$). In such a baseline, we use MLP as classifier with Negative Log Likelighood (NLL) loss~\cite{platt1999probabilistic}.\\
Similar to \tool, Russell~\etal~\cite{russell2018automated}'s proposed approach deconstructed the \vp task in two step method. They used Random Forest(RF) classifier as their representation learning model. To investigate RF model's suitability in \tool's pipeline, we create second baseline \tool with RF as classifier (RF). \\
Objective of \tool's triplet loss is to maximally separate vulnerable and non-vulnerable examples. Support Vector Machine (SVM) with radial basis function kernel~\cite{baesens2000empirical} learns similar objective. We create our third baseline where we use SVM with RBF as classifier (SVM). 

\observations \Cref{tab:comparison_models} shows the \tool's performance with different classification models. In both \realdata and \devigndata, \tool with MLP and triplet loss achieves best performance. \tool's median F1-score is 62.8\%, 13.3\%, 3.5\% higher than that of RF, MLP$^{\dagger}$, and SVM baselines respectively in \realdata. For \devigndata improvement in median F1-score is 23.33\%, 7.5\%, 6.5\% respectively. \Cref{fig:model_abl} shows the spread of F1-score with  different classification models. 

Max-margin models results in better performance in classifying vulnerable code in general. \tool with MLP and triplet loss performs even better than SVM with statistical significance in both \realdata and \devigndata. We conjecture that such improvement is attributed to the fact that SVM is shallower model than \tool's representation learning model, thus \tool learn more complex patterns than SVM.


\begin{result}
\tool's representation learning model with MLP and triplet loss performs best compared to other machine learning models. \tool increases median F1-score by 3.5\% and 6.5\% respectively in \realdata and \devigndata respectively compared to SVM. \tool's loss function increases F1-score 13.3\% and 7.49\% in \realdata and \devigndata compared to NLL loss with MLP.
% Representation Learning in \tool with MLP and Triplet loss results in best performance compared to other models with statistical significance.  
\end{result}

==> RQ_answers/rq5_new.tex <==
\subsubsection{Effect of Representation Learning (RQ5)}
\label{sect:rq5}

% \noindent\textbf{RQ5:} \textit{How does \tool perform when other classifiers are used instead of Representation Learning?}


\motivation In this research question, we investigate \tool's chose of model for representation learning. Recall from~\Cref{sect:training}, \tool uses Multi Layer Perceptron (MLP) with triplet loss (see~\Cref{eqn:full_loss}). We investigate use of other models and use of the triplet loss.

\input{RQ_answers/Tables/rq4_models}
\input{RQ_answers/Tables/rq4_boxplot}

\approach Our first obvious baseline is MLP without the triplet loss (MLP$^\dagger$). In such a baseline, we use MLP as classifier with Negative Log Likelighood (NLL) loss~\cite{platt1999probabilistic}.\\
Similar to \tool, Russell~\etal~\cite{russell2018automated}'s proposed approach deconstructed the \vp task in two step method. They used Random Forest(RF) classifier as their representation learning model. To investigate RF model's suitability in \tool's pipeline, we create second baseline \tool with RF as classifier (RF). \\
Objective of \tool's triplet loss is to maximally separate vulnerable and non-vulnerable examples. Support Vector Machine (SVM) with radial basis function kernel~\cite{baesens2000empirical} learns similar objective. We create our third baseline where we use SVM with RBF as classifier (SVM). 

\observations \Cref{tab:comparison_models} shows the \tool's performance with different classification models. In both \realdata and \devigndata, \tool with MLP and triplet loss achieves best performance. \tool's median F1-score is 62.8\%, 13.3\%, 3.5\% higher than that of RF, MLP$^{\dagger}$, and SVM baselines respectively in \realdata. For \devigndata improvement in median F1-score is 23.33\%, 7.5\%, 6.5\% respectively. \Cref{fig:model_abl} shows the spread of F1-score with  different classification models. 

Max-margin models results in better performance in classifying vulnerable code in general. \tool with MLP and triplet loss performs even better than SVM with statistical significance in both \realdata and \devigndata. We conjecture that such improvement is attributed to the fact that SVM is shallower model than \tool's representation learning model, thus \tool learn more complex patterns than SVM.


\begin{result}
\tool's representation learning model with MLP and triplet loss performs best compared to other machine learning models. \tool increases median F1-score by 3.5\% and 6.5\% respectively in \realdata and \devigndata respectively compared to SVM. \tool's loss function increases F1-score 13.3\% and 7.49\% in \realdata and \devigndata compared to NLL loss with MLP.
% Representation Learning in \tool with MLP and Triplet loss results in best performance compared to other models with statistical significance.  
\end{result}

==> RQ_details/rq1.tex <==
\subsection{Limitations of Synthetic Data (RQ1)}
\label{sect:rq1}


In this RQ, we investigate the limitations of (semi-)synthetic data and their capabilities in predicting real-world vulnerabilities. We start with a straightforward question: how do the models trained with  (semi-)synthetic dataset perform on detecting real-world vulnerabilities. Without much of a surprise, we found that they perform poorly.  Our in-depth investigation reveals that these datasets are too simple and homogeneous to be representative of the intricacies of real-world vulnerabilities. Essentially, the models trained on the synthetic datasets are learning trivial and shallow features that are not related to the core logic of the vulnerabilities.

\input{Tables/rq1-data-problem}

% Real-world vulnerabilities are characterized by distinct properties that may not be fully represented by the (semi-)synthetic data widely used by current approaches (see \tion{challenges}). This research question evaluates how well DL models trained on the synthetic data can predict vulnerabilities observed in the real-world. 
%To begin with, we ask the following question:

\noindent
\textbf{RQ1-A. How do DLVP methods trained on semi-synthetic vulnerabilities perform on real-world counterparts?}

% \smallskip

% \noindent\textbf{Approach.} 
We use the vulnerability prediction models from
three existing techniques: (a)~ VulDeePecker~\cite{li2018vuldeepecker}, (b)~SySeVR~\cite{li2018sysevr}, and (c)~Russell~\etal~\cite{russell2018automated} to predict for vulnerabilities in the two real-world datasets examples FFMPeg + Qemu~\cite{zhou2019devign} and \realdata. 

VulDeePecker and SySeVR offer vulnerability prediction models trained on a mixture of vulnerable examples from NVD and SARD datasets; Russell~\etal offers a vulnerability prediction model trained on GitHub+Debian data which are annotated with a static-analysis tool (see~\tab{existing_approach_design_choices}). We used these approaches since they train their models on datasets (NVD, SARD, and GitHub+Debian) containing source code examples and annotations obtained from the real world.

% \red{TO SECTION 3--- VulDeePecker and Russell~\etal have not made the implementation of the DL models publicly available, therefore, we re-implement their models closely following the respective articles. We have released our implementations in a replication package~\footnote{https://www.github.com/}. For SySeVR, they made their implementation publicly available, therefore we reuse those for this study. As for the training examples, in case of VulDeePecker and SySeVR, they released the ``code gadgets’’ used to train their models; we trained our implementation on those code gadgets. In the case of Russell~\etal’s model, we trained our implementation on the data provided by them. To validate the correctness of our implementation, we ensure that we achieve similar performance reported by the respective articles; the performance scores in the row labeled ``baseline'' in~\tab{rq1_real_world_prediction} matches the performance reported in those papers.}


% \smallskip
% \noindent \textbf{Observations.} 
Table~\ref{tab:rq1_real_world_prediction} shows the performance of existing techniques for detecting real world vulnerability. For comparison, we tabulate the baseline results reported in the respective papers in the rows labeled ``baseline''. For baselines, VulDeePecker and SySeVR use a combination of NVD and SARD datasets for training and testing; Russell~\etal use GitHub + Debian for training and testing. We observe the following:


\noindent \textbf{VulDeePecker}. VulDeePecker works by extracting so called ``code gadgets'' from API function calls. We follow the same code-gadget extraction technique from \devigndata and \realdata. We could extract code gadgets from only \textit{27.96\% of the available code} in \devigndata and from \textit{only 21.46\% of the available code} in \realdata. Vulnerabilities in the rest of the code in both the datasets cannot be discovered by VulDeePecker. This is problematic because it leaves a large number of the real-world code unusable. In terms of predictive performance on the usable code, we observe that VulDeePecker performs significantly worse on both the real-world datasets. In \realdata, VulDeePecker achieves an F1-score of \textit{only} $\mathit{12.08}\%$ and in \devigndata VulDeePecker achieves an F1-score $\mathit{14.33}\%$, while in the baseline case which used semi-synthetic data for testing, the F1-score of VulDeePecker was as high as $85.4\%$.

\noindent \textbf{SySeVR}.  SySeVR works by extracting so ``code gadgets'' from API function calls, Array Usage, Arithmetic Operations, and  Pointer Usage. Using their technique, we could extract code gadgets from \textit{84.08\% of the available code} in \devigndata and from \textit{only 66.42\% of the available code} in \realdata. While this is higher than VulDeePecker, vulnerabilities in the rest of the code in both the datasets cannot be can still not be discovered by SySeVR. In terms of predictive performance on the usable code from real-world data, we observed that SySeVR still  performed significantly worse on both \realdata and \devigndata datasets. In \realdata, SySeVR achieved an F1-score of \textit{only} $\mathit{10.27}\%$ and in \devigndata SySeVR achieved an F1-score $\mathit{16.85}\%$, this was significantly lower than the F1-score of $85.2\%$ that was reported on baseline case which used semi-synthetic data for testing.

\noindent \textbf{Russell~\etal} Unlike the previous two techniques, Russell~\etal does not use code gadgets. Instead, Russell~\etal. tokenize available code and create abstract representation of the tokens to build their models. Therefore, they are able to perform predictions on 100\% of the available real-world data from \devigndata and \realdata. Even so, when we use the DL models offered by Russell~\etal on the real-world data from \realdata and \devigndata, we observe a notable reduction in predictive performance of the model. In the case of \devigndata, DL model from Russell~\etal's method produced an F1-score of $46.77\%$ on \devigndata compared to the baseline of $56.6\%$. In \realdata, the F1-score was only $23.67\%$.


% Since, Russell~\etal classifies the whole function, whole 100\% of \devigndata~ and \realdata are in-scope for their model. For VulDeePecker and SySeVR, we report the conservative code level performances -- \ie, in case there are more than one code gadgets, if one of them are predicted as vulnerable, we declare that code vulnerable. Although this approach of reporting creates a possibility of generating higher number of false positives and lower number of false negatives, the results show that is not the case. Overall, both the false positives are false negatives are very high causing both low precision and low recall in both the datasets. 

We conjecture that the possible reason why Russell~\etal performs better than both VulDeePecker and SySeVR is due to the quality of the code used by each of the models to train their DLVP models. Both VulDeePecker and SySeVR are trained on NVD and SARD data. While NVD consists of real world production code, it only accounts for 7.85\%, 10.21\% of the total the training data in VulDeePecker and SySeVR respectively. Rest of the training examples belong to SARD dataset which is mostly synthetic and academic data. In contrast, all the code used for Russell~\etal's model come from open source repositories and the Debian distribution.

% \smallskip
% \begin{result}
% The datasets used in current DLVP literature \textit{are not suitable for DL based \vp in real world}. VulDeePecker and SySeVR cannot detect vulnerabilities in $\sim 78\%, 33\%$ of the real-world code in \realdata and $\sim72\%, 16\%$ of the code in \devigndata respectively. In terms of predictive performance, VulDeePecker achieves an F1-Score of $\sim12\%$ in \realdata and $\sim14\%$ in \devigndata; SySeVR achieves an F1-Score of $\sim11\%$ in \realdata and $\sim17\%$ in \devigndata. While Russell~\etal can detect vulnerabilities in all real-world code in \realdata and \devigndata, their data can achieve an F1-score of $\sim24\%$ in \realdata and $\sim46\%$ in \devigndata.
% \end{result}

% As we have seen the weakness of these datasets, we move only investigating what property of the datasets are causing these weaknesses. Now we ask,

% \noindent\textbf{RQ1-B. What causes the discrepancy in performance between semi-synthetic data and their real-world counterparts?}

% \noindent\textbf{Approach.}~To answer this question, we inspect the three datasets that were used to train the models in RQ1-A, \ie, VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr} and GitHub+Debian~\cite{russell2018automated}). To analyze the characteristics of the datasets, we investigate repetitiveness and the homogeneity of the data. Repetitiveness is introduced by the preprocessing technique used by the DLVP method; this informs us of how much of the the training and testing samples are exactly the same after the code has been preprocessed. Homogeneity informs us of the complexity of the vulnerable and non-vulnerable code patterns in the dataset. The more homogeneous vulnerable and non-vulnerable code patterns are, the easier they are to classify. To analyze the repetitiveness of the the data, we determine what fraction of the datasets have duplicate examples after preprocessing with the respective DLVP methods. To measure the homogeneity, we use Deckard~\cite{jiang2007deckard} to detect code clones in the data. We then cluster the functions in different datasets based on their similarity as given by Deckard. 

% As an aside, we note that VulDeePecker and SySeVR datasets were not originally intended to be used for vulnerability prediction task. These datasets were designed to elicit false negatives/false positives in static analyzers and also for human reference (in the form of CWEs). Therefore, they offer a simplified representation of the real vulnerability. Unlike these datasets, the GitHub + Debian dataset was collected by Russell~\etal~\cite{russell2018automated} from the real world projects on GitHub and some examples from the Debian distribution. However, the annotations for GitHub + Debian were made using a collection of static analyzers, therefore, it is difficult to know how many of these annotated vulnerabilities are False Positives. 

% \noindent\textbf{Observations.} We make the following observations:

% \noindent$\bullet$ \textit{Duplication:}~Table~\ref{tab:duplicate} shows the percentage of duplicate samples generated by different DLVP methods. For NVD and SARD datasets, the preprocessing technique from VulDeePecker results in $\mathbf{\sim75\%}$ duplicate examples (leaving only $\sim$25\% unique examples). $\mathbf{\sim50\%}$ of the examples are duplicated for NVD and SARD datasets when preprocessing technique from SySeVR is used. In Juliet and Github+Debian datasets, Russell~\etal.'s method produces $57\%$ and $2.98\%$ duplicate examples, respectively. 

% Ideally, a DL based model should be trained and tested on a dataset where 100\% of the examples are unique.  Duplication tends to artificially increase the overall performance of the method~\cite{allamanis2019adverse} (as reported in Baseline row of~\tab{rq1_real_world_prediction}).

% When these preprocessing techniques are applied to real-world data, the percentage of duplicates generated are significantly lower, as shown in~\tab{duplicate} for \devigndata and \realdata. This, consequently, results in significantly lower vulnerability prediction performance for real-world see in~\tab{rq1_real_world_prediction}.

% \noindent$\bullet$~The results in Figure~\ref{fig:clone-distro} shows the homogeneity plot for clusters of code in each of the datasets. The \blue{Blue} cluster represents when all the function in that cluster are non-vulnerable, \red{Red} when all are vulnerable. Other colors represent various percentage of vulnerable and non-vulnerables; \orange{Yellow} being the cluster where the there are almost equal number of vulnerable and non-vulnerable examples. The datasets are sorted based on their width of the Yellow cluster. As the figure shows, for Juliet~\cite{okun2013report}, VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and GitHub + Debian~\cite{russell2018automated} data, the width of the  yellow cluster are on the left part of the spectrum indicating that it is the presence of super simple patterns. These patterns are so easy that a clone detection tool can identify those. However, the two real world dataset that we experimented in this study are on the far right part of the spectrum indicating that the pattern that are exhibited by real world vulnerability are not super trivial to pick up. At the least, those patterns are more complex than that of other datasets that existing tools are evaluated on.

% % Figure~\ref{fig:lemna_sard} and Figure~\ref{fig:lemna_nvd} show examples of visualization using Lemna. Both has been predicted as vulnerable by the model, with one having ground truth as non-vulnerable and one having ground truth as vulnerable. The background color of each token indicates corresponding token's contribution in the prediction. For Figure~\ref{fig:lemna_ex1}, as shown in the picture the token sub-sequence contributing to the prediction of the code snippet is {\tt \textbf{() \{ wchar\_t *}}, which apparently has nothing to do with vulnerabilities. For Figure~\ref{fig:lemna_ex2}, although the prediction result is correct, the token sub-sequence that contributed the most is the {\tt \textbf{if (ss\_tc\_root != NULL)}} statement which is likely an artifact of the dataset similar to the example (Figure~\ref{fig:example}) we showed before. 

% \begin{table}[!tb]
%     \centering
%     \scriptsize
%     \caption{\small Percentage of duplicate samples in datasets. Draper data provide specific train, dev, and test split of the dataset. 94.93\% examples are unique to dev and test set from the corresponding train set. We found 97.02\% unique examples when we combine all the examples together.}
%     \begin{tabular}{c|c|c}
%         \hlineB{2}
%         \textbf{Dataset} &\textbf{Preprocessing Techniqu} & \textbf{\% of duplicates}\bigstrut\\
%         \hlineB{2}
%          Juliet & Russell~\etal & 68.63 \bigstrut\\
%          \hlineB{1}
%          \multirow{2}{*}{NVD + SARD} & VulDeePecker &  67.33 \bigstrut\\
%          & SySeVR &  61.991 \bigstrut\\
%          \hlineB{1}
%          Github+Debian & Russell~\etal & 6.07 / 2.99 \bigstrut\\
%          \hlineB{2}
%     \end{tabular}
%     \label{tab:duplicate}
% \end{table}

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.8\linewidth]{imgs/dist_clone.pdf}
%   \caption{\small{\textbf{Homogeneity of clone clusters for each dataset, red denotes cluster that is mostly constituted with vulnerable code, blue denotes cluster that is mostly constituted with non-vulnerable code.}}}
%   \label{fig:clone-distro}
% \end{figure}

% % From the homogeneity plot, we can notice that the baseline dataset, the SATE IV Juliet dataset~\cite{okun2013report}, and the VulDeePecker dataset~\cite{li2018vuldeepecker} have the two classes mixed in the clone clusters which might potentially help the generalizability of the model trained on them since it is not likely the model will pick up the clones as meaningful features, while SySeVR~\cite{li2018sysevr} and GitHub + Debian~\cite{russell2018automated} dataset have most of their clone clusters consisted of only one class code samples which could make the clones as features for the model to learn.

% \begin{result}
% Existing datasets are highly repetitive and exhibit much simple properties which can be identified by a code similarity/clone detection tool. Real world vulnerabilities exhibit much more complex patterns.
% \end{result} 

% \noindent\textbf{RQ1-C. What DLVP models trained on semi-synthetic data learn?}

\medskip
\noindent\textbf{RQ1-B. What do DLVP models trained on semi-synthetic data learn?}

To understand the difference between baseline performance of VulDeePecker, SySeVR, and Russell~\etal and their corresponding performance on real world performance, we inspect what features are learned by the different approaches. To do this, we use Lemna~\cite{guo2018lemna} which is popular explainability framework for deep learning models. Lemna~\cite{guo2018lemna} attempts to explain black-box (\ie, non-explainable) deep learning models by estimating the local decision boundary around a data point using a white-box (\ie, explainable) linear model. 

Specifically, given an example data point $(x_i,\;y_i),\;i\in \{1,\ldots,N\}$ where $x_i$ is the input and $y_i$ is the corresponding label, Lemna draws samples around $x_i$ to obtain $L$ synthetic input sequences $z_{i,j},\;j\in \{1,\ldots,L\}$ and its prediction labels $w_{i,j},\;j\in \{1,\ldots,L\}$. Lemna then learns a linear regression model from the original data point along with the sampled data points. Each of the token $x_i^t$ is assigned a value $\omega_i^t$ representing the contribution of that token for prediction. Higher value of $\omega_i^t$ would indicate larger contribution of token $x_i^t$ in predicting $y_i$~\footnote{For a detailed discussion, see~\cite{guo2018lemna}}. 


We use a heatmap to visualize the contribution of different tokens in an input code snippet for predicting the existence of vulnerability. 
\begin{figure}[!htb]
\input{Tables/lemna_example_1_integer_overflow}
\vspace{5mm}
\input{Tables/lemna_example_2_memory_overflow}
\vspace{5mm}
\input{Tables/lemna_example_3_draper_G_D}
\vspace{5mm}
\caption{\small \textbf{Code examples visualization with Lemna~\cite{guo2018lemna}. All of these code examples are predicted as vulnerable by respective models. \cref{fig:lemna_int_overflow} and \cref{fig:lemna_memory_overflow} are code slices from NVD+SARD dataset and SySeVR predicted those as vulnerable. \cref{fig:lemna_draper} is also predicted as vulnerable by Russel~\etal's CNN+RF~\cite{russell2018automated} model. \lone{Red} colored tokens contributed the most in respective predictions. \lfive{Green} colored tokens contributed the least.}}
\label{fig:lemna_examples}
\end{figure}
~\Cref{fig:lemna_examples} shows three examples of vulnerable code snippets.~\Cref{fig:lemna_int_overflow}, and~\Cref{fig:lemna_memory_overflow} are from NVD and SARD datasets and used by VulDeePecker~\cite{li2018vuldeepecker}, and SySeVR~\cite{li2018sysevr} to train their models repectively. Thus both of those code snippets show code slices extracted from the program.~\Cref{fig:lemna_draper} shows a function from Github + Debian~\cite{russell2018automated}, which Russel~\etal~\cite{russell2018automated} used to train their model. Note that, while we show the actual code tokens for analysis purpose, for training we used approach specific tokenization.

Each token in~\fig{lemna_examples} is highlighted with a color corresponding to the token's contribution to the prediction. Most important tokens are highlighted in \lone{red} and the least important tokens are colored \lfive{green}. We make the following observations:

\smallskip
\noindent\textbf{NVD + SARD dataset.}~\Cref{fig:lemna_int_overflow} and \Cref{fig:lemna_memory_overflow} show two code slices extracted by SySeVR from NVD and SARD datasets. Although these examples are predicted correctly by SySeVR, the most important token sequences used for the prediction are not related to the tokens pertaining to the actual vulnerability. % SySeVR correctly predicted as vulnerable code slices. 


~\Cref{fig:lemna_int_overflow} demonstrates an integer overflow vulnerability (CWE-190) where multiplying two integers (or a floating point variable) might result in an overflow. The actual vulnerability in this case lies in line 7, however \lone{\tt \textbf{void}} \lone{\tt CWE190\_Integer\_Overflow\_Unsigned\_int...()} contributes the most to SySeVR's Deep Learning model followed by \ltwo{\tt \textbf{unsigned int} data} and \ltwo{data = 0;}. 
% None of these token sequences are actually related to the vulnerability.

\Cref{fig:lemna_memory_overflow} shows a similar example for Uncontrolled Memory Vulnerability (CWE-789), where size of the memory allocated comes from a user input or the output of an API call. Without explicit sanitization, it can cause an uncontrolled memory allocation leading to a crash. Even though the main reason for the vulnerability in this example lies in lines 5, 9, and 10, however \lone{\tt \textbf{void} CWE789\_Uncontrolled\_Mem\_Alloc... ()} contributes the most in SySeVR's Prediction, followed by \ltwo{\tt \textbf{size\_t} data ;} and \ltwo{\tt data = 0;}.

\smallskip
\noindent\textbf{Github + Debian dataset.}~\Cref{fig:lemna_draper} shows an example from Github + Debian dataset. The plausible reason for this code to be vulnerable is the use of {\tt sprintf} function in line 6, 8, and 10. The length of {\tt buf} is not checked before writing to it through the {\tt sprintf} function. The CNN+RF model proposed by Russel~\etal~\cite{russell2018automated} picked up \lone{\tt \textbf{struct} port\_attribute} \lone{\tt *unused, \textbf{char} * buf)\{ \textbf{switch}} as the highest contributing token sequence. Similar to previous two examples, neither highest, nor the second highest contributing token sequences are related to the vulnerability.

We note that dataset used to train VulDeePecker and SySeVR\footnote{NVD + SARD dataset, mostly examples from SARD} were not originally intended to be used for vulnerability prediction task. These datasets were designed to elicit false negatives/false positives in static analyzers and also for human reference (in the form of CWEs). Therefore, they offer a simplified representation of the real vulnerability. Unlike these datasets, the GitHub + Debian dataset was collected by Russell~\etal~\cite{russell2018automated} from the real world projects on GitHub and some examples from the Debian distribution. However, the annotations for GitHub + Debian were made using a collection of static analyzers, therefore, it is difficult to know how noisy the dataset is \ie how many of these annotated vulnerabilities are False Positives. The simplicity and the noise in the datasets are forcing models to learn irrelevant features from the datasets. 
% 
% \begin{figure}[!tb]
% \begin{subfigure}{0.45\textwidth}
% \centering
%     \includegraphics[width=0.85\linewidth]{imgs/Lemna-viz-ex-1.pdf}
%     \vspace{-2mm}
%     \caption{\small{Example from SARD Dataset.}}
%     \label{fig:lemna_sard}
% \end{subfigure}

% \begin{subfigure}{0.45\textwidth}
%     \centering
%     \includegraphics[width=0.85\linewidth]{imgs/Lemna-viz-ex-2.pdf}
%     \caption{\small{Example from NVD dataset.}}
%     \label{fig:lemna_nvd}
% \end{subfigure}
% \caption{\small{Contribution of token subsequences in \vp from two examples in SARD and NVD datasets. Highest contribution to lowest contribution in the order of {\color{red} red}, {\color{orange} orange}, {\color{yellow} yellow}, {\color{green} green}.}}
% \label{fig:all_lemna_examples}
% \end{figure}
% 
% \Cref{fig:all_lemna_examples} shows two vulnerable examples from SARD~\cite{SARD}(\fig{lemna_sard}) and NVD~\cite{booth2013national} (\fig{lemna_nvd}). The each token is highlighted with a color corresponding to the token's contribution to the prediction. Most important tokens are highlighted in \colorbox{red!33}{red} and the least important tokens are colored \colorbox{green!33}{green}. %We make the following observations:

% In~\Cref{fig:lemna_sard}, code sub-sequence {\tt \colorbox{red!33}{() \{ wchar\_t *}} is indicated to be the most useful token, however it does not have any relationship with the vulnerability. %\blue{saikat: where is the vulnerability?}. 
% This example also illustrates the simplicity of the vulnerabilities in SARD dataset which was originally curated with synthetic examples for academic purposed to illustrate the vulnerability. Therefore, training a vulnerability prediction model on these examples may be sub-optimal.

% % Second, the original purpose of this dataset is to evaluate a \vp tool, not learn from this dataset, which is much difficult task than evaluation. 

% % \noindent $\bullet$~~
% Figure~\ref{fig:lemna_nvd} shows a vulnerable example from NDV dataset. Here the token sequence, {\tt \colorbox{red!33}{{if (ss\_tc\_root != NULL)}}} contributes the most in predicting that this code snippet was vulnerable. Although, this example look slightly more complex than that of SARD dataset, there is not apparent reason how this specific portion of the code is the reason for real vulnerability \blue{saikat: where is the real vulnerability in this example. The NVD dataset does not annotate line level vulnerability, nor it localizes the vulnerability to a specific point. Thus, we don't know about the exact location of the vulnerability in this case.}. 


% As an aside, we note that VulDeePecker and SySeVR datasets were not originally intended to be used for vulnerability prediction task. These datasets were designed to elicit false negatives/false positives in static analyzers and also for human reference (in the form of CWEs). Therefore, they offer a simplified representation of the real vulnerability. Unlike these datasets, the GitHub + Debian dataset was collected by Russell~\etal~\cite{russell2018automated} from the real world projects on GitHub and some examples from the Debian distribution. However, the annotations for GitHub + Debian were made using a collection of static analyzers, therefore, it is difficult to know how many of these annotated vulnerabilities are False Positives. 

% We not that this token sub-sequence is an artifact of NVD dataset. 

% Finally, we summarize the lessons learned through the investigation and experiment in this section as, 

% \smallskip
% \noindent\textbf{Lesson 1:}~The existing dataset do not represent real world vulnerabilities very well. Result show that when we deploy such models in real world, those incur a lot of false positives and false negatives posing a threat to the applicability of those techniques in real world. To predict vulnerabilities in real world, we have to train a model with real world datasets.


\noindent\textbf{RQ1-C. What causes the discrepancy in performance between (semi-)synthetic data and their real-world counterparts?}

% \noindent\textbf{Approach.}~
To further understand \tab{rq1_real_world_prediction} and \Cref{fig:lemna_examples}, we inspect the (semi-)synthetic datasets that were used in this paper, \ie, VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr} and GitHub+Debian~\cite{russell2018automated}). To analyze the characteristics of those datasets, we investigate repetitiveness and the homogeneity of the data. Repetitiveness is introduced by the preprocessing technique used by the DLVP method; this informs us of how much of the training and testing samples are exactly the same after the code has been preprocessed. Homogeneity informs us of the complexity of the vulnerable and non-vulnerable code patterns in the dataset. The more homogeneous vulnerable and non-vulnerable code patterns are, the easier they are to classify. To analyze the repetitiveness of the the data, we determine what fraction of the datasets have duplicate examples after preprocessing with the respective DLVP methods. To measure the homogeneity, we use Deckard~\cite{jiang2007deckard} to detect code clones in the data. We then cluster the functions in different datasets based on their similarity as given by Deckard. 
% \noindent\textbf{Observations.} 
We make the following observations:

\noindent$\bullet$ \textit{Duplication:}~Table~\ref{tab:duplicate} shows the percentage of duplicate samples generated by different DLVP methods. For NVD and SARD datasets, the preprocessing technique from VulDeePecker results in $\mathbf{\sim75\%}$ duplicate examples (leaving only $\sim$25\% unique examples). $\mathbf{\sim50\%}$ of the examples are duplicated for NVD and SARD datasets when preprocessing technique from SySeVR is used. In Juliet and Github+Debian datasets, Russell~\etal.'s method produces $57\%$ and $2.98\%$ duplicate examples, respectively. 

Ideally, a DL based model should be trained and tested on a dataset where 100\% of the examples are unique.  Duplication tends to artificially increase the overall performance of the method~\cite{allamanis2019adverse} (as reported in Baseline row of~\tab{rq1_real_world_prediction}).

% When these preprocessing techniques are applied to real-world data, the percentage of duplicates generated are significantly lower, as shown in~\tab{duplicate} for \devigndata and \realdata. This, consequently, results in significantly lower vulnerability prediction performance for real-world see in~\tab{rq1_real_world_prediction}.

\noindent$\bullet$~ \textit{Homogeneity.}~The results in Figure~\ref{fig:clone-distro} shows the homogeneity plot for clusters of code clones in each of the datasets. The \blue{Blue} cluster represents when all the samples in that cluster are non-vulnerable, \red{Red} when all samples are vulnerable. Other colors represent various percentages of vulnerable and non-vulnerable samples; \orange{Yellow} being the cluster where the there are almost equal number of vulnerable and non-vulnerable examples. The datasets are sorted based on their width of the Yellow cluster. As the figure shows, for Juliet~\cite{okun2013report}, VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and GitHub + Debian~\cite{russell2018automated} data, the width of the  yellow cluster are on the left part of the spectrum indicating that it is the presence of super simple patterns. These patterns are so easy that a clone detection tool can identify those. However, the two real world dataset that we experimented in this study are on the far right part of the spectrum indicating that the pattern that are exhibited by real world vulnerability are not super trivial to pick up. At the least, those patterns are more complex than that of other datasets that existing tools are evaluated on.

% Figure~\ref{fig:lemna_sard} and Figure~\ref{fig:lemna_nvd} show examples of visualization using Lemna. Both has been predicted as vulnerable by the model, with one having ground truth as non-vulnerable and one having ground truth as vulnerable. The background color of each token indicates corresponding token's contribution in the prediction. For Figure~\ref{fig:lemna_ex1}, as shown in the picture the token sub-sequence contributing to the prediction of the code snippet is {\tt \textbf{() \{ wchar\_t *}}, which apparently has nothing to do with vulnerabilities. For Figure~\ref{fig:lemna_ex2}, although the prediction result is correct, the token sub-sequence that contributed the most is the {\tt \textbf{if (ss\_tc\_root != NULL)}} statement which is likely an artifact of the dataset similar to the example (Figure~\ref{fig:example}) we showed before. 

\begin{table}[!tb]
    \centering
    \footnotesize
    \caption{\small Percentage of duplicate samples in datasets. Draper data provide specific train, dev, and test split of the dataset. 94.93\% examples are unique to dev and test set from the corresponding train set. We found 97.02\% unique examples when we combine all the examples together.}
    \begin{tabular}{c|c|c}
        \hlineB{2}
        \textbf{Dataset} &\textbf{Preprocessing Technique} & \textbf{\% of duplicates}\bigstrut\\
        \hlineB{2}
         Juliet & Russell~\etal & 68.63 \bigstrut\\
         \hlineB{1}
         \multirow{2}{*}{NVD + SARD} & VulDeePecker &  67.33 \bigstrut\\
         & SySeVR &  61.991 \bigstrut\\
         \hlineB{1}
         Github+Debian & Russell~\etal & 6.07 / 2.99 \bigstrut\\
         \hlineB{2}
    \end{tabular}
    \label{tab:duplicate}
\end{table}

\begin{figure}[!htb]
    \centering
  \includegraphics[width=0.8\linewidth]{imgs/dist_clone.pdf}
  \caption{\small{\textbf{Homogeneity of clone clusters for each dataset, red denotes cluster that is mostly constituted with vulnerable code, blue denotes cluster that is mostly constituted with non-vulnerable code.}}}
  \label{fig:clone-distro}
\end{figure}

% From the homogeneity plot, we can notice that the baseline dataset, the SATE IV Juliet dataset~\cite{okun2013report}, and the VulDeePecker dataset~\cite{li2018vuldeepecker} have the two classes mixed in the clone clusters which might potentially help the generalizability of the model trained on them since it is not likely the model will pick up the clones as meaningful features, while SySeVR~\cite{li2018sysevr} and GitHub + Debian~\cite{russell2018automated} dataset have most of their clone clusters consisted of only one class code samples which could make the clones as features for the model to learn.

% \begin{result}
% \end{result} 


% \smallskip
% \noindent\textbf{}

% For Figure~\ref{fig:lemna_ex2}, although the prediction result is correct, the token sub-sequence that contributed the most is the {\tt \textbf{if (ss\_tc\_root != NULL)}} statement which is likely an artifact of the dataset similar to the example (Figure~\ref{fig:example}) we showed before. 
% We answer this question from two different real world scenario. Our first scenario is when developers might not have sufficient annotated training data. In this case, they might want to use knowledge from other projects --\ie they would want to use the pre-trained model from other dataset. To investigate further, we chose four different Deep Learning models -- CNN, CNN+RF, BGRU, BLSTM. These models are proposed by previous approaches~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated} and four different datasets -- \ie Juliet~\cite{okun2013report}, VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and GitHub and Debian~\cite{russell2018automated}. These datasets are used to evaluate respective approaches. For predicting vulnerabilities from one dataset, we measure the performance of pre-trained models from other dataset. In this scenario, we are simulating a case, where for each test dataset, there is not enough annotated examples to train on. The dataset under test works as a proxy of real world vulnerabilities. Note that this paper's purpose is not to compare the performance of different deep learning architectures using the same dataset; such comparisons have already been shown in different researches~\cite{russell2018automated, li2018vuldeepecker, li2018sysevr}. Instead, we intend to explore how representative the datasets are across different DL models, where we pick a model that is reported to be the best-performing one \wrt a given dataset. We also designed an ensemble method 
% where we consult all the pre-trained models from existing datasets to predict vulnerabilities from a particular dataset.  

% \noindent Our second scenario is when there are annotated real world datasets are available. In this case, we tested the performance of aforementioned four models on two dataset. Our first dataset is real world vulnerabilities from Qemu and FFMpeg projects proposed by Zhou~\etal~\cite{zhou2019devign}. Our second dataset is real world vulnerabilities from Chromium and Debian project. 


% \smallskip
% \noindent
% \textbf{Results:}
% Table \ref{tab:cross} shows the experiment results on our first scenario. In this case, pre-trained models from all four approaches \ie  CNN+RF(\ref{tab:cross_cnnrf}), CNN(\ref{tab:cross_cnn}), BLSTM(\ref{tab:cross_blstm}), and BGRU(\ref{tab:cross_bgru}) are not very effective to predict vulnerabilities in the wild. Even though they all exhibit very high performance while tested on intra-dataset. 

% % \input{Tables/cross-dataset.tex}

% From the result, it is evident that the models trained on these datasets are not likely to generalize well on unseen data and real-world applications, given that they do not generalize well among themselves.
% For example, see the first row: when CNN+RF Model is trained and tested on Juliet dataset, it achieved 87\% accuracy. However, when tested with other datasets, the mean accuracy is dropped to 38\%.  The same observation is valid for F1 scores. Thus, it is clear that the such pre-trained model are not suitable for real-world applications, given that they do not generalize well among themselves. Table~\ref{tab:cross_ensemble} shows the performance when we ensemble the all the  pre-trained models. The results clearly show that, even if we try to leverage all the pre-trained models, it fails to effectively detect vulnerabilities. 

% \input{Tables/token_real_world}

% \noindent Table~\ref{tab:token_real_world} shows the performance of existing approaches on two different real world dataset. In both of those dataset vulnerability annotated examples are available to train DL based models. The results show that existing approaches fail to detect real world vulnerability even when there are annotated vulnerability data to train on. All four of the existing approach exhibit very poor performance in detecting those vulnerabilities.

% \input{Tables/slice_real_world}
% To understand the effect of slicing as championed by VulDeePecker and SySeVR, we extracted slices from functions in Devign dataset and \realdata. To have a fair comparison, if at least one of the slice extracted from a function is predicted by the models as vulnerable, we predict that function as vulnerable. Table~\ref{tab:slice_real_world} shows a comparison of two different slicing mechanisms and corresponding result. In slice granularity, CNN+RF model shows very poor performance. In function granularity, although the result is bit more promising, not all the code samples are considered to be prediction by a respective model. For instance, in \realdata, model trained on slices extracted from array indexing, the F1 is 25.55, but only 30.70\% (\%f column in the table) of the total function had at least one slice from array indexing statement and hence considered for prediction. This makes the model ineffective in predicting the rest 69.30\% functions.


% \noindent \textbf{Observation:} Existing pre-trained models fail to effectively detect vulnerabilities in the wild. Even when trained on real world vulnerabilities, those models do not generalize well. 

% \noindent
% \begin{table}[!htb]
%     \centering
%     \footnotesize
%     \vspace{-5mm}
%     \caption{\textbf{\small Test performance of existing dataset in ensemble settings.}}
%     \vspace{-3mm}
%     \begin{tabular}{c|c|c}
%     \toprule
%         Dataset under test & Accuracy & F1 \\
%         \midrule
%         Juliet & 54.5 & 41.08\\
%         \midrule
%         VulDeePecker & 52.83 & 44.08\\
%         \midrule
%         SySeVR & 46.5 & 26.58\\
%         \midrule
%         GitHub + Debian & 50.08 & 12.33\\
%         \bottomrule
%     \end{tabular}
%     \vspace{-3mm}
%     \label{tab:ensemble}
% \end{table}

% Since there are a lot of datasets available, one could ask what if, we learn from all the available datasets and models. To investigate this aspect, we designed an ensemble of different models and different datasets.  In this experiment, when we are predicting vulnerability from  a particular dataset, we consult the models developed from other datasets.  
 




==> RQ_details/rq1_backup.tex <==
% !TEX root = ../fse_results.tex

\subsection{RQ1}
\label{sec:rq1}

\noindent\textbf{RQ1: How well do state-of-the-art vulnerability prediction models work in a real-world situations?}

\noindent
A vulnerability prediction approach is useful when it can successfully predict real world vulnerabilities. Different Deep Learning(DL) based vulnerability prediction approaches are proposed and showed to have very good performance. A limited evaluation on prediction of real world vulnerabilities poses a threat to the applicability of those approaches in predicting security vulnerabilities. In this research question, we shed light on applying those proposed techniques real world development scenario. 

\noindent
\textbf{Experimental Setup:}
We answer this question from two different real world scenario. Our first scenario is when developers might not have sufficient annotated training data. In this case, they might want to use knowledge from other projects --\ie they would want to use the pre-trained model from other dataset. To investigate further, we chose four different Deep Learning models -- CNN, CNN+RF, BGRU, BLSTM. These models are proposed by previous approaches~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated} and four different datasets -- \ie Juliet~\cite{okun2013report}, VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and Github and Debian~\cite{russell2018automated}. These datasets are used to evaluate respective approaches. For predicting vulnerabilities from one dataset, we measure the performance of pre-trained models from other dataset. In this scenario, we are simulating a case, where for each test dataset, there is not enough annotated examples to train on. The dataset under test works as a proxy of real world vulnerabilities. Note that this paper's purpose is not to compare the performance of different deep learning architectures using the same dataset; such comparisons have already been shown in different researches~\cite{russell2018automated, li2018vuldeepecker, li2018sysevr}. Instead, we intend to explore how representative the datasets are across different DL models, where we pick a model that is reported to be the best-performing one \wrt a given dataset. We also designed an ensemble method 
where we consult all the pre-trained models from existing datasets to predict vulnerabilities from a particular dataset.  

\noindent Our second scenario is when there are annotated real world datasets are available. In this case, we tested the performance of aforementioned four models on two dataset. Our first dataset is real world vulnerabilities from Qemu and FFMpeg projects proposed by Zhou~\etal~\cite{zhou2019devign}. Our second dataset is real world vulnerabilities from Chromium and Debian project. 


\smallskip
\noindent
\textbf{Results:}
Table \ref{tab:cross} shows the experiment results on our first scenario. In this case, pre-trained models from all four approaches \ie  CNN+RF(\ref{tab:cross_cnnrf}), CNN(\ref{tab:cross_cnn}), BLSTM(\ref{tab:cross_blstm}), and BGRU(\ref{tab:cross_bgru}) are not very effective to predict vulnerabilities in the wild. Even though they all exhibit very high performance while tested on intra-dataset. 

\input{Tables/cross-dataset.tex}

From the result, it is evident that the models trained on these datasets are not likely to generalize well on unseen data and real-world applications, given that they do not generalize well among themselves.
For example, see the first row: when CNN+RF Model is trained and tested on Juliet dataset, it achieved 87\% accuracy. However, when tested with other datasets, the mean accuracy is dropped to 38\%.  The same observation is valid for F1 scores. Thus, it is clear that the such pre-trained model are not suitable for real-world applications, given that they do not generalize well among themselves. Table~\ref{tab:cross_ensemble} shows the performance when we ensemble the all the  pre-trained models. The results clearly show that, even if we try to leverage all the pre-trained models, it fails to effectively detect vulnerabilities. 

\input{Tables/token_real_world}

\noindent Table~\ref{tab:token_real_world} shows the performance of existing approaches on two different real world dataset. In both of those dataset vulnerability annotated examples are available to train DL based models. The results show that existing approaches fail to detect real world vulnerability even when there are annotated vulnerability data to train on. All four of the existing approach exhibit very poor performance in detecting those vulnerabilities.

\input{Tables/slice_real_world}
To understand the effect of slicing as championed by VulDeePecker and SySeVR, we extracted slices from functions in Devign dataset and \realdata. To have a fair comparison, if at least one of the slice extracted from a function is predicted by the models as vulnerable, we predict that function as vulnerable. Table~\ref{tab:slice_real_world} shows a comparison of two different slicing mechanisms and corresponding result. In slice granularity, CNN+RF model shows very poor performance. In function granularity, although the result is bit more promising, not all the code samples are considered to be prediction by a respective model. For instance, in \realdata, model trained on slices extracted from array indexing, the F1 is 25.55, but only 30.70\% (\%f column in the table) of the total function had at least one slice from array indexing statement and hence considered for prediction. This makes the model ineffective in predicting the rest 69.30\% functions.


\noindent \textbf{Observation:} Existing pre-trained models fail to effectively detect vulnerabilities in the wild. Even when trained on real world vulnerabilities, those models do not generalize well. 

% \noindent
% \begin{table}[!htb]
%     \centering
%     \footnotesize
%     \vspace{-5mm}
%     \caption{\textbf{\small Test performance of existing dataset in ensemble settings.}}
%     \vspace{-3mm}
%     \begin{tabular}{c|c|c}
%     \toprule
%         Dataset under test & Accuracy & F1 \\
%         \midrule
%         Juliet & 54.5 & 41.08\\
%         \midrule
%         VulDeePecker & 52.83 & 44.08\\
%         \midrule
%         SySeVR & 46.5 & 26.58\\
%         \midrule
%         Github + Debian & 50.08 & 12.33\\
%         \bottomrule
%     \end{tabular}
%     \vspace{-3mm}
%     \label{tab:ensemble}
% \end{table}

% Since there are a lot of datasets available, one could ask what if, we learn from all the available datasets and models. To investigate this aspect, we designed an ensemble of different models and different datasets.  In this experiment, when we are predicting vulnerability from  a particular dataset, we consult the models developed from other datasets.  
 




==> RQ_details/rq1_backup1.tex <==
% !TEX root = ../fse_results.tex

\subsection{Representativeness of Synthetic Data (RQ1)}
\label{sect:rq1}

% A vulnerability prediction approach is useful when it can successfully predict real world vulnerabilities. Different Deep Learning(DL) based vulnerability prediction approaches are proposed and showed to have very good performance. 

% A limited evaluation on prediction of real world vulnerabilities poses a threat to the applicability of those approaches in predicting security vulnerabilities. In this research question, we shed light on applying those proposed techniques real world development scenario. 

Real-world vulnerabilities are characterized by distinct properties that may not be fully represented by the (semi-)synthetic data widely used by current approaches (see \tion{challenges}). This research question evaluates how well DL models trained on the synthetic data can predict vulnerabilities observed in the real-world. To begin with, we ask the following question:

\noindent
\textbf{RQ1-A. How do DLVP methods trained on semi-synthetic vulnerabilities perform on real-world counterparts?}

\smallskip

\noindent\textbf{Approach.} We use the vulnerability prediction models from
three existing techniques: (a)~ VulDeePecker~\cite{li2018vuldeepecker}, (b)~SySeVR~\cite{li2018sysevr}, and (c)~Russel~\etal~\cite{russell2018automated} to predict for vulnerabilities in the two real-world datasets examples FFMPeg + Qemu~\cite{zhou2019devign} and \realdata. 

VulDeePecker and SySeVR offer vulnerability prediction models trained on a mixture of vulnerable examples from NVD and SARD datasets; Russel~\etal offers a vulnerability prediction model trained on GitHub+Debian data which are annotated with a static-analysis tool (see~\tab{existing_approach_design_choices}). We used these approaches since they train their models on datasets (NVD, SARD, and GitHub+Debian) containing source code examples and annotations obtained from the real world.

VulDeePecker and Russel~\etal have not made the implementation of the DL models publicly available, therefore, we re-implement their models closely following the respective articles. We have released our implementations in a replication package~\footnote{\url{https://www.GitHub.com/}}. For SySeVR, they made their implementation publicly available, therefore we reuse those for this study. As for the training examples, in case of VulDeePecker and SySeVR, they released the ``code gadgets’’ used to train their models; we trained our implementation on those code gadgets. In the case of Russel~\etal’s model, we trained our implementation on the data provided by them. To validate the correctness of our implementation, we ensure that we achieve similar performance reported by the respective articles; the performance scores in the row labeled ``baseline'' in~\tab{rq1_real_world_prediction} matches the performance reported in those papers.

\input{Tables/rq1-data-problem}

\smallskip
\noindent \textbf{Observations.} Table~\ref{tab:rq1_real_world_prediction} shows the performance of existing techniques for detecting real world vulnerability. For comparison, we tabulate the baseline results reported in the respective papers in the rows labeled ``baseline''. For baselines, VulDeePecker and SySeVR use a combination of NVD and SARD datasets for training and testing; Russel~\etal use GitHub + Debian for training and testing. We observe the following:
\bi
\item \textit{VulDeePecker}: VulDeePecker works by extracting so called ``code gadgets'' from API function calls. We follow the same code-gadget extraction technique from \devigndata and \realdata. We could extract code gadgets from only \textit{27.96\% of the available code} in \devigndata and from \textit{only 21.46\% of the available code} in \realdata. Vulnerabilities in the rest of the code in both the datasets cannot be discovered by VulDeePecker. This is problematic because it leaves a large number of the real-world code unusable. In terms of predictive performance on the usable code, we observe that VulDeePecker performs significantly worse on both the real-world datasets. In \realdata, VulDeePecker achieves an F1-score of \textit{only} $\mathit{12.08}\%$ and in \devigndata VulDeePecker achieves an F1-score $\mathit{14.33}\%$, while in the baseline case which used semi-synthetic data for testing, the F1-score of VulDeePecker was as high as $85.4\%$.

\item \textit{SySeVR}:  SySeVR works by extracting so ``code gadgets'' from API function calls, Array Usage, Arithmetic Operations, and  Pointer Usage. Using their technique, we could extract code gadgets from \textit{84.08\% of the available code} in \devigndata and from \textit{only 66.42\% of the available code} in \realdata. While this is higher than VulDeePecker, vulnerabilities in the rest of the code in both the datasets cannot be can still not be discovered by SySeVR. In terms of predictive performance on the usable code from real-world data, we observed that SySeVR still  performed significantly worse on both \realdata and \devigndata datasets. In \realdata, SySeVR achieved an F1-score of \textit{only} $\mathit{10.27}\%$ and in \devigndata SySeVR achieved an F1-score $\mathit{16.85}\%$, this was significantly lower than the F1-score of $85.2\%$ that was reported on baseline case which used semi-synthetic data for testing.

\item \textit{Russel~\etal}: Unlike the previous two techniques, Russel~\etal does not use code gadgets. Instead, Russel~\etal. tokenize available code and create abstract representation of the tokens to build their models. Therefore, they are able to perform predictions on 100\% of the available real-world data from \devigndata and \realdata. Even so, when we use the DL models offered by Russel~\etal on the real-world data from \realdata and \devigndata, we observe a notable reduction in predictive performance of the model. In the case of \devigndata, DL model from Russel~\etal's method produced an F1-score of $46.77\%$ on \devigndata compared to the baseline of $56.6\%$. In \realdata, the F1-score was much lower (only $23.67\%$).
\ei

% Since, Russel~\etal classifies the whole function, whole 100\% of \devigndata~ and \realdata are in-scope for their model. For VulDeePecker and SySeVR, we report the conservative code level performances -- \ie, in case there are more than one code gadgets, if one of them are predicted as vulnerable, we declare that code vulnerable. Although this approach of reporting creates a possibility of generating higher number of false positives and lower number of false negatives, the results show that is not the case. Overall, both the false positives are false negatives are very high causing both low precision and low recall in both the datasets. 

We conjecture that the possible reason why Russel~\etal performs better than both VulDeePecker and SySeVR is due to the quality of the code used by each of the models to train their DLVP models. Both VulDeePecker and SySeVR are trained on NVD and SARD data. While NVD consists of real world production code, it only accounts for 7.85\%, 10.21\% of the total the training data in VulDeePecker and SySeVR respectively. Rest of the training examples belong to SARD dataset which is mostly synthetic and academic data. In contrast, all the code used for Russel~\etal's model come from open source repositories and the Debian distribution.

\smallskip
\begin{result}
The datasets used in current DLVP literature \textit{are not suitable for DL based \vp in real world}. VulDeePecker and SySeVR cannot detect vulnerabilities in $\sim 78\%, 33\%$ of the real-world code in \realdata and $\sim72\%, 16\%$ of the code in \devigndata respectively. In terms of predictive performance, VulDeePecker achieves an F1-Score of $\sim12\%$ in \realdata and $\sim14\%$ in \devigndata; SySeVR achieves an F1-Score of $\sim11\%$ in \realdata and $\sim17\%$ in \devigndata. While Russel~\etal can detect vulnerabilities in all real-world code in \realdata and \devigndata, their data can achieve an F1-score of $\sim24\%$ in \realdata and $\sim46\%$ in \devigndata.
\end{result}

% As we have seen the weakness of these datasets, we move only investigating what property of the datasets are causing these weaknesses. Now we ask,

\noindent\textbf{RQ1-B. What causes the discrepancy in performance between semi-synthetic data and their real-world counterparts?}

\noindent\textbf{Approach.}~To answer this question, we inspect the three datasets that were used to train the models in RQ1-A, \ie, VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr} and GitHub+Debian~\cite{russell2018automated}). To analyze the characteristics of the datasets, we investigate repetitiveness and the homogeneity of the data. Repetitiveness is introduced by the preprocessing technique used by the DLVP method; this informs us of how much of the the training and testing samples are exactly the same after the code has been preprocessed. Homogeneity informs us of the complexity of the vulnerable and non-vulnerable code patterns in the dataset. The more homogeneous vulnerable and non-vulnerable code patterns are, the easier they are to classify. To analyze the repetitiveness of the the data, we determine what fraction of the datasets have duplicate examples after preprocessing with the respective DLVP methods. To measure the homogeneity, we use Deckard~\cite{jiang2007deckard} to detect code clones in the data. We then cluster the functions in different datasets based on their similarity as given by Deckard. 

As an aside, we note that VulDeePecker and SySeVR datasets were not originally intended to be used for vulnerability prediction task. These datasets were designed to elicit false negatives/false positives in static analyzers and also for human reference (in the form of CWEs). Therefore, they offer a simplified representation of the real vulnerability. Unlike these datasets, the GitHub + Debian dataset was collected by Russel~\etal~\cite{russell2018automated} from the real world projects on GitHub and some examples from the Debian distribution. However, the annotations for GitHub + Debian were made using a collection of static analyzers, therefore, it is difficult to know how many of these annotated vulnerabilities are False Positives. 

\noindent\textbf{Observations.} We make the following observations:

\noindent$\bullet$ \textit{Duplication:}~Table~\ref{tab:duplicate} shows the percentage of duplicate samples generated by different DLVP methods. For NVD and SARD datasets, the preprocessing technique from VulDeePecker results in $\mathbf{\sim75\%}$ duplicate examples (leaving only $\sim$25\% unique examples). $\mathbf{\sim50\%}$ of the examples are duplicated for NVD and SARD datasets when preprocessing technique from SySeVR is used. In Juliet and Github+Debian datasets, Russel~\etal.'s method produces $57\%$ and $2.98\%$ duplicate examples, respectively. 

Ideally, a DL based model should be trained and tested on a dataset where 100\% of the examples are unique.  Duplication tends to artificially increase the overall performance of the method~\cite{allamanis2019adverse} (as reported in Baseline row of~\tab{rq1_real_world_prediction}).

When these preprocessing techniques are applied to real-world data, the percentage of duplicates generated are significantly lower, as shown in~\tab{duplicate} for \devigndata and \realdata. This, consequently, results in significantly lower vulnerability prediction performance for real-world see in~\tab{rq1_real_world_prediction}.

\noindent$\bullet$~The results in Figure~\ref{fig:clone-distro} shows the homogeneity plot for clusters of code in each of the datasets. The \blue{Blue} cluster represents when all the function in that cluster are non-vulnerable, \red{Red} when all are vulnerable. Other colors represent various percentage of vulnerable and non-vulnerables; \orange{Yellow} being the cluster where the there are almost equal number of vulnerable and non-vulnerable examples. The datasets are sorted based on their width of the Yellow cluster. As the figure shows, for Juliet~\cite{okun2013report}, VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and GitHub + Debian~\cite{russell2018automated} data, the width of the  yellow cluster are on the left part of the spectrum indicating that it is the presence of super simple patterns. These patterns are so easy that a clone detection tool can identify those. However, the two real world dataset that we experimented in this study are on the far right part of the spectrum indicating that the pattern that are exhibited by real world vulnerability are not super trivial to pick up. At the least, those patterns are more complex than that of other datasets that existing tools are evaluated on.

% Figure~\ref{fig:lemna_sard} and Figure~\ref{fig:lemna_nvd} show examples of visualization using LEMNA. Both has been predicted as vulnerable by the model, with one having ground truth as non-vulnerable and one having ground truth as vulnerable. The background color of each token indicates corresponding token's contribution in the prediction. For Figure~\ref{fig:lemna_ex1}, as shown in the picture the token sub-sequence contributing to the prediction of the code snippet is {\tt \textbf{() \{ wchar\_t *}}, which apparently has nothing to do with vulnerabilities. For Figure~\ref{fig:lemna_ex2}, although the prediction result is correct, the token sub-sequence that contributed the most is the {\tt \textbf{if (ss\_tc\_root != NULL)}} statement which is likely an artifact of the dataset similar to the example (Figure~\ref{fig:example}) we showed before. 

\begin{table}[!tb]
    \centering
    \scriptsize
    \caption{\small Percentage of duplicate samples in datasets. Draper data provide specific train, dev, and test split of the dataset. 94.93\% examples are unique to dev and test set from the corresponding train set. We found 97.02\% unique examples when we combine all the examples together.}
    \begin{tabular}{c|c|c}
        \hlineB{2}
        \textbf{Dataset} &\textbf{Preprocessing Techniqu} & \textbf{\% of duplicates}\bigstrut\\
        \hlineB{2}
         Juliet & Russel~\etal & 68.63 \bigstrut\\
         \hlineB{1}
         \multirow{2}{*}{NVD + SARD} & VulDeePecker &  67.33 \bigstrut\\
         & SySeVR &  61.991 \bigstrut\\
         \hlineB{1}
         Github+Debian & Russel~\etal & 6.07 / 2.99 \bigstrut\\
         \hlineB{2}
    \end{tabular}
    \label{tab:duplicate}
\end{table}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.8\linewidth]{imgs/dist_clone.pdf}
  \caption{\small{\textbf{Homogeneity of clone clusters for each dataset, red denotes cluster that is mostly constituted with vulnerable code, blue denotes cluster that is mostly constituted with non-vulnerable code.}}}
  \label{fig:clone-distro}
\end{figure}

% From the homogeneity plot, we can notice that the baseline dataset, the SATE IV Juliet dataset~\cite{okun2013report}, and the VulDeePecker dataset~\cite{li2018vuldeepecker} have the two classes mixed in the clone clusters which might potentially help the generalizability of the model trained on them since it is not likely the model will pick up the clones as meaningful features, while SySeVR~\cite{li2018sysevr} and GitHub + Debian~\cite{russell2018automated} dataset have most of their clone clusters consisted of only one class code samples which could make the clones as features for the model to learn.

\begin{result}
Existing datasets are highly repetitive and exhibit much simple properties which can be identified by a code similarity/clone detection tool. Real world vulnerabilities exhibit much more complex patterns.
\end{result} 

\noindent\textbf{RQ1-C. What DLVP models trained on semi-synthetic data learn?}

\smallskip

Given, we found a big difference between reported performance (intra-dataset evaluation) and real world performance, we do a case study to understand what are the features that are learned by different approaches. Explaining DL based models is hard. In some case it is very hard to the point that it is impossible to fully explain a model~\cite{samek2019explainable}. There are some methods to partially explain a model, and/or explain a dataset by building a parallel model which often are guided by original models~\cite{guo2018lemna, frosst2017distilling}. 

Lemna~\cite{guo2018lemna} is such a tool to explain black-box (\ie, non-explainable) deep learning models by estimating the local decision boundary around a data point using a white-box (\ie, explainable) linear model. Given an example data point $(x_i,\;y_i),\;i\in \{1,\ldots,N\}$ where $x_i$ is the input sequence and $y_i$ is the label, LEMNA~\cite{guo2018lemna} samples around $x_i$ to obtain $L$ synthetic input sequences $z_{i,j},\;j\in \{1,\ldots,L\}$ and its prediction labels $w_{i,j},\;j\in \{1,\ldots,L\}$. Lemna learns a linear regression model from the original data point along with the sampled data points. Each of the token $x_i^t$ is assigned a \emph{heatmap} $\omega_i^t$ representing the contribution of that token for prediction. Higher value of $\omega_i^t$ would indicate larger contribution of token $x_i^t$ in predicting $y_i$. Details can be found in the paper~\cite{guo2018lemna}. We adopted this visualization technique to investigate contribution on different token sub-sequences of a input code snippet on the output vulnerability label. 

\begin{figure}[!htb]
\begin{subfigure}{0.45\textwidth}
\centering
    \includegraphics[width=0.85\linewidth]{imgs/lemna-viz-ex-1.pdf}
    \vspace{-2mm}
    \caption{\small{Example from SARD Dataset.}}
    \label{fig:lemna_sard}
\end{subfigure}

\begin{subfigure}{0.45\textwidth}
    \centering
    \includegraphics[width=0.85\linewidth]{imgs/lemna-viz-ex-2.pdf}
    \caption{\small{Example from NVD dataset.}}
    \label{fig:lemna_nvd}
\end{subfigure}
\caption{\small{Contribution of token subsequences in \vp from two examples in SARD and NVD datasets. Highest contribution to lowest contribution in the order of {\color{red} red}, {\color{orange} orange}, {\color{yellow} yellow}, {\color{green} green}.}}
\label{fig:all_lemna_examples}
\end{figure}

Figure~\ref{fig:all_lemna_examples} shows two random examples from SARD~\cite{SARD}(\S\ref{fig:lemna_sard}) and NVD~\cite{booth2013national}(\S\ref{fig:lemna_nvd}). We show the \emph{heatmap} of each of the tokens in those examples as generated by LEMNA. Both of these examples are predicted a vulnerable. The background color of each token indicates corresponding token's \emph{heatmap} in the prediction. Most important code sub-sequence in the example shown in Figure~\ref{fig:lemna_sard} are {\tt \textbf{() \{ wchar\_t *}}, which apparently has nothing to do with vulnerability. This example also show how simple the code look in SARD dataset. This main reason behind the simplicity of the SARD dataset are twofold -- first, most of the examples in this dataset are synthetic and academic to illustrate the vulnerability. Second, the original purpose of this dataset is to evaluate a \vp tool, not learn from this dataset, which is much difficult task than evaluation. 

Figure~\ref{fig:lemna_nvd} shows an example from NDV dataset. Here the token sequence, {\tt \textbf{if (ss\_tc\_root != NULL)}} contributes the most in predicting this code snippet as vulnerable. Although, this example look slightly more complex than that of SARD dataset, there is not apparent reason how this specific portion of the code is the reason for real vulnerability. Most probably, this token sub-sequence is an artifact of NVD dataset. 

Finally, we summarize the lessons learned through the investigation and experiment in this section as, 

\smallskip
\noindent\textbf{Lesson 1:}~The existing dataset do not represent real world vulnerabilities very well. Result show that when we deploy such models in real world, those incur a lot of false positives and false negatives posing a threat to the applicability of those techniques in real world. To predict vulnerabilities in real world, we have to train a model with real world datasets.
% \smallskip
% \noindent\textbf{}

% For Figure~\ref{fig:lemna_ex2}, although the prediction result is correct, the token sub-sequence that contributed the most is the {\tt \textbf{if (ss\_tc\_root != NULL)}} statement which is likely an artifact of the dataset similar to the example (Figure~\ref{fig:example}) we showed before. 
% We answer this question from two different real world scenario. Our first scenario is when developers might not have sufficient annotated training data. In this case, they might want to use knowledge from other projects --\ie they would want to use the pre-trained model from other dataset. To investigate further, we chose four different Deep Learning models -- CNN, CNN+RF, BGRU, BLSTM. These models are proposed by previous approaches~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated} and four different datasets -- \ie Juliet~\cite{okun2013report}, VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and GitHub and Debian~\cite{russell2018automated}. These datasets are used to evaluate respective approaches. For predicting vulnerabilities from one dataset, we measure the performance of pre-trained models from other dataset. In this scenario, we are simulating a case, where for each test dataset, there is not enough annotated examples to train on. The dataset under test works as a proxy of real world vulnerabilities. Note that this paper's purpose is not to compare the performance of different deep learning architectures using the same dataset; such comparisons have already been shown in different researches~\cite{russell2018automated, li2018vuldeepecker, li2018sysevr}. Instead, we intend to explore how representative the datasets are across different DL models, where we pick a model that is reported to be the best-performing one \wrt a given dataset. We also designed an ensemble method 
% where we consult all the pre-trained models from existing datasets to predict vulnerabilities from a particular dataset.  

% \noindent Our second scenario is when there are annotated real world datasets are available. In this case, we tested the performance of aforementioned four models on two dataset. Our first dataset is real world vulnerabilities from Qemu and FFMpeg projects proposed by Zhou~\etal~\cite{zhou2019devign}. Our second dataset is real world vulnerabilities from Chromium and Debian project. 


% \smallskip
% \noindent
% \textbf{Results:}
% Table \ref{tab:cross} shows the experiment results on our first scenario. In this case, pre-trained models from all four approaches \ie  CNN+RF(\ref{tab:cross_cnnrf}), CNN(\ref{tab:cross_cnn}), BLSTM(\ref{tab:cross_blstm}), and BGRU(\ref{tab:cross_bgru}) are not very effective to predict vulnerabilities in the wild. Even though they all exhibit very high performance while tested on intra-dataset. 

% % \input{Tables/cross-dataset.tex}

% From the result, it is evident that the models trained on these datasets are not likely to generalize well on unseen data and real-world applications, given that they do not generalize well among themselves.
% For example, see the first row: when CNN+RF Model is trained and tested on Juliet dataset, it achieved 87\% accuracy. However, when tested with other datasets, the mean accuracy is dropped to 38\%.  The same observation is valid for F1 scores. Thus, it is clear that the such pre-trained model are not suitable for real-world applications, given that they do not generalize well among themselves. Table~\ref{tab:cross_ensemble} shows the performance when we ensemble the all the  pre-trained models. The results clearly show that, even if we try to leverage all the pre-trained models, it fails to effectively detect vulnerabilities. 

% \input{Tables/token_real_world}

% \noindent Table~\ref{tab:token_real_world} shows the performance of existing approaches on two different real world dataset. In both of those dataset vulnerability annotated examples are available to train DL based models. The results show that existing approaches fail to detect real world vulnerability even when there are annotated vulnerability data to train on. All four of the existing approach exhibit very poor performance in detecting those vulnerabilities.

% \input{Tables/slice_real_world}
% To understand the effect of slicing as championed by VulDeePecker and SySeVR, we extracted slices from functions in Devign dataset and \realdata. To have a fair comparison, if at least one of the slice extracted from a function is predicted by the models as vulnerable, we predict that function as vulnerable. Table~\ref{tab:slice_real_world} shows a comparison of two different slicing mechanisms and corresponding result. In slice granularity, CNN+RF model shows very poor performance. In function granularity, although the result is bit more promising, not all the code samples are considered to be prediction by a respective model. For instance, in \realdata, model trained on slices extracted from array indexing, the F1 is 25.55, but only 30.70\% (\%f column in the table) of the total function had at least one slice from array indexing statement and hence considered for prediction. This makes the model ineffective in predicting the rest 69.30\% functions.


% \noindent \textbf{Observation:} Existing pre-trained models fail to effectively detect vulnerabilities in the wild. Even when trained on real world vulnerabilities, those models do not generalize well. 

% \noindent
% \begin{table}[!htb]
%     \centering
%     \footnotesize
%     \vspace{-5mm}
%     \caption{\textbf{\small Test performance of existing dataset in ensemble settings.}}
%     \vspace{-3mm}
%     \begin{tabular}{c|c|c}
%     \toprule
%         Dataset under test & Accuracy & F1 \\
%         \midrule
%         Juliet & 54.5 & 41.08\\
%         \midrule
%         VulDeePecker & 52.83 & 44.08\\
%         \midrule
%         SySeVR & 46.5 & 26.58\\
%         \midrule
%         GitHub + Debian & 50.08 & 12.33\\
%         \bottomrule
%     \end{tabular}
%     \vspace{-3mm}
%     \label{tab:ensemble}
% \end{table}

% Since there are a lot of datasets available, one could ask what if, we learn from all the available datasets and models. To investigate this aspect, we designed an ensemble of different models and different datasets.  In this experiment, when we are predicting vulnerability from  a particular dataset, we consult the models developed from other datasets.  
 




==> RQ_details/rq2.tex <==
% !TEX root = ../fse_results.tex

\subsection{Limitations of Existing Modeling Techniques (RQ2)}
\label{sect:rq2}

% \begin{figure}
%     \centering
    
%     \begin{subfigure}{\linewidth}
%     \centering
%     \caption{Before Training}
%     \vspace{-3mm}
%     \includegraphics[width=\linewidth]{imgs/before-training.pdf}
%     \label{fig:before_train}
%     \end{subfigure}
%     \vspace{10mm}
%     \begin{subfigure}{\linewidth}
%     \centering
%     \caption{Training with CE Loss, Acc: 83.824	Pr: 29.730	Rc 56.156	F1: 38.877}
%     \vspace{-3mm}
%     \includegraphics[width=\linewidth]{imgs/no-triplet.pdf}
%     \label{fig:ce_loss}
%     \end{subfigure}
    
%     \vspace{10mm}
%     \begin{subfigure}{\linewidth}
%     \centering
%     \caption{Training with Triplet Loss, Acc: 85.667	Pr: 32.528	Rc 52.553	F1: 40.184}
%     \vspace{-3mm}
%     \includegraphics[width=\linewidth]{imgs/triplet.pdf}
%     \label{fig:triplet_loss}
%     \end{subfigure}
    
%     \caption{Caption}
%     \label{fig:my_label}
% \end{figure}

\input{Tables/rq2_problems}

In this RQ, we investigate on performances of different \dlvp approaches when they are trained on real world data. We distinguish between semantics based \vp techniques and syntax based vulnerability (\saikat{add a reference here to the section where these concepts were introduced}). We start with training various techniques on two real world datasets. We compare the baseline performance of the studied \vp techniques with their corresponding performance on real-world datasets. Hence we ask--

\red{Saikat: This paragraph reads like a summary, move to the result box} We observe that all those techniques do not achieve the same level of performance in real world dataset as those in (semi)-synthetic datasets. We also find that, to find vulnerability in real world dataset, model should consider the semantics of the code, in contrast to considering code as token sequences.

\smallskip
\noindent\textbf{\small RQ2: How do different \dlvp approaches perform when trained on real world data} 

We adopt three \vp techniques (\ie VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and Russel~\etal~\cite{russell2018automated}) proposed in existing literature and train those on real world datasets. For VulDeePecker, we extracted the code slices from API calls (backward slice only as reported by VulDeePecker) in the code. 
% VulDeePecker data repository does not provide API entry points for slice extraction, hence we used corresponding API entry points in SySeVR. 
For SySeVR, along with API call slice, we also extract the slices from Array Index, Arithmetic expression, and Pointer Usage. Slicing results in numerous duplicates\saikat{Add the numbers in ~\Cref{tab:duplicate}}. For instance, in the same line if an API is called with a pointer access, we will have two different slices (one from API slice, one from pointer slice). To understand the performance of the model itself, and to ensure that the model does not memorize specific slice due to the repetition, we de-duplicated the respective slice datasets for VulDeePecker and SySeVR. Note that, with VulDeePecker and SySeVR, we could not extract slices for all the examples in the dataset two dataset(\ie \realdata, and \devigndata). For all three of these techniques, we use the respective tokenization method.

We categorize these approaches in two categories -- (a) Syntax based modeling, (b) Semantic based modeling. Russel~\etal~\cite{russell2018automated}'s proposed approach is purely syntax based approach, since they consider the code as a sequence of tokens. Thus, their approach fall into Syntax based modeling category. VulDeePecker~\cite{li2018vuldeepecker} and SySeVR~\cite{li2018sysevr}, in contrast extract code slices from Control flow and data flow graphs and predict vulnerabilities on those slices. Since these two approaches consider some form of semantics into account, we categorize these two as semantic based modeling. 

Table~\ref{tab:all_method_comparison_real_world_datasets} shows the result of different approaches in predicting vulnerability in real world. Here we report the accuracy, precision, recall, and F1 score in each case. These performance measures are median on scores across 30 runs. We also show the inter-quartile range(IQR) to understand the spread of performances. 

VulDeePecker accounts from 21.46\% of the function in \realdata and 27.96\% of the functions in \devigndata \ie at least one slice from API calls can be extracted from those functions. But within that specific portion of the dataset, it achieves median F1 score of 45.06 in \realdata and 54.45 in \devigndata. SySeVR can be thought of extension of VulDeePecker where instead of extracting slice from one type of statement, SySeVR extracts from four types (API call, Array usage, Arithmatic Expression, and Pointer usage). This extension significantly improves the scope -- 66.42\% in \realdata and 84.08\% in \devigndata. In case of performance, SySeVR achieves higher performances than VulDeePecker. Note that, all the functions that are in VulDeePecker's scope are also in SySeVR's scope. 

Russel~\etal's proposed approach account for 100\% of the functions in both the dataset, since it does not rely of any specifics of the code. This type of approach can be thought of as holistic approach, since it tries to learn from the whole dataset rather than part of the dataset. However, as the result shows, the predictive performance of this model is significantly less than that of SySeVR. 

We conjecture that the performance boost in semantic based models than that of syntax based model is due to the consideration of the code semantics. In Russel~\etal's approach, code fractions that are semantically related might be far apart from one another with semantically irrelevant code fragments in between. When slices are extracted in VulDeePecker and SySeVR, any irrelevant code fragment are stripped away from the slice. Thus, from a DL model's perspective, it is easier to reason about slice than to reason about the whole code. 

\begin{result}
To effective \vp in real world data, semantic reasoning is necessary. One way of achieving semantic reasoning in \dlvp is extracting slices. However, with slicing it is tedious to define all slicing criteria. A holistic model that can reason with the semantics of the code can be very useful in real world \dlvp.
\end{result}
% \result{}

% Next, we focused on the structure of the code. First, we wanted some model based on the syntactic structure of the code. For doing so, we parsed the code into nodes using Joern~\cite{yamaguchi2015automatic}. These node mostly include AST nodes, other nodes include variable definition nodes, CFG nodes etc. We initialize each node with node type and node features. We extract node feature using Word2Vec~\cite{rong2014word2vec}. After getting the representation of every node, we get the graph level representation by summing up all the node in a graph. Hence, every graph is transformed to a real valued vector containing the information about all the node in that graph. Then we classify these vectors using traditional machine learning tools \eg Support Vector Machine (SVM), Logistic Regression (LR), K-Nearest Neighbor(KNN) etc. Note that, any trainable ML model can be used for this experiment, we chose these three as case study model. Also note that, while computing the graph representation in this case, we are not considering the any edges in the graph. Thus this representation is \emph{not} a complete semantic model, since semantic information (through control and data dependency edge) are not present here. 

% Finally, we consider the semantic model. For doing so, we collect the graph with six different type of edges \ie AST, control flow, data flow, data dependency (def-use), DOM and PDOM edges. We initialize the node in the same way as decribe in previous step. We then pass this graph to Gated Graph Neural Network(GGNN)~\cite{li2015gated}.  After generating the final representation of every node in a GGNN, we calculate the graph level representation by summing up all the node information and then pass that graph representation to a Fully Connected Neural Network to classify into vulnerable and non-vulnerable category. 

% In each case, we randomly split the dataset into 80\%-20\% train-test sets. To avoid any biases created by this randomness, we repeat the experiment 30 times.


% This result gives us a \emph{rough estimate} of how different types of model perform in predicting vulnerability. 



% As we can see, Graph + DL (GGNN) model performs best in both \realdata and \devigndata in terms of F1- score. In both the dataset, GGNN gives the highest recall (with statistical significance) meaning that it predicts less number of false negatives. KNN has the highest average value of precision. However, the precision result of KNN are \emph{not} significantly better compared to other method with statistical significance.

% Note that, among the token based models, SySeVR performs very well in both the datasets. However, as we have already mentioned, 66.42\% of the test code in \realdata and 84.08\% in \devigndata are in the scope for SySeVR (\ie at least once slice can be extracted following the 4 slice extraction method proposed by SySeVR). The performance of SySeVR and VulDeePecker in Table~\ref{tab:all_method_comparison_real_world_datasets} are \wrt to the code that are in-scope only for respective technique. 

% \smallskip
% \noindent\textbf{Observation 2.1} Semantic information and reasoning about it, plays a very important role in \vp task. Models that explicitly learn from semantic graph perform better in real world \vp. Having limited semantics information, VulDeePecker and SySeVR learn to do some reasoning about the semantics of the code and hence perform well in cases where appropriate slice can be extracted. In fact, SySeVR works very well in examples that are in its' scope. SySeVR proposed four different types if entry points for extracting slices. 

% In theory, slices can be extracted from any point of the program. However, if we extract slices from every point in the code, number of slices will explode. This problem is similar to the path explosion problem in testing~\cite{boonstoppel2008rwset}. Thus we argue, reasoning on graph as a whole instead of reasoning on individual slices are better choices. 

% Since rest five methods (Russel~\etal~\cite{russell2018automated}, SVM, LR, KNN, and GGNN) work with 100\% of the data, we present a Scott-Knott ranking on the F1 score of different approaches to prove an approach is better with statistical significance.
% \smallskip
% \noindent\textbf{Statistically Sound Comparison.} As described in Section~\ref{subsec:real-world-evaluation}, to prove a technique is better than another, some statistical test is necessary. There are several statistical test available to testing hypotheses with different assumptions and different properties. For instance, t-statistic test assumes that the samples we are testing would follow a gaussian distribution. In our evaluation, we will be comparing performance of multiple approaches. For such case, Scott-Knott method is championed by software engineering researchers~\cite{krishna2018bellwethers, mittas2012ranking}. For a group of samples (in our case performance measures), Scott-Knott, recursively splits the group to establish statistical significance of one group over other using Hypothesis testing. In theory, any hypothesis testing can be used in conjunction to Scott-Knott method. In our evaluation, we followed the A12 test, which has been highly used and championed in Software Engineering research~\cite{krishna2018bellwethers}.

% \input{Tables/rq2_comparison}

% Table~\ref{tab:statistical_comparison} shows the ranking of those five methods, the median performance, and Inter-Quartile Range(IQR) of each of the approaches. As we can see, in both the dataset, GGNN is in the top rank and is not ties with any other method. Here is an interesting finding from this result, even though Russel~\etal has the higher average f1-score than SVM in \realdata, it is not significantly better. Thus, in Table~\ref{table:comparison_chrome_deb_f1}, those two method are tied in third rank. Similarly, in \devigndata, SVM, LR and Russel~\etal are not significantly better than one another.

% \smallskip
% \noindent\textbf{Observation 2.2. Having good result in one run of the experiment, even having good result on average does not prove a method is significantly better than other.}

% Thus we summarize the lessons learned in this research question, 

% \smallskip
% \noindent\textbf{Lesson 2} Graph based models should be used for real world \vp. Further investigation of improved graph based model will unveil better reasoning. While comparing with two approaches, statistical significance test should be performed to rule our the ``luck factor''.



% \begin{table}[]
%     \centering
    
% \end{table}

% \begin{table}[!htb]
%     \centering
    
% \end{table}


% \noindent\textbf{RQ2. Why do current vulnerability prediction models fail in real-world situations?}

% In this RQ, we thoroughly investigate why existing Deep Learning based Vulnerability Detection systems fail to generalize in real world scenario. We investigate the problems with existing approaches from different angles -- first, we investigate the data on which the models pre-trained on; second, we investigate different aspect of the existing approaches. 

% Our first part of investigate research question is 

% \noindent\textbf{Experiment 2.1.2} As we have seen in the previous experiment, the existing datasets are highly repetitive, we investigate on the learned features from those datasets. To understand that better, we intend to examine the activation of the data with respect to its predictions, namely what kind of patterns are triggering the prediction for a piece of code to be vulnerable. As a case study, we examine the trained CNN model. We use the guided back-propagation technique~\cite{springenberg2014striving} to calculate the gradient given its prediction label with respect to the input token embedding. 
% To understand what is actually triggering a prediction, we only take the positive guided-gradients and normalize it. Since each embedding is a vector, to get the activation value per embedding, we sum them over the embedding dimension. The procedure is described in Algorithm~\ref{algo:guided_backprop} in details.

% \begin{algorithm}
% \footnotesize
% \SetAlgoLined
% \KwResult{Activation values $av_{i,j}$ for $i^{th}$ sample's $j^{th}$ token}
%  \textbf{Input} Data $x_i, \forall i \in \{1,\ldots, N\}$ with sequence length $M$ and embedding size $K$\;
%  \textbf{Model} $F(\cdot): \mathbb{R}^{M\times K} \to \mathbb{R}^{2}$\;
%  \For{$i \in \{1,\ldots, N\}$}{
%  $\hat{y_i} = \arg \max F(x_i)$\;
%  $\nabla_i = $ GuidedBackPropagation($F(\cdot), x_i, \hat{y_i}) \in \mathbb{R}^{M\times K}$\;
%  $\nabla_i^{+} = \max(0, \nabla_i) ./ \max(\nabla_i)$\;
%  $av_i = $ RowSum($\nabla_i^{+}$) $\in \mathbb{R}^{M}$
%  }
%  \caption{The procedure for obtaining activation values using guided back-propagation.}
%  \label{algo:guided_backprop}
% \end{algorithm}

% Since we are dealing with sequences, we search for the top sub-sequences that have highest average activation values in between consecutive tokens up to a certain length across the data entries. In this case we set the maximum length to five based on our experiment results. These sub-sequences are  the top features that the CNN model is learning. To investigate the prevalence of those features, we also calculated the top features' prevalence ratio, that is defined as the following.

% The prevalence ratio for $i^{th}$ feature ($f_i$) of $j^{th}$ class ($y=j$):

% \begin{align*}
%     \mathrm{Prevalence_{i, j}} = \frac{\sum_{k:\; y_k = j} \mathrm{Count}_{f_i}(x_k)}{\sum_{k:\; y_k \neq j} \mathrm{Count}_{f_i}(x_k)} \cdot \frac{|\{x_k:\; y_k \neq j\}|}{|\{x_k:\; y_k = j\}|}
% \end{align*}
% $\mathrm{Count_{f_i}(\cdot)}$ counts the number of occurrence of $f_i$ in its input, $|\{x_k:\; y_k = j\}|$ calculates the number of samples that belongs to $j^{th}$ class, similarly $|\{x_k:\; y_k \neq j\}|$ calculates the number of samples that does not belong to $j^{th}$ class.

% In plain English, the higher the prevalence ratio, the more the featured appeared in the specified class.

% \input{Tables/learned_features}

% \noindent \textbf{Result 2.1.2:} It can be observed that the model learnt different features from different datasets. In general, the top features can not be directly linked to any vulnerabilities by simply looking at it except for the features learnt from Github + Debian~\cite{russell2018automated}, which is likely to be related to buffer overflow but it is also plausible to be an artifact due to its high prevalence ratio. 

% The top features learnt from SATE IV Juliet~\cite{okun2013report} are mostly related to referencing variables and identifiers, difficult to see what these features represent but not necessarily meaningless. The features have low prevalence ratio which indicates that they are not learnt based on local patterns.

% \begin{figure}
%     \centering
% \begin{lstlisting}
% init_JSON_config(JSON_config* config)
% {
%     if (config) {
%         memset(config, 0, sizeof(*config));
%         config->depth = JSON_PARSER_STACK_SIZE - 1;
%         config->malloc = malloc;
%         config->free = free;
%     }
% }
% \end{lstlisting}
%     \caption{\small{\textbf{One non-vulnerable code example from Github + Debian~\cite{russell2018automated} dataset that contains the top features (such as {\tt malloc}) and was misclassified as vulnerable.}}}
%     \label{lst:codesample}
% \end{figure}
% \vspace{-6mm}

% Most of the top features learnt from VulDeePecker~\cite{okun2013report} are clearly not related to vulnerabilities, ``5" and ``[ 5" are likely appeared in the original dataset as a part of some Flow Variants. The last feature ``FUNC ( DEC , LITERAL" could be related to vulnerabilities induced by function calling. However, it has two features that have prevalence ratio greater than one, which point out that these two, especially ``- LITERAL ;", might be an artifact. 
% The top features learnt from SySeVR~\cite{li2018sysevr} are similar to the features learnt from VulDeePecker~\cite{li2018vuldeepecker}, mostly related manipulation of variables that are difficult to decipher. However, they have three features with greater than one prevalence ratio, which indicates that the features are likely to be bound locally.

% The top features learnt from Github + Debian~\cite{russell2018automated} are significantly different from the previous, all of them are C/C++ library functions such as {\tt fopen}, {\tt malloc}, {\tt memcpy} and {\tt read}. Notice that these features have much higher prevalence ratio than the previous features, also these functions is highly likely to be related to memory/buffer-based vulnerabilities, we conjure that these features might be caused by its labelling functions that are static analyzers, which are inclined to be artifacts. Listing~\ref{lst:codesample} shows an example to illustrate a typical scenario where these learnt features might misguide the prediction. In this case, the buffer overflow is properly handled and hence it is not a vulnerable code. However, this code snippet is classified as vulnerable by the model. So although the learned features are more reasonable, the system is still far from perfect.

% \noindent \textbf{Observation 2.1.2 :} The code sub-sequences that are learned as top features by existing Deep Learning are not directly related to vulnerability. High prevalence of such features forces models to learn those patterns instead of effectively learning the vulnerability patterns. 

% So far, we have seen that the four synthetic dataset are biased. Now we are curious to see why those model should not work if trained on real world code and real world vulnerability annotations. Thus, the second part of our research question, \textbf{RQ2.2 What are the challenges with the available approaches?}

% \noindent\textbf{Experiment 2.2 } To answer this question, we systematically investigate several aspects -- \eg code pre-processing method, code abstraction methods, type of the models, etc., from the existing approaches. We observe that CNN~\cite{russell2018automated}, BLSTM~\cite{li2018vuldeepecker}, BGRU~\cite{li2018sysevr} all are token based models. In addition, all these approaches use symbolic code pre-processing techniques, where concrete identifier names are replaced by abstract identifiers. To this end, we investigate,
% \textit{What if we use concrete identifier names instead of the abstract?},  
% \textit{What if we consider structural and semantic information of the code?}, and
% \textit{What if we learn structural neural networks for code?}

% We first trained a Word2Vec~\cite{rong2014word2vec} model trained on large corpus of code. 
% To really understand the contribution of concrete identifier names, we design a simple SVM based model on top of the Word2Vec based token embedding. Next, we concatenate the AST node type information with the token embedding and use SVM to understand influence of AST information. Finally, we design a Graph Based Neural Network to detect vulnerability given the flow graph of a program.  

% \textbf{Result 2.2 } Table~\ref{tab:rq2_table} shows accuracy and F1 score on \realdata and Devign dataset. As the results show in both the cases, if we use Word2Vec, even a very simple model line Linear SVM outperforms Deep Learning based CNN + RF models' performance. The F1 score increases from 45.71 to 53.18 in Devign data and from 8.78 to 16.55 in \realdata respectively. This result clearly indicates the code tokens play important role in real-world vulnerability detection task. In addition, if we add AST node type information, the performance increases slightly. Finally, we extract the control and data flow graph from the program function and use Graph Based Neural Network to classify that. Similar graph neural network based technique is recently used by Xhou~\etal~\cite{zhou2019devign}. When a Graph Neural Network is used, the F1 score increases to 61.61 in Devign dataset and 25.97 in \realdata rendering 35\% and 195\% improvement than that of original CNN + RF approach. 

% \noindent\textbf{Observation 2.2 } Concrete names of the code tokens, structural and semantic information play very important role in real life vulnerability detection. Existing models ignored these properties and hence failed to work well in real world scenario. 



% % \begin{itemize}
% %     \item Data Problem
% %     \begin{itemize}
% %         \item Clone
% %         \item Repetitive Features
% %     \end{itemize}
% %     \item Approach Problem
% %     \begin{itemize}
% %         \item Preprocessing
% %         \item Simple model 
% %     \end{itemize}
% % \end{itemize}


% % \noindent \textbf{Data Problem}


==> RQ_details/rq2_backup.tex <==
\textbf{Question :  Why models trained with existing approaches fail to detect vulnerabilities in the wild? }

\begin{figure}[!htb]
\vspace{-3mm}
  \centering
  \includegraphics[width=0.8\linewidth,height=0.8\linewidth, keepaspectratio = true]{./imgs/clone_percent.pdf}
  \caption{\small{\textbf{Portion of code clones in each dataset.}}}
  \label{fig:clone-ratio}
\vspace{-2mm}
\end{figure}

\begin{figure}[!htb]
\vspace{-1mm}
  \centering
  \includegraphics[width=0.8\linewidth,height=0.8\linewidth, keepaspectratio = true]{./imgs/dist_clone.pdf}
  \caption{\small{\textbf{Homogeneity of clone clusters for each dataset, red denotes cluster that is mostly constituted with vulnerable code, blue denotes cluster that is mostly constituted with non-vulnerable code.}}}
  \label{fig:clone-distro}
\vspace{-4mm}
\end{figure}

\textit{Result.} 
The results in figure~\ref{fig:clone-ratio} and figure~\ref{fig:clone-distro} show that Github + Debian~\cite{russell2018automated} and SATE IV Juliet~\cite{okun2013report} have less than 50\% of the code samples that are unique to each other, and the majority of the datasets, including our baseline dataset, has around 30\% code samples that has a clone in it. From the homogeneity plot, we can notice that the baseline dataset, the SATE IV Juliet dataset~\cite{okun2013report}, and the VulDeePecker dataset~\cite{li2018vuldeepecker} have the two classes mixed in the clone clusters which might potentially help the generalizability of the model trained on them since it is not likely the model will pick up the clones as meaningful features, while SySeVR~\cite{li2018sysevr} and Github + Debian~\cite{russell2018automated} dataset have most of their clone clusters consisted of only one class code samples which could make the clones as features for the model to learn.

LEMNA~\cite{guo2018lemna} is proposed to explain the black-box (\ie, non-explainable) deep learning models by estimating the local decision boundary around a data point using a white-box (\ie, explainable) linear model.

Given an example data point $(x_i,\;y_i),\;i\in \{1,\ldots,N\}$ where $x_i$ is the input sequence and $y_i$ is the label, LEMNA~\cite{guo2018lemna} samples around $x_i$ to obtain $L$ synthetic input sequences $z_{i,j},\;j\in \{1,\ldots,L\}$ and its prediction labels $w_{i,j},\;j\in \{1,\ldots,L\}$. Put the original data point along with the sampled data points, a mixture linear regression model with fused lasso regularization is fitted. Each of the token $x_i^t$ is assigned a weight $\omega_i^t$ representing the contribution of that token for prediction. Higher value of $\omega_i^t$ would indicate larger contribution of token $x_i^t$ in predicting $y_i$. Details can be found in the paper~\cite{guo2018lemna}. We adopted this visualization technique to investigate contribution on different token sub-sequences of a input code snippet on the output vulnerability label. 
\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{imgs/lemna-viz-ex-1.pdf}
    \caption{\small{\textbf{Contribution of different token sub-sequences for a given sample code snippet with false vulnerable prediction. Highest contribution to lowest contribution in the order of {\color{red} red}, {\color{orange} orange}, {\color{yellow} yellow}, {\color{green} green}. }}}
    \label{fig:lemna_ex1}
    \vspace{-2mm}
\end{figure}

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{imgs/lemna-viz-ex-2.pdf}
    \caption{\small{\textbf{Contribution of different token sub-sequences for a given sample code snippet with true vulnerable prediction. Highest contribution to lowest contribution in the order of {\color{red} red}, {\color{orange} orange}, {\color{yellow} yellow}, {\color{green} green}.}}}
    \label{fig:lemna_ex2}
\end{figure}

Figure~\ref{fig:lemna_ex1} and Figure~\ref{fig:lemna_ex2} show examples of visualization using LEMNA. Both has been predicted as vulnerable by the model, with one having ground truth as non-vulnerable and one having ground truth as vulnerable. The background color of each token indicates corresponding token's contribution in the prediction. For Figure~\ref{fig:lemna_ex1}, as shown in the picture the token sub-sequence contributing to the prediction of the code snippet is {\tt \textbf{() \{ wchar\_t *}}, which apparently has nothing to do with vulnerabilities. For Figure~\ref{fig:lemna_ex2}, although the prediction result is correct, the token sub-sequence that contributed the most is the {\tt \textbf{if (ss\_tc\_root != NULL)}} statement which is likely an artifact of the dataset similar to the example (Figure~\ref{fig:example}) we showed before. 


While this visualization technique gives us an initial pointer for investigating the feature (token) contribution in each of the individual prediction, this does not give us a collective idea of what are the feature captured by a trained model. To investigate that, we propose a feature ranking mechanism by guided back propagation in the model. 

\textbf{Feature Ranking with Guided Back-propagation}
\subsubsection*{\textbf{Methodology \& Experiment Setting}}
We intend to examine the activation of the data with respect to its predictions, namely what kind of patterns are triggering the prediction for a piece of code to be vulnerable. As a case study, we examine the CNN model that is trained according to the description in Section~\ref{sec:Empirical_Generalization_Test}. We use the guided back-propagation technique~\cite{springenberg2014striving} to calculate the gradient given its prediction label with respect to the input token embeddings. In the next step, we extracted the positive saliency map by zero-out the negative numbers in the guided-gradient and normalize it since we only cared about what triggers the prediction not what suppress the prediction. We then sum over the embedding dimensions to obtain the activation values for each token. The entire procedure is described in Algorithm~\ref{algo:guided_backprop} in details.

\begin{algorithm}
\SetAlgoLined
\KwResult{Activation values $av_{i,j}$ for $i^{th}$ sample's $j^{th}$ token}
 \textbf{Input} Data $x_i, \forall i \in \{1,\ldots, N\}$ with sequence length $M$ and embedding size $K$\;
 \textbf{Model} $F(\cdot): \mathbb{R}^{M\times K} \to \mathbb{R}^{2}$\;
 \For{$i \in \{1,\ldots, N\}$}{
 $\hat{y_i} = \arg \max F(x_i)$\;
 $\nabla_i = $ GuidedBackPropagation($F(\cdot), x_i, \hat{y_i}) \in \mathbb{R}^{M\times K}$\;
 $\nabla_i^{+} = \max(0, \nabla_i) ./ \max(\nabla_i)$\;
 $av_i = $ RowSum($\nabla_i^{+}$) $\in \mathbb{R}^{M}$
 }
 \caption{The procedure for obtaining activation values using guided back-propagation.}
 \label{algo:guided_backprop}
\end{algorithm}

Since we are dealing with sequences, we search for the top sub-sequences that have highest average activation values in between consecutive tokens up to a certain length across the data entries. In this case we set the maximum length to five based on our experiment results. We also calculated the top features' prevalence ratio, that is defined as the following.

The prevalence ratio for $i^{th}$ feature ($f_i$) of $j^{th}$ class ($y=j$):

\begin{align*}
    \mathrm{Prevalence_{i, j}} = \frac{\sum_{k:\; y_k = j} \mathrm{Count}_{f_i}(x_k)}{\sum_{k:\; y_k \neq j} \mathrm{Count}_{f_i}(x_k)} \cdot \frac{|\{x_k:\; y_k \neq j\}|}{|\{x_k:\; y_k = j\}|}
\end{align*}
$\mathrm{Count_{f_i}(\cdot)}$ counts the number of occurrence of $f_i$ in its input, $|\{x_k:\; y_k = j\}|$ calculates the number of samples that belongs to $j^{th}$ class, similarly $|\{x_k:\; y_k \neq j\}|$ calculates the number of samples that does not belong to $j^{th}$ class.

In plain English, the higher the prevalence ratio, the more the featured appeared in the specified class.

\subsubsection*{\textbf{Experiment Result}} We listed the top five features learnt by the CNN model from the existing datasets, as well as their average activation value and prevalence ratio in Table~\ref{tab:feature}.

\begin{table}[!htb]
\caption{\small{\textbf{Feature exploration experiment results.}}}
\centering
\footnotesize

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{3cm}|c|c}
\toprule
\textbf{Feature}        & \textbf{Mean Activation}              & \textbf{Prevalence}   \\ 
\midrule
IDENT ( *                   & 5.56  & 0.65 \\
VARIABLE *            & 5.38  & 0.42 \\
\{ IDENT ( *                & 5.32 & 0.63 \\
\{ IDENT * VARIABLE ; & 5.24  & 0.59  \\
) \{ IDENT * VARIABLE & 5.17  & 0.59 \\
\bottomrule
\end{tabular}
\caption{\small{Top vulnerability-related features in SATE IV Juliet~\cite{okun2013report}.}}
\end{subtable}

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{3cm}|c|c}
\toprule
\textbf{Feature}        & \textbf{Mean Activation}              & \textbf{Prevalence}               \\
\midrule
5                              & 5.38 & 0.97 \\
{[} 5                          & 4.84 & 0.86  \\
\{ IDENT                       & 4.80 & 0.73 \\
- LITERAL ;                    & 4.64 & 12.75  \\
FUNC ( DEC , LITERAL       & 4.57 & 1.10 \\ 
\bottomrule
\end{tabular}
\caption{\small{Top vulnerability-related features in VulDeePecker~\cite{li2018vuldeepecker}.}}
\end{subtable}

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{3cm}|c|c}
\toprule
\textbf{Feature}        & \textbf{Mean Activation}              & \textbf{Prevalence}               \\ 
\midrule
NULL ; VARIABLE      & 5.14  & 1.22 \\
$>$ strlen        & 5.10  & 2.08  \\
VARIABLE -           & 4.88  & 0.18 \\
, IDENT $|$                  & 4.66  & 2.01 \\
int VARIABLE = IDENT & 4.66  & 0.70 \\
\bottomrule
\end{tabular}
\caption{\small{Top vulnerability-related features in SySeVR~\cite{li2018sysevr}.}}
\end{subtable}

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{3cm}|c|c}
\toprule
\textbf{Feature}        & \textbf{Mean Activation}              & \textbf{Prevalence}               \\ 
\midrule
fopen   & 6.69 & 17.61 \\
malloc  & 6.02 & 7.20  \\
fopen ( & 5.22 & 17.64 \\
memcpy  & 4.99 & 10.62 \\
read    & 4.82 & 4.49  \\
\bottomrule
\end{tabular}
\caption{\small{Top vulnerability-related features in Github + Debian~\cite{russell2018automated}.}}
\end{subtable}
\label{tab:feature}
\vspace{-4mm}
\end{table}

It can be observed that the model learnt different features from different datasets. In general, the top features can not be directly linked to any vulnerabilities by simply looking at it except for the features learnt from Github + Debian~\cite{russell2018automated}, which is likely to be related to buffer overflow but it is also plausible to be an artifact due to its high prevalence ratio. 

The top features learnt from SATE IV Juliet~\cite{okun2013report} are mostly related to referencing variables and identifiers, difficult to see what these features represent but not necessarily meaningless. The features have low prevalence ratio which indicates that they are not learnt based on local patterns.

Most of the top features learnt from VulDeePecker~\cite{okun2013report} are clearly not related to vulnerabilities, ``5" and ``[ 5" are likely appeared in the original dataset as a part of some Flow Variants such as the example showed in Section~\ref{sec:back}. The last feature ``FUNC ( DEC , LITERAL" could be related to vulnerabilities induced by function calling. However, it has two features that have prevalence ratio greater than one, which point out that these two, especially ``- LITERAL ;", might be an artifact. 

The top features learnt from SySeVR~\cite{li2018sysevr} are similar to the features learnt from VulDeePecker~\cite{li2018vuldeepecker}, mostly related manipulation of variables that are difficult to decipher. However, they have three features with greater than one prevalence ratio, which indicates that the features are likely to be bound locally.

\begin{lstlisting}[caption = \small{\textbf{One non-vulnerable code example from Github + Debian~\cite{russell2018automated} dataset that contains the top features (such as {\tt malloc}) and was misclassified as vulnerable.}},basicstyle=\scriptsize\tt ,captionpos=b, label = {lst:codesample}]
init_JSON_config(JSON_config* config)
{
    if (config) {
        memset(config, 0, sizeof(*config));
        config->depth = JSON_PARSER_STACK_SIZE - 1;
        config->malloc = malloc;
        config->free = free;
    }
}
\end{lstlisting}

The top features learnt from Github + Debian~\cite{russell2018automated} are significantly different from the previous, all of them are C/C++ library functions such as {\tt fopen}, {\tt malloc}, {\tt memcpy} and {\tt read}. Notice that these features have much higher prevalence ratio than the previous features, also these functions is highly likely to be related to memory/buffer-based vulnerabilities, we conjure that these features might be caused by its labelling functions that are static analyzers, which are inclined to be artifacts. Listing~\ref{lst:codesample} shows an example to illustrate a typical scenario where these learnt features might misguide the prediction. In this case, the buffer overflow is properly handled and hence it is not a vulnerable code. However, this code snippet is classified as vulnerable by the model. So although the learned features are more reasonable, the system is still far from perfect.




==> RQ_details/rq3.tex <==
% !TEX root = ../fse_results.tex

\subsection{Improving real-world DLVP}
\label{sect:rq3}

In this section, we look closer into the two real world dataset (\realdata and \devigndata) we investigated in this study. We look into different properties of the data from conceptual and empirical point of view. 

\smallskip
\noindent\textbf{Contrast between \realdata and \devigndata}~ Recall our proposed data collection algorithm(Algorithm~\ref{alg:real_data_collection}), from a vulnerable issue report, we extracted the functions that are changed to fix that vulnerability. For those functions, the version before the fix are vulnerable. and the the version after the fix are non-vulnerable. Until this point our data collection and \devigndata data collection is similar. However, as described in Section~\ref{subsec:background_overview}, From this data, this data represents how a function changes while a vulnerability is fixed -- any model trained on this dataset will supposedly learn the contrast between the version in the fix. We call such data \horizontal data. 

Now, let think about the use case scenario --\ie how a trained \vp is model will be used by a software developer. At some phase of development, they will deploy the model to check whether there is a vulnerability in their code or not. In such a scenario, the model has to distinguish between a vulnerable function and other ``supposedly'' non-vulnerable function from a particular snapshot of the codebase. Intuitively, a model which is only learned from different version of code will not do very good in such a use case. With this intuition in mind, we also annotated any function in the file that are not changed in the fix as non-vulnerable. A new type of dataset can be created that contains functions from only the version before the vulnerability fix for learning to discriminate a vulnerable function from every other functions in its' context. We call such a dataset \vertical data. Note that, \realdata is a combination of both \vertical and \horizontal data. \devigndata, in contrast only \horizontal data. 

The \horizontal nature of \devigndata makes it highly balanced. For instance, \ie 45\% of functions in \devigndata are vulnerable. Intuitively, this ratio of vulnerability is not natural -- certainly not 45\% of the function is a project are not vulnerable. In contrast, \realdata contains only 10\% vulnerable code. We considered only the files that are changed in a particular vulnerability fix. If we also consider the files that are not changes, the percentage will be even lower. Thus, we argue that, any evaluation shown on a test set which contains 45\% of vulnerable data is not a plausible real world evaluation. 

\subsubsection{Effect of Data Imbalance}
\label{subsec:rq3-data-imbalance}
Recall Section~\ref{sec3:models}, where we argued that training data has to be balanced to train effectively. We agree that developer and/or researchers are at liberty to manipulate the ``\emph{training}'' data distribution in anyway to facilitate the effective training, but the testing data should follow the actual distribution. To empirically test whether imbalance in test data has any influence on the performance, we design the following experiment. 

For a random disjoint split of train and test data in \devigndata, we train a GGNN model on the training data. Now, we artificially create imbalance in the testing data to mimic the imbalance in real world. We create a modified test set from the original test set by randomly dropping vulnerable examples. Then we calculate performance of this modified test set. To avoid any bias created by this randomness, we repeat this experiment 30 times. 

\begin{table}[!htb]
    \centering
    \footnotesize
    \caption{\small Effect of test set imbalance in \devigndata.}
    \begin{tabular}{l|r|r|r}
    \textbf{Settings}  & \textbf{Precision} & \textbf{Recall} &  \textbf{F1}\\
     \hlineB{2}
    Balanced & \textbf{56.27} & 65.49 & \textbf{60.40} \bigstrut\\
    \hline
    Imbalanced & 14.04 & 66.97 & 23.22 \bigstrut\\
    \hlineB{2}
    \end{tabular}
    \label{tab:artificial_imbalance}
\end{table}


Table~\ref{tab:artificial_imbalance} shows the result when we impose the real world test data distribution(approx.) in the \devigndata. As we can see, precision significantly reduced resulting is a significant loss in f1-score. This result now is consistent with GGNN result in \realdata where we has low precision and moderate recall. Thus, the lesson we learned, 

\smallskip
\noindent\textbf{Lesson 3.1} Having code and annotation from real world is not good enough. Any approach to be effectively used in real world should evaluate on real world data distribution as well.

\subsubsection{Data Balancing in Training}
\label{subsec:data_balancing_evaluation}

\input{Tables/balance_exp}

In this section, we show an ablation study on the effect of data balancing before training as proposed in Section~\ref{sec3:models}. We limit this experiment to \realdata, since \devigndata is already almost balanced. In this experiment, we train a model on imbalanced training dataset. Then we create 10 different strategy of balancing the training data. We created 10 different settings of balanced training data with various degree of under-sampling and over-sampling(see section ~\ref{sec3:models} for details). 

The effects of various data balancing are shown in Table~\ref{tab:balance_exp}. When $k$ is 1, it implies no over-sampling. When $k$ is 10, it implies the vulnerable examples are replicated 10 times and there is no under-sampling. Table~\ref{tab:balance_exp} shows the result in terms of F-1 score. We also did a Scott-Knott ranking to understand relative capabilities of the settings. As we can see, training on a balanced data improves the test f1 score ~40\% more than that of imbalanced training. Different balancing setting results in different f1 outcome. All of which are statistically significant than that of learning from imbalanced data. 

\noindent\textbf{Lesson 3.2} Training data should be balanced to reduce any bias in the training from the data imbalance. 


% \noindent\textbf{RQ3. How to improve real world \vp?}

% \noindent 
% \textbf{Motivation }
% Now that we have seen Graph Neural Network Based modeling works better on detecting real world vulnerabilities, we restrict ourselves on studying that model only. However, all the empirical finding reported in this section also holds for SVM based model that is described in previous RQ. In this research question, we investigate what other problem we might face while graph based vulnerability modeling. Investigation of other more sophisticated models than graph based models are beyond scope of this paper. One clear observation from Table~\ref{tab:rq2_table} show significantly lower f1 score in \realdata ~than
% % we should specify f1 rather than the word "performance", since the in the table-8, the acc in chrome is higher than devign, which will puzzle the reader and weaker our motivation
% Devign~\cite{zhou2019devign} dataset, which led us investigate on the properties of these two dataset. For better understanding the data property, we look at the data collection procedure. In summary, to collect vulnerability data, Devign first looked at the vulnerability fix commits. The version of a function before a vulnerability fix commit is marked as vulnerable code and the  version after the commit is marked as non-vulnerable code, rendering a very balanced set ($\sim$46\% code vulnerable and $\sim$54\% non-vulnerable code). 
% % This is a legitimate data collection approach. Data collected this way is better suitable for training purpose. However, this collected data does not simulate the real world \vp scenario, since in such case, most of the code are vulnerable. 
% In contrast, \realdata contains only $\sim$10\% vulnerable code and $\sim$90\% non-vulnerable code. Hence, ask 
% \textbf{RQ3.1 How does imbalance in data effect in \vp performance and how to solve this problem?}

% \noindent First, we intent to investigate the affect of imbalance in a trained model.

% \noindent\textbf{Experiment 3.1.1} In this experiment, we choose a fully trained model trained with Devign train set. Then we artificially impose the realistic data imbalance by randomly dropping vulnerable examples in the test set and measure the performance. To mitigate the threat of any potential bias introduced by random dropping, we repeat this experiment 30 times since we expect the performance to follow a Gaussian distribution and 30 is sufficient sample size for this. 

% \noindent\textbf{Result 3.1.1} In this experiment, we find the accuracy of Devign dropped to 59.74\% and F1 score dropped to 23.22  compared to the 62.56\% accuracy and 61.61 F1 score in balanced setting. In this experiment, we empirically proved the point that a model may perform very well in balanced test data. However, the performance drops drastically 
% when there is a high imbalance in the test data. Note that, creating imbalance in the way we described here does not anyway mimic the real distribution. Even with simulated imbalance, models trained in this fashion break.


% \noindent The data distribution between vulnerable and non-vulnerable classes in Devign dataset does not resemble real distribution. \realdata , in contrast, mimics real world \vp scenario better, since we annotated the function that is changed in a vulnerability fix commit as vulnerable, and rest of the functions in that file as non-vulnerable (see Section~\ref{sec:back} for details of data collection procedure). Both the training and testing data in \realdata~are highly imbalanced with ($\sim$10\% vulnerable code, and $\sim$90\% non-vulnerable code). We observe that this imbalance in training data is hindering the performance of the model. Thus, we investigate, how do we fix the data imbalance problem in \realdata?

% % \textbf{Question: How well does existing models perform in real world dataset? (RQ3)}

% \noindent\textbf{Background } Learning from imbalanced data is a very well studied topic in machine learning~\cite{liu2008exploratory, chawla2002smote, chawla2009data, barua2012mwmote}. Several technique are proposed to solve this imbalance learning problem. Two prominent directions of approach are Undersampling (where samples from majority class are discarded) and Oversampling (where synthetic samples are added to the minority class)\footnote{In our case, non-vulnerable samples and minority belong to majority class and vulnerable samples to the minority class.}. Often the Oversampling and Undersampling techniques are guided by domain knowledge specific to the problem. For instance, SMOTE~\cite{chawla2002smote} and MWMOTE~\cite{barua2012mwmote} finds interesting minority samples sample based on their distance from the nearest majority sample and synthesize around those minority samples. 

% \noindent\textbf{Experiment 3.1.2 } In this experiment, every time we train a model, we re-balance the training set without altering the ratio in the held out test set. We test various degree of oversampling and undersampling.Unlike SMOTE or MWMOTE, all vulnerable code are interesting to us, and we give equal preference to all vulnerable samples for oversampling, and during undersampling, we randomly discard non-vulnerable code to match the count of vulnerable samples in the training data. We do not directly adopt SMOTE or MWMOTE, because it is not clear how to synthesize vulnerable code. Even if we manage to synthesize vulnerable code sample, that synthetic data might suffer from the same problem we investigated in Section~\ref{subsec:rq2}.



% \noindent\textbf{Result 3.1.2 } Table~\ref{tab:balance_exp} shows the \vp performance with various degree of oversampling and undersampling. We measure 10 different settings, in each settings, we replicate each of the vulnerable samples by $N$ times and discard $P\%$ of non-vulnerable samples. At every balanced settings, the dataset is perfectly balanced. With vulnerable samples replicated 0 times (\ie no oversampling) and discarding 90\% of non-vulnerable code is one extreme of our test spectrum \textemdash this is most undersampling. Another extreme point is where each vulnerable samples are replicated 9 times and none of the non-vulnerable code is discarded \textemdash this is most oversampling. The result shows that as we increase the oversampling, the precision is increasing indicating that the model is better learning to predict non-vulnerable examples \ie producing less number of False Positives. With the increasing percentage of undersampling, the recall is increasing indicating that model better learning to predict vulnerable examples \ie producing less number of False Negatives. A good tradeoff between these 2 trends (N = 7 and P = 20\%) leads to the optimal performance in F1. In optimum setting, the F1 is 35.89 which is 38.2\% more than that of the baseline imbalanced settings. However, we make N and P as user parameter so that they can choose based of their preference between precision and recall. 

% \noindent\textbf{Observation 3.1 } Real world \vp data are highly imbalanced and a good model working very well in balanced setting may perform poorly in imbalanced test settings. To learn from any imabalanced \vp dataset, proper balancing should be done only on the training part of the data before training a model.

% So far, we have seen that model trained on Devign data breaks on imbalanced settings, even if we simulate that imbalance. However, we realize that \realdata and Devign datasets are fundamentally different. As described in section~\ref{sec:real_world}, \realdata is collected to differentiate between vulnerable function from other non-vulnerable functions in its context. Devign, on the other hand is collected to learn to discriminate between before and after changes of a vulnerability fix commit. In that way, \realdata is a vertical information source and Devign dataset is a horizontal information source, making this two sources orthogonal to each other and creating a potential  of learning from both. 
% Following the aforementioned intuition, we investigate \textbf{RQ3.2 What if we combine multiple orthogonal sources of data?}



% \noindent \textbf{Experiment 3.2}~ In this experiment, for each patch we collected from Chromium and Debian issue tracker, we also collect the before and after version of the changed function, and created \realdata-v2; this is horizontal \realdata(\realdatah)-while previous version of \realdata is the vertical \realdata(\realdatav). Since, Devign data does not provide vertical information about their dataset, we are unable to perform this experiment on Devign dataset. Nevertheless, we conducted two different experiments in this investigation. First, we trained two different models based on the \realdatah and \realdatav. We predict a code as vulnerable using two different settings \ie i. both the models say it is vulnerable ii. at least one model says it is vulnerable. In the second experiment, we take the balanced version of \realdatah as described in RQ3.1 and merge it with \realdatav and trained a unified model to predict. 

% \begin{table}[!htb]
%     \centering
%     \caption{\vp performance when orthogonal sources are combined in \realdata.}
%     \footnotesize
%     \begin{tabular}{l|l|c|c}
%     \toprule
%     \textbf{Model Types} & \textbf{Data Source} & \textbf{Accuracy} & \textbf{F1}\\
%     \midrule
%     \multirow{5}{*}{Separate} & \realdatah & 80.43 & 35.89\\
%     \cmidrule{2-4}
%      & \realdatav & 31.69 & 17.03\\
%      \cmidrule{2-4}
%     & \multicolumn{3}{l}{\realdatav, \realdatah}\\
%     & {~~~~~~~~i. Both predicts vuln.} & 83.30 & 36.59\\
%     & {~~~~~~~~ii. At least one predicts vuln.} & 31.15 & 18.36\\
%     \midrule
%     Unified & \realdatah + \realdatav & \red{\textbf{85.49}} & \red{\textbf{49.12}}\\
%     \bottomrule
%     \end{tabular}
%     \label{tab:v1_v2}
% \end{table}
% \noindent \textbf{Result 3.2} Table~\ref{tab:v1_v2} shows the performance of combining orthogonal source of information in \realdata (\ie \realdatah and \realdatav). As we can see, if we train separate models, the performance does not increase significantly.  However, a unified model trained on combination of both the sources of data improves the performance significantly. In such settings, the f1 is increased to 49.12 in contrast to the \realdatah f1 score 35.89 resulting in a 36.86\% performance gain. This is reasonable, since from a combined dataset the model is learning to discriminate a vulnerable function both from other non-vulnerable function from its context and also from the fine grained changes from the changed version of the function with no vulnerability. 

% \noindent\textbf{Observation 3.2} Combining multiple orthogonal source of information leads a model to better learn fine grained patterns of vulnerability. 

==> RQ_details/rq4.tex <==
% !TEX root = ../fse_results.tex

\subsection{RQ4}
\label{sec:rq4}

\textbf{Question : Does semantic information in code help improve the performance of Vulnerability Detection model? (RQ4)}

\begin{table*}[!htb]
    \centering
    \footnotesize
    \caption{\textbf{\small Influence of Semantic information on vulnerability prediction.}}
    \begin{tabular}{c|c|c|c}
    \toprule
    Method & Dataset & Accuracy & F1\\
    \midrule
    \multirow{2}{*}{Only Graph (without GGNN) + MLP} & Neurips data & 60.85 & 54.46\\
    & Chrome and Debian data & 88.57 & 16.46\\
    \midrule
    \multirow{2}{*}{Graph with GGNN} &  Neurips data & 62.56 & 61.61\\
    & Chrome and Debian data & 87.66 & 25.97\\
    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table*}

%  Neurips with artificial imbalance 59.83 & 23.76.


\begin{table}[!htb]
\centering
\footnotesize
\caption{\textbf{\small Graph classification without the GGNN (Chrome and Debian data).}}
\begin{tabular}{lcccc}
\toprule
Settings             & Acccuracy & Precision & Recall & F1    \\
\toprule
Imbalanced Setting   & \Red{88.57}     & 21.59     & 13.48  & 16.46 \\
\midrule
SMOTE                & 79.55     & 20.89     & 50.86  & 29.61 \\
\toprule
Complete Undersample & 63.51     & 16.1      & \Red{78.15}  & 26.67 \\
\midrule
2 times oversample                   & 73.56     & 19.54     & 67.92  & 30.31 \\
\midrule
3 times oversample                   & 76.22     & 20.69     & 63.77  & 31.24 \\
\midrule
4 times oversample                   & 76.92     & 21.3      & 63.96  & 31.96 \\
\midrule
5 times oversample                   & 77.87     & 21.74     & 61.85  & \Red{32.16} \\
\midrule
6 times oversample                   & 78.5      & 21.66     & 58.85  & 31.67 \\
\midrule
7 times oversample                   & 78.38     & 21.76     & 59.87  & 31.91 \\
\midrule
8 times oversample                   & 79.36     & 21.9      & 55.91  & 31.46 \\
\midrule
9 times oversample                   & 79.51     & \Red{22.07}     & 56.23  & 31.69 \\
\midrule
Full Oversample      & 79.22     & 21.69     & 55.59  & 31.2 \\
\bottomrule
\end{tabular}
\end{table}


==> RQ_details/rq5.tex <==
% !TEX root = ../fse_results.tex

\subsection{RQ5}
\label{sec:rq5}
\robin{Please put the result that you got with artificial imbalance.}

==> RQ_details/rq6.tex <==
% !TEX root = ../fse_results.tex

\subsection{RQ6}
\label{sec:rq6}

\begin{table}[!htb]
\centering
\footnotesize
\caption{\textbf{\small Chrome and Debian data with GGNN and sampling.} RQ6}
\begin{tabular}{lcccc}
\toprule
\textbf{}            & Accuracy & Precision & Recall & F1    \\
\midrule
Complete Undersample & 72.83    & 20.26     & \Red{74.96}  & 31.87 \\
\midrule
2 times oversample                  & 75.46    & 21.72     & 72.79  & 33.43 \\
\midrule
3 times oversample                   & 77.18    & 22.78     & 70.5   & 34.39 \\
\midrule
4 times oversample                   & 78.76    & 23.94     & 68.91  & 35.5  \\
\midrule
5 times oversample                  & 78.27    & 23.32     & 68.05  & 34.68 \\
\midrule
6 times oversample                  & 78.54    & 23.64     & 68.22  & 35.05 \\
\midrule
7 times oversample                  & 79.38    & 23.94     & 65.47  & 35.01 \\
\midrule
8 times oversample                  & \Red{80.43}    & \Red{25.13}     & 64.5   & \Red{35.89} \\
\midrule
9 times oversample                  & 80.13    & 24.86     & 64.45  & 35.49 \\
\midrule
Full Oversample      & 79.26    & 24.19     & 66.54  & 35.36\\
\bottomrule
\end{tabular}
\end{table}

==> Tables/approaches.tex <==
\begin{table*}[!htpb]
    \centering
    \footnotesize
    \caption{\small \textbf{Summary for vulnerability detection deep learning papers that are included as baseline.}}
    \label{tab:paper_sum}
    \begin{tabular}{llcrr}
        \toprule
        \textbf{Approach} & \textbf{Data Source}  & \textbf{Token Representation} & \textbf{Granularity} & \textbf{Model}\\ 
        \toprule
        Russell et al. \cite{russell2018automated}   & Juliet, Github, Debian Kernel & Abstract & Full function    & CNN+RF  \\
        VulDeePecker \cite{li2018vuldeepecker}    & Juliet, Open Source Projects   & Symbolic     & Backward slice(intra function) & BLSTM \\
        SySeVR \cite{li2018sysevr}    & Juliet, Open Source Projects    & Symbolic     & Both Forward and Backward slice & BGRU\\
        Devign~\cite{zhou2019devign} & Devign (5 real world projects) & Original token & Function Graph & GGNN\\
        \bottomrule
    \end{tabular}
\end{table*}


==> Tables/balance_exp.tex <==
% ! TEX root = ../RQ_Details/rq3.tex

\begin{table}[!htb]
    \centering
    \caption{\small{\textbf{Effect of various degree of data balancing for \vp.}}}
    \footnotesize
    % \begin{tabular}{l|c|c|c|c|c}
    % \hlineB{2}
    %      \textbf{Settings} & $k$ & \textbf{Accuracy} & \textbf{Precision} & \textbf{Recall} & \textbf{F1 score}\bigstrut\\
    %      \hlineB{1}
    %      Imbalanced & -  & 87.66 & 26.49 & 25.48 & 25.97\bigstrut\\
    %      \hlineB{1}
    %      \multirow{10}{*}{Balanced} & 1 & 72.83 & 20.26 & 74.96 & 31.87 \bigstrut\\
    %         \cline{2-6}
    %         & 2 & 75.46 & 21.72 & 72.79 & 33.43 \bigstrut\\
    %         \cline{2-6}
    %         & 3 & 77.18 & 22.78 & 70.50 & 34.39 \bigstrut\\
    %         \cline{2-6}
    %         & 4 & 78.76 & 23.94 & 68.91 & 35.50 \bigstrut\\
    %         \cline{2-6}
    %         & 5 & 78.27 & 23.32 & 68.05 & 34.68 \bigstrut\\
    %         \cline{2-6}
    %         & 6 & 78.54 & 23.64 & 68.22 & 35.05 \bigstrut\\
    %         \cline{2-6}
    %         & 7 & 79.38 & 23.94 & 65.47 & 35.01 \bigstrut\\
    %         \cline{2-6}
    %         & 8 & 80.43 & 25.13 & 64.50 & 35.89 \bigstrut\\
    %         \cline{2-6}
    %         & 9 & 80.13 & 24.86 & 64.45 & 35.49 \bigstrut\\
    %         \cline{2-6}
    %         & 10& 79.26 & 24.19 & 66.54 & 35.36 \bigstrut\\
    %       \hlineB{2}
    % \end{tabular}
    % \\
    % $k$ = Number of time vulnerable examples are replicated as described in Section~\ref{sec3:models}. 
    
\begin{tabular}
{l|l|rrrc}
\hline
\textbf{Rank} & \textbf{Settings} & k & \textbf{Median} & \textbf{IQR} & \bigstrut\\
\hline
%   1 &   \multirow{9}{*}{Balanced} & 8 &    0.36  &  0.03 & \quart{53}{20}{66}{66487} \\
%   1 &    & 4 &    0.36  &  0.03 & \quart{53}{20}{66}{66487} \\
%   1 &    & 9 &    0.36  &  0.04 & \quart{53}{26}{66}{66487} \\
%   1 &   & 10 &    0.35  &  0.03 & \quart{53}{20}{59}{66487} \\
%   1 &    & 6 &    0.35  &  0.02 & \quart{53}{13}{59}{66487} \\
%   1 &    & 5 &    0.35  &  0.02 & \quart{53}{13}{59}{66487} \\
%   1 &    & 7 &    0.34  &  0.04 & \quart{46}{27}{53}{66487} \\
%   1 &    & 3 &    0.34  &  0.01 & \quart{53}{6}{53}{66487} \\
%   1 &    & 2 &    0.34  &  0.01 & \quart{46}{7}{53}{66487} \\

  1 &       \multirow{9}{*}{Balanced}     & 8 &    35.97  &  2.53 & \quart{56}{18}{67}{499} \\
  1 &           & 4 &    35.86  &  2.95 & \quart{56}{20}{66}{499} \\
  1 &           & 9 &    35.8  &  4.04 & \quart{52}{27}{66}{499} \\
  1 &           & 10 &    35.28  &  3.19 & \quart{51}{21}{63}{499} \\
\cline{3-6}
 2 &           & 6 &    34.8  &  2.44 & \quart{53}{16}{59}{499} \\
  2 &           & 5 &    34.79  &  2.47 & \quart{51}{17}{59}{499} \\
  2 &           & 7 &    34.22  &  3.65 & \quart{49}{25}{55}{499} \\
\cline{3-6}
 3 &           & 3 &    34.17  &  1.47 & \quart{52}{9}{55}{499} \\
  3 &           & 2 &    33.51  &  1.61 & \quart{46}{11}{51}{499} \\
\cline{3-6}
 4 &           & 1 &    31.67  &  1.27 & \quart{36}{8}{38}{499} \\
\hline
 5 &  Imbalanced & - &    25.94  &  0.03 & \quart{0}{0}{0}{499} \bigstrut \\
\hline
\end{tabular}
    \label{tab:balance_exp}
\end{table}

==> Tables/challenge.tex <==
% Table generated by Excel2LaTeX from sheet 'Sheet1'
\begin{table*}[htbp]
\footnotesize
  \centering
  \caption{Add caption}
    \begin{tabular}{r|p{10em}|p{17.335em}|p{13.085em}|p{17.085em}}
    \toprule
    \textbf{Dataset} & \textbf{Problem} & \textbf{Description} & \textbf{Impact} & \textbf{Remedy} \\
    \midrule
    \multicolumn{1}{|r|}{\multirow{3}[6]{*}{Synthetic Data}} & Selection Bias & Based on the different distribution of bug categories in synthetic datasets, the selected samples have bias on some specific kinds of bugs. & \multirow{2}[4]{*}{Model may overfit to some specific kinds of bugs or corresponding datasets, and failed to generalize across datasets.} & \multirow{2}[4]{*}{Use Real world Data\newline{}- Chrome\newline{}- Debian\newline{}- Neurips Data\newline{}\newline{}Ensemble Learning} \\
\cmidrule{2-3}          & Capture Bias\newline{}- Repetition bias\newline{}- Contextual bias & The trivial contextual structure and replications exist in synthetic dataset & \multicolumn{1}{r|}{} & \multicolumn{1}{r|}{} \\
\cmidrule{2-5}          & Ensemble Learning (TBD) & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} & \multicolumn{1}{l|}{} \\
    \midrule
    \multicolumn{1}{|r|}{\multirow{3}[6]{*}{Real World Data}} & Models are simple & Token-based models tend to ignore the semantic information of code (e.g. CFG, DFG) & Low precision/recall & Capture the semantic information by GGNN (neurips paper have shown some promising results) \\
\cmidrule{2-5}          & Unreal distribution of data & the unbalanced distribution of vulnerable/non-vulnerable code makes GNN fail to capture the ÒrealÓ semantic information & Still low precision/recall & Make the training dataset balanced by undersampling and oversampling \\
\cmidrule{2-5}          & How to balance the data & The dataset can be balanced in different ways (i.e. different ratio of undersample / oversample) & Different balanced data will lead to the varied performances & Search for the best-performing undersample/oversample ratio \\
    \bottomrule
    \end{tabular}%
  \label{tab:addlabel}%
\end{table*}%

==> Tables/cross-dataset.tex <==
% !TEX root = ../RQ_details/rq1.tex

% \begin{table}[!htb]

% \caption{\small{\textbf{Cross-dataset generalization experiment results.} 
% % The column ``Self'' denotes the test result evaluated on the same train dataset, and the column ``Other'' denotes the average value evaluated on the datasets other than the training dataset 
% }}


% \footnotesize
% \begin{center}
% \begin{subtable}{0.5\textwidth}\centering
% \begin{tabular}{l|llll|ll}
% \toprule
% Pretrained models$\backslash$Test dataset    & Juliet & Vul & SySe  & G + D  & Self & Other   \\ \midrule
% Juliet  & 87/87 &  44/44   & 40/27 & 30/12 & 87/87  &  38/28  \\ %\hline
% Vul     & 52/25 &  90/82   & 68/26 & 77/11 & 90/82  &  66/21 \\ 
% SySe    & 60/41 &  69/41   & 97/89 & 89/ 9  & 97/89  &  73/30   \\ 
% G + D   & 50/23 &  63/33   & 76/22 & 92/34 & 92/34  &  63/26   \\ 
% \bottomrule
% \end{tabular}
% \caption{\small{\bf CNN+RF Model Results (Accuracy/F1-score)}}
% \end{subtable}

% \begin{subtable}{0.5\textwidth}\centering
% \begin{tabular}{l|llll|ll}
% \toprule
% Train$\backslash$Test    & Juliet & Vul & SySe  & G + D  & Self & Other   \\ \midrule
% Juliet  & 88/90 & 37/47 & 25/24 & 11/12 & 88/90 & 24/28  \\ 
% Vul     & 55/43 & 89/83 & 37/23 & 50/14 & 89/83 & 47/27 \\ 
% SySe    & 64/51 & 68/56 & 97/90 & 92/11 & 97/90 & 75/39   \\ 
% G + D   & 54/38 & 55/40 & 66/26 & 93/54 & 93/54 &  58/35   \\ 
% \bottomrule
% \end{tabular}
% \caption{\small{\bf CNN Model Results (Accuracy/F1-score)}}
% \end{subtable}

% \begin{subtable}{0.5\textwidth}\centering
% \begin{tabular}{l|llll|ll}
% \toprule
% Train$\backslash$Test    & Juliet & Vul & SySe  & G + D  & Self & Other   \\ \midrule
% Juliet     & 89/90 &  30/44  & 32/27 & 13/12 & 89/90 & 25/28   \\ 
% Vul        & 49/30 &  91/85  & 31/22 & 40/13 & 90/84 & 40/22 \\ 
% SySe       & 62/64 &  55/47  & 96/88 & 87/15 & 88/64 & 68/42   \\ 
% G + D      & 51/39 &  60/40  & 74/35 & 92/48 & 91/46 & 62/38   \\ 
% \bottomrule
% \end{tabular}
% \caption{\small{\bf BGRU Model Results (Accuracy/F1-score)}}
% \end{subtable}

% \begin{subtable}{0.5\textwidth}\centering
% \begin{tabular}{l|llll|ll}
% \toprule
% Train$\backslash$Test    & Juliet & Vul & SySe  & G + D  & Self & Other   \\ \midrule
% Juliet        & 87/89 &  29/44    & 23/26  & 7 /12 &   87/89   &  20/27    \\ 
% Vul  & 46/27  &  88/82    & 27/19 & 27/12 &  88/82   &  33/19 \\ 
% SySe       & 61/68  &  62/49    & 97/89 & 78/15 & 97/89 &  67/44    \\ 
% G + D & 50/44 &  62/43    & 59/30  & 92/51 &  92/51  &  57/39    \\ 
% \bottomrule
% \end{tabular}
% \caption{\small{\bf BLSTM Model Results (Accuracy/F1-score)}}
% \end{subtable}
% \label{tab:cross}
% \end{center}
% \vspace{-4mm}
% \end{table}


\begin{table}[!htb]

\caption{\small{\textbf{Preformance of pretrained models on predicting vulnerabilities in the wild (accuracy/f1 score).}}}


\footnotesize
\begin{center}
\begin{subtable}{0.5\textwidth}\centering
\begin{tabular}{l|cccc}
\toprule
Train$\backslash$Test  & Juliet & VulDeePecker & SySeVR  & Github + Debian \\
\midrule
Juliet          & \Red{87/87} &  44/44   & 40/27 & 30/12 \\ %\hline
VulDeePecker    & 52/25 &  \Red{90/82}   & 68/26 & 77/11 \\ 
SySeVR          & 60/41 &  69/41   & \Red{97/89} & 89/ 9 \\ 
Github + Debian & 50/23 &  63/33   & 76/22 & \Red{92/34} \\ 
\bottomrule
\end{tabular}
\caption{\small{\bf CNN+RF Model Results. 
% (Accuracy/F1-score)
}}
\label{tab:cross_cnnrf}
\end{subtable}

\begin{subtable}{0.5\textwidth}\centering
\begin{tabular}{l|cccc}
\toprule
Train$\backslash$Test  & Juliet & VulDeePecker & SySeVR  & Github + Debian \\ 
\midrule
Juliet          & \Red{88/90} & 37/47 & 25/24 & 11/12 \\ 
VulDeePecker    & 55/43 & \Red{89/83} & 37/23 & 50/14 \\ 
SySeVR          & 64/51 & 68/56 & \Red{97/90} & 92/11 \\ 
Github + Debian & 54/38 & 55/40 & 66/26 & \Red{93/54} \\ 
\bottomrule
\end{tabular}
\caption{\small{\bf CNN Model Results. 
% (Accuracy/F1-score)
}}
\label{tab:cross_cnn}
\end{subtable}

\begin{subtable}{0.5\textwidth}\centering
\begin{tabular}{l|cccc}
\toprule
Train$\backslash$Test  & Juliet & VulDeePecker & SySeVR  & Github + Debian \\
\midrule
Juliet          & \Red{89/90} &  30/44  & 32/27 & 13/12 \\ 
VulDeePecker    & 49/30 &  \Red{91/85}  & 31/22 & 40/13 \\ 
SySeVR          & 62/64 &  55/47  & \Red{96/88} & 87/15 \\ 
Github + Debian & 51/39 &  60/40  & 74/35 & \Red{92/48} \\ 
\bottomrule
\end{tabular}
\caption{\small{\bf BGRU Model Results. 
% (Accuracy/F1-score)
}}
\label{tab:cross_blstm}
\end{subtable}

\begin{subtable}{0.5\textwidth}\centering
\begin{tabular}{l|cccc}
\toprule
Train$\backslash$Test  & Juliet & VulDeePecker & SySeVR  & Github + Debian \\
\midrule
Juliet          & \Red{87/89} & 29/44 & 23/26 & 7 /12 \\ 
VulDeePecker    & 46/27 & \Red{88/82} & 27/19 & 27/12 \\ 
SySeVR          & 61/68 & 62/49 & \Red{97/89} & 78/15 \\ 
Github + Debian & 50/44 & 62/43 & 59/30 & \Red{92/51}\\ 
\bottomrule
\end{tabular}
\caption{\small{\bf BLSTM Model Results.
% (Accuracy/F1-score)
}}
\label{tab:cross_bgru}
\end{subtable}

\begin{subtable}{0.5\textwidth}\centering
\begin{tabular}{l|cccc}
\toprule
Settings$\backslash$Test dataset  & Juliet & VulDeePecker & SySeVR  & Github + Debian \\
\midrule
Emsemble    & 55/41    & 53/44 & 47/27 & 50/12\\
\bottomrule
\end{tabular}
\caption{\small{\bf Results from ensemble of all available models.}}
\label{tab:cross_ensemble}
\end{subtable}
\label{tab:cross}
\end{center}
\vspace{-4mm}
\end{table}

==> Tables/dataset.tex <==
% \begin{table}[!htpb]
% \centering
% \caption{\small \textbf{List of Existing Baseline Datasets}}
% \begin{tabular}{lr}
% \toprule
% \textbf{Primary Dataset Content} &  \textbf{Number of Samples} \\ 
% \midrule 
% SATE IV Juliet \cite{okun2013report}   & 192,146 \\
% VulDeePecker CWE 119     \cite{li2018vuldeepecker}   &  39,753  \\
% VulDeePecker CWE 399    \cite{li2018vuldeepecker}   & 21,885 \\
% SySeVR API Call      \cite{li2018sysevr}  & 64,403  \\
% SySeVR Arithmetic Expr    \cite{li2018sysevr} & 22,154 \\ 
% SySeVR Array Usage     \cite{li2018sysevr}  & 42,229 \\ 
% SySeVR Pointer Usage    \cite{li2018sysevr}  & 291,841 \\ 
% Github + Debian   \cite{russell2018automated}   & 1,274,366 \\ 
% \bottomrule
% \end{tabular}
% \label{tab:number_samples}
% \end{table}

\begin{table}[!htpb]
\footnotesize
\centering
\caption{\small \textbf{Details about different datasets investigated in this study.}}
\begin{tabular}{llcr}
\toprule
\textbf{Dataset } & \textbf{Sub-Category} &\textbf{Sample\#} & \textbf{Type}\\ 
\midrule 
SATE IV Juliet~\cite{okun2013report} (Jul)  & N/A & 202,462 & Synthetic\\
\midrule
\multirow{ 2}{*}{VulDeePecker~\cite{li2018vuldeepecker}} & CWE 119   &  39,753  & \multirow{ 2}{*}{Semi-Synthetic}\\
 & CWE 399      & 21,885 &\\
\midrule
\multirow{4}{*}{SySeVR~\cite{li2018sysevr}} & API Call  & 64,403  & \multirow{4}{*}{Semi-Synthetic}\\
 & Arithmetic Expr   & 22,154 & \\ 
 & Array Usage    & 42,229 &\\ 
 & Pointer Usage    & 291,841 &\\ 
\midrule
Github + Debian~\cite{russell2018automated}  & N/A  & 1,274,366 & Semi-Real\\ 
\midrule
FFMpeg + QEMU~\cite{zhou2019devign} (Devign)& N/A & 22155 & Real\\
\midrule
\multirow{2}{*}{Chromium + Debian} & Vertical & 18466 & \multirow{2}{*}{Real}\\
&  Horizontal & 2569 & \\ 
\bottomrule
\end{tabular}
\label{tab:dataset_num_samples}
\end{table}

==> Tables/learned_features.tex <==
\begin{table}[!htb]
\caption{\small{\textbf{Top features from different datasets that is learned by CNN model.}}}
\centering
\footnotesize

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{3cm}|c|c}
\toprule
\textbf{Feature}        & \textbf{Mean Activation}              & \textbf{Prevalence}   \\ 
\midrule
IDENT ( *                   & 5.56  & 0.65 \\
VARIABLE *            & 5.38  & 0.42 \\
\{ IDENT ( *                & 5.32 & 0.63 \\
\{ IDENT * VARIABLE ; & 5.24  & 0.59  \\
) \{ IDENT * VARIABLE & 5.17  & 0.59 \\
\bottomrule
\end{tabular}
\caption{\small{Top vulnerability-related features in SATE IV Juliet~\cite{okun2013report}.}}
\end{subtable}

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{3cm}|c|c}
\toprule
\textbf{Feature}        & \textbf{Mean Activation}              & \textbf{Prevalence}               \\
\midrule
5                              & 5.38 & 0.97 \\
{[} 5                          & 4.84 & 0.86  \\
\{ IDENT                       & 4.80 & 0.73 \\
- LITERAL ;                    & 4.64 & 12.75  \\
FUNC ( DEC , LITERAL       & 4.57 & 1.10 \\ 
\bottomrule
\end{tabular}
\caption{\small{Top vulnerability-related features in VulDeePecker~\cite{li2018vuldeepecker}.}}
\end{subtable}

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{3cm}|c|c}
\toprule
\textbf{Feature}        & \textbf{Mean Activation}              & \textbf{Prevalence}               \\ 
\midrule
NULL ; VARIABLE      & 5.14  & 1.22 \\
$>$ strlen        & 5.10  & 2.08  \\
VARIABLE -           & 4.88  & 0.18 \\
, IDENT $|$                  & 4.66  & 2.01 \\
int VARIABLE = IDENT & 4.66  & 0.70 \\
\bottomrule
\end{tabular}
\caption{\small{Top vulnerability-related features in SySeVR~\cite{li2018sysevr}.}}
\end{subtable}

\begin{subtable}{\linewidth}
\centering
\begin{tabular}{p{3cm}|c|c}
\toprule
\textbf{Feature}        & \textbf{Mean Activation}              & \textbf{Prevalence}               \\ 
\midrule
fopen   & 6.69 & 17.61 \\
malloc  & 6.02 & 7.20  \\
fopen ( & 5.22 & 17.64 \\
memcpy  & 4.99 & 10.62 \\
read    & 4.82 & 4.49  \\
\bottomrule
\end{tabular}
\caption{\small{Top vulnerability-related features in Github + Debian~\cite{russell2018automated}.}}
\end{subtable}
\label{tab:feature}
\vspace{-4mm}
\end{table}

==> Tables/lemna_example_1_integer_overflow.tex <==
\begin{subfigure}{0.95\linewidth}
\scriptsize
\tt
\begin{tabular}{|r p{0.89\linewidth}|}
\hline
1 & \lone{\textbf{void} CWE190\_Integer\_Overflow\_Unsigned\_int...()}\\
2 & ~~~~\ltwo{\textbf{unsigned int} data ;}\\
3 & ~~~~\ltwo{data = 0 ;}\\
4 & ~~~~\lfive{badSink ( data ) ;}\\
5 & \lfive{\textbf{static void} badSink ( \textbf{unsigned int} data )}\\
6 & ~~~~\lfive{\textbf{if} ( badStatic )}\\
7 & ~~~~~~~~\lfive{\textbf{unsigned int} result = data * }\lthree{data ;}\\
8 & ~~~~~~~~\lthree{printUnsignedLine ( result );}\\
9 & \lthree{\textbf{void} printUnsignedLine(unsigned unsignedNumber)}\\
10 & ~~~~\lthree{printf ( "\%u$\backslash$n" , unsignedNumber ); }\\
\hline
\end{tabular}
\caption{\textbf{\small Integer Overflow vulnerability (CWE-190).}}
\label{fig:lemna_int_overflow}
\end{subfigure}


==> Tables/lemna_example_2_memory_overflow.tex <==
\begin{subfigure}{0.95\linewidth}
\scriptsize
\tt
\begin{tabular}{|rp{0.89\linewidth}|}
\hline
1 & \lone{\textbf{void} CWE789\_Uncontrolled\_Mem\_Alloc...()}\\
2 & ~~~~\ltwo{\textbf{size\_t} data ;}\\
3 & ~~~~\ltwo{data = 0;}\\
4 & ~~~~\lfour{\textbf{if} ( staticFive == 5 )}\\
5 & ~~~~~~~~\lfour{data = rand ( );}\\
6 & ~~~~\lfour{\textbf{if} ( staticFive == 5 )}\\
7 & ~~~~~~~~\lfour{\textbf{char *} myString ;}\\
8 & ~~~~~~~~\lfour{\textbf{if} ( data > strlen ( HELLO\_STRING ) )}\\
9 & ~~~~~~~~~~~\lfour{myString = (\textbf{char *})malloc( }\\
10 & ~~~~~~~~~~~~~~~~~~~~~~~~\lfour{data * }\lthree{\textbf{sizeof}(char));}\\
11 & ~~~~~~~~~~~\lthree{strcpy ( myString , HELLO\_STRING );}\\
12 & ~~~~~~~~~~~\lthree{printLine ( myString );}\\
13 & \lthree{\textbf{void} printLine (\textbf{const char *} line)}\\
14 & ~~~~\lthree{\textbf{if} ( line != NULL )}\\
15 & ~~~~~~~~\lthree{printf ( "\%s$\backslash$n" , }\lfive{line );}\\
16 & ~~~~\lfive{free ( myString );}\\
\hline
\end{tabular}
\caption{\textbf{\small Uncontrolled Memory vulnerability (CWE-789).}}
\label{fig:lemna_memory_overflow}
\end{subfigure}


==> Tables/lemna_example_3_draper_G_D.tex <==
\begin{subfigure}{0.95\linewidth}
\scriptsize
\tt
\begin{tabular}{|r p{0.89\linewidth}|}
\hline
1  & \ltwo{link\_layer\_show(\textbf{struct} ib\_port \textbf{*}p, } \\
2  & ~~~~~~~\lone{\textbf{struct} port\_attribute \textbf{*}unused, \textbf{char *} buf)\{}\\
3  & ~~~\lone{\textbf{switch} }\lthree{(rdma\_port\_get\_link\_layer(}\\
4  & ~~~~~~~~~~~~~~~\lthree{p->ibdev, p->port\_num))}\lfive{ \{}\\
5  & ~~~~~~\lfive{\textbf{case} }\lfour{IB\_LINK\_LAYER\_INFINIBAND:}\\
6  & ~~~~~~~~~\lfour{\textbf{return} sprintf(buf, "\%s$\backslash$n", "InfiniBand");}\\
7  & ~~~~~~\lfive{\textbf{case} IB\_LINK\_LAYER\_ETHERNET:}\\
8  & ~~~~~~~~~\lfive{\textbf{return} sprintf(buf, "\%s$\backslash$n", "Ethernet");}\\
9  & ~~~~~~\lfive{\textbf{default}:}\\
10 & ~~~~~~~~~\lfive{\textbf{return} sprintf(buf, "\%s$\backslash$n", "Unknown");}\\
11 & ~~~\lfive{\}}\\
12 & \lfive{\}}\\
\hline
\end{tabular}
\caption{\textbf{\small Vulnerable code example in \draper \cite{russell2018automated} dataset.}}
\label{fig:lemna_draper}
\end{subfigure}


==> Tables/rq2_comparison.tex <==
\begin{table*}[!htb]
    \centering
    \caption{\small Relative ordering of the approaches based on F1 score using ScottKnott statistical ordering. Different approaches with the same rank indicate that they are not significantly better than each other.  KNN refers to K-Nearest Neighbor based classifier, LR refers to Logistic regression classifier, SVM referes to Support Vector Machine. Column IQR shows the Inter Quartile Range of the F1 score from different runs of an experiment. Low IQR indicates low variability in performance \ie stability of the approach.}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \footnotesize
        \begin{tabular}{llrrc}
        \hlineB{2}
        \textbf{Rank} & \textbf{Approach} & \textbf{Median} & \textbf{IQR} & \textbf{Range}\bigstrut\\
        \hlineB{2}
        1 & GGNN & 35.97 & 2.53 & \quart{71}{9}{74}{237} \bigstrut\\
        \hlineB{1}
        2 & KNN & 18.53 & 4.3 & \quart{41}{5}{43}{237} \bigstrut\\
        2 & Russel~\etal & 19.97  & 1.75 & \quart{35}{4}{37}{237} \bigstrut\\
        \hlineB{1}
        3 & SVM & 14.48 & 5.85 & \quart{13}{15}{23}{237} \bigstrut\\
        \hlineB{1}
        4 & LR & 7.4 & 3.82 & \quart{0}{9}{6}{237} \bigstrut\\
        \hlineB{2}
        \end{tabular}
        % \vspace{-2mm}
        \caption{\small Different approaches on \realdata}
        \label{table:comparison_chrome_deb_f1}
    \end{subfigure}
    \begin{subfigure}{0.49\textwidth}
        \centering
        \footnotesize
        \begin{tabular}{llrrc}
        \hlineB{2}
        \textbf{Rank} & \textbf{Approach} & \textbf{Median} & \textbf{IQR} & \textbf{Range}\bigstrut\\
        \hlineB{2}
        
        1 &  GGNN &  60.29  &  3.2 & \quart{68}{11}{75}{215} \bigstrut\\
        \hlineB{1}
        2 &  KNN &  54.88 &  0.66 & \quart{55}{2}{56}{215} \bigstrut\\
        \hlineB{1}
        3 & Russel~\etal & 44.79 & 1.77 & \quart{18}{6}{20}{215} \bigstrut\\
        3 & SVM & 43.5  &  6.15 & \quart{0}{21}{16}{215} \bigstrut\\
        3 & LR & 42.33  &  1.94 & \quart{9}{7}{12}{215} \bigstrut\\
        \hlineB{2}
        \end{tabular}
        % \vspace{-2mm}
        \caption{\small Different approaches on \devigndata}
        \label{table:comparison_devign_f1}
    \end{subfigure}
    \label{tab:statistical_comparison}
\end{table*}

==> Tables/rq2_problems.tex <==
% ! TEX root = ../RQ_Details/rq2.tex

% \begin{table*}[!htb]
%     \centering
%     \caption{\small{\textbf{Existing approaches' performance on real world datasets (accuracy/f1-score).}}}
%     \footnotesize
%     \begin{tabular}{p{0.20\linewidth}|p{0.25\linewidth}|p{0.18\linewidth}|p{0.23\linewidth}}
%     \toprule
%     Approach     &   Data processing  &   Dataset   & Accuracy/F1\\
%     \midrule
%     \midrule
%     \multirow{3}{=}{Deep Learning (CNN)} & Symbolic Tokenization & Devign & xx.xx / xx.xx\\
%     \cline{3-4}
%     &  & \realdata & xx.xx / xx.xx\\
%     \midrule
%     \multirow{7}{=}{Traditional Machine Learning (SVM)} & \multirow{3}{=}{Original Token with Word2Vec initialization} & Devign & xx.xx / xx.xx\\
%     \cline{3-4}
%     & & \realdata & xx.xx / xx.xx\\
%     &&&\\
%     \cline{2-4}
%      & \multirow{2}{=}{AST node type only} & Devign & xx.xx / xx.xx\\
%     \cline{3-4}
%     & & \realdata & xx.xx / xx.xx\\
%     \cline{2-4}
%      & \multirow{3}{=}{Both the AST node type and Word2Vec token embeddings} & Devign & xx.xx / xx.xx\\
%     \cline{3-4}
%     & & \realdata & xx.xx / xx.xx\\
%     &&& \\
%     \midrule
%     \multirow{3}{=}{Graph Based Neural Networks} & \multirow{3}{=}{Both the AST node type and Word2Vec token embeddings} & Devign & xx.xx / xx.xx\\
%     \cline{3-4}
%     & & \realdata & xx.xx / xx.xx\\
%     & & &\\
%     \bottomrule
%     \end{tabular}
    
%     \label{tab:token_real_world}
% \end{table*}

% \begin{table}[!htb]
%     \centering
%     \caption{\small{\textbf{Comparative analysis of different aspect of different approaches.}}}
%     \footnotesize
%     \begin{tabular}{p{0.20\linewidth}|c|c|c|c|c}
%          \toprule
%          \textbf{Approach} & \textbf{Token} & \textbf{AST}  & \textbf{Dataset} & \textbf{Accuracy} & \textbf{F1} \\
%          & \textbf{Repr.} & \textbf{Node} & & & \textbf{score}\\
%          \midrule
%          \multirow{2}{=}{Deep Learning (CNN + RF)} & \multirow{2}{*}{Abstract} & \multirow{2}{*}{\xmark} & Devign & 54.65 & 45.71\\
%          \cline{4-6}
%         %  & & & \realdata & 89.83 & 8.78\\
%         & & & \realdata & 90.53 & 18.12\\
%          \midrule
%          \multirow{6}{=}{Traditional Machine Learning (SVM)}  & \multirow{2}{*}{N/A} & \multirow{2}{*}{\cmark} & Devign & 54.00 & 27.76\\
%          \cline{4-6}
%          & & & \realdata & 91.44 & 3.83\\
%          \cline{2-6}
%          & \multirow{2}{*}{Word2Vec} & \multirow{2}{*}{\xmark} & Devign & 58.53 & 53.18\\
%          \cline{4-6}
%          & & & \realdata & 83.46 & 16.55\\
%          \cline{2-6}
%          & \multirow{2}{*}{Word2Vec} & \multirow{2}{*}{\cmark} & Devign & 60.30 & 54.27\\
%          \cline{4-6}
%          & & & \realdata & 79.39 & 17.01\\
%          \midrule
%          \multirow{2}{=}{Graph Neural Network} & \multirow{2}{*}{Word2Vec} & \multirow{2}{*}{\cmark} & Devign & \red{\textbf{62.56}} & \red{\textbf{61.61}}\\
%          \cline{4-6}
%          & & & \realdata & \red{\textbf{87.66}} & \red{\textbf{25.97}}\\
%          \bottomrule
%     \end{tabular}
%     \label{tab:rq2_table}
% \end{table}


% \begin{table*}[!htpb]
%     \centering
%     \footnotesize
%     \caption{\realdata}
%     \begin{tabular}{l|l|r|r|r|r|r}
%         \hlineB{2}
%         \textbf{Approach} & \multirow{2}{*}{\textbf{Approach}} & \textbf{\% samples} & \multirow{2}{*}{\textbf{Accuracy}} & \multirow{2}{*}{\textbf{Precision}}  & \multirow{2}{*}{\textbf{Recall}} & \multirow{2}{*}{\textbf{F1-score}}\\
%         \textbf{Type} & & \textbf{in-scope} & & & \\
%         \hlineB{2}
%         \multirow{3}{*}{Token based} & VulDeePecker & 
%         21.46 & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx \bigstrut\\
%         \cline{2-7}
%         & SySeVR & 66.42 & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx \bigstrut\\
%         \cline{2-7}
%         & Russel~\etal & 100 & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx \bigstrut\\
%         \hlineB{1}
%         \multirow{3}{*}{Graph + ML} & SVM & 100 & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx \bigstrut\\
%         \cline{2-7}
%         & LR & 100 & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx \bigstrut\\
%         \cline{2-7}
%         & KNN & 100 & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx \bigstrut\\
%         \hlineB{1}
%         Graph + DL& GGNN & 100 & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx & xx.xx / xx.xx \bigstrut\\
%         \hlineB{1}
%     \end{tabular}
%     \label{tab:rq2_table_our_data}
% \end{table*}


%%%%%%% This results are in-scope result %%%%%%%%%%%%%%%%
\begin{table*}[!htpb]
    \centering
    \footnotesize
    \caption{\small Result of different approaches when trained on Real World Data (Median / IQR).}
    \begin{tabular}{@{}l|l|l|r|r|r|r|r}
        \hlineB{2}
        \textbf{Dataset} & \textbf{Approach} & \textbf{Approach Type} & \textbf{\% in-scope} & \textbf{Accuracy} & \textbf{Precision}  & \textbf{Recall} & \textbf{F1-score}\bigstrut\\
        \hlineB{2}
        \multirow{3}{*}{\realdata} & \multirow{1}{*}{Syntax Based} & 
		Russel~\etal & 100 & 91.34 / 0.60 & 27.72 / 1.79 & 15.53 / 2.00 & 19.97 / 1.75 \bigstrut\\
         \cline{2-8}
%       &&
% 		SVM & 100 & 87.06 / 3.23 & 13.37 / 3.93 & 16.43 / 11.78 & 14.48 / 5.85 \bigstrut\\
%       \cline{3-8}
%       && 	LR & 100 & 90.72 / 0.23 & 21.60 / 12.56 & 4.36 / 2.49 & 7.40 / 3.82 \bigstrut\\
% 	    \cline{3-8}
%       && 	KNN & 100 & 89.89 / 0.50 & 29.63 / 2.75 & 14.46 / 4.40 & 18.53 / 4.30 \bigstrut\\
%       \cline{2-8}
        &\multirow{2}{*}{Semantics Based} & 
		VulDeePecker & 21.46 & 81.49 / 1.57 & 39.33 / 4.20 & 55.92 / 11.47 & 45.06 / 4.89 \bigstrut\\
        \cline{3-8}
       \rowcolor{green!15} \cellcolor{white}{}& \cellcolor{white}{}& SySeVR & 66.42 & 87.29 / 1.98 & 60.03 / 6.91 & 68.03 / 10.20 & 63.97 / 6.94 \bigstrut\\	
        \cline{2-8}
      &\multirow{4}{*}{Graph Based} &   GGNN & 100 & 80.79 / 2.65 & 24.78 / 3.58 & 64.86 / 5.11 & 35.97 / 2.53 \bigstrut\\
      &&   GGNN (CFG) & 100 & 80.79 / 2.65 & 24.78 / 3.58 & 64.86 / 5.11 & 37.03 / 2.53 \bigstrut\\
      &&   GGNN (DFG) & 100 & 80.79 / 2.65 & 24.78 / 3.58 & 64.86 / 5.11 & 37.97 / 2.53 \bigstrut\\
      &&   GGNN (Both) & 100 & 80.79 / 2.65 & 24.78 / 3.58 & 64.86 / 5.11 & 36.82 / 2.53 \bigstrut\\
       \hlineB{2}
        \multirow{3}{*}{\devigndata} & \multirow{1}{*}{Syntax Based} & 
		Russel~\etal & 100 & 57.47 / 0.69 & 53.29 / 2.88 & 38.79 / 1.63 & 44.79 / 1.77 \bigstrut\\
        \cline{2-8}
        % &&
% 		SVM & 100 & 54.03 / 1.29 & 47.52 / 1.74 & 39.74 / 11.21 & 43.50 / 6.15 \bigstrut\\ 
%         \cline{3-8}
%         && 
% 		LR & 100 & 57.61 / 0.77 & 55.10 / 0.89 & 34.36 / 2.88 & 42.33 / 1.94 \bigstrut\\
%         \cline{3-8}
%         && 
% 		KNN & 100 & 60.80 / 0.51 & 56.01 / 0.76 & 53.76 / 1.11 & 54.88 / 0.66 \bigstrut\\	
		
        \cline{2-8}
        &\multirow{2}{*}{Semantics Based} & 
		VulDeePecker & 27.96 & 58.49 / 4.25 & 56.56 / 4.54 & 55.45 / 10.81 & 54.46 / 4.49 \bigstrut\\
        \cline{3-8}
       \rowcolor{green!15} \cellcolor{white}{}& \cellcolor{white}{}&  SySeVR & 84.08 & 68.02 / 2.35 & 64.68 / 0.99 & 78.29 / 1.10 & 70.96 / 1.03 \bigstrut\\
        \cline{2-8}
      &\multirow{4}{*}{Graph Based} &   GGNN & 100 & 62.86 / 3.08 & 56.96 / 4.73 & 65.36 / 3.78 & 60.29 / 3.20 \bigstrut\\
      &&   GGNN (CFG) & 100 & 80.79 / 2.65 & 24.78 / 3.58 & 64.86 / 5.11 & 55.30 / 2.53 \bigstrut\\
      &&   GGNN (DFG) & 100 & 80.79 / 2.65 & 24.78 / 3.58 & 64.86 / 5.11 & 55.97 / 2.53 \bigstrut\\
      &&   GGNN (Both) & 100 & 80.79 / 2.65 & 24.78 / 3.58 & 64.86 / 5.11 & 57.94 / 2.53 \bigstrut\\        \hlineB{2}
    \end{tabular}
    \label{tab:all_method_comparison_real_world_datasets}
\end{table*}

\begin{table}[!htb]
    \centering
    \footnotesize
    \caption{Comparisons of all available baselines in \realdata.  VulDeePecker$^1$ refers to VulDeePecker with one vote for Vulnerability, VulDeePecker$^m$ refers to VulDeePecker with majority vote for Vulnerability. Similar notation for SySeVR$^*$ in case of SySeVR.}
    \begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
        \hlineB{2}
        \textbf{Rank} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \bigstrut\\
        \hlineB{2}
          1 &    Repr+GGNN &    41.25  &  2.28 & \quart{74}{5}{77}{231} \bigstrut\\
        \hline
          2 & Repr-wo-GGNN &    38.97  &  2.0 & \quart{68}{5}{71}{231} \bigstrut\\
          2 &     GGNN-b &    38.63  &  0.83 & \quart{69}{2}{70}{231} \bigstrut\\
        \hline
          3 &     GGNN-i &    33.05  &  2.17 & \quart{53}{5}{55}{231} \bigstrut\\
        \hline
          4 &       SySeVR$^1$ &    30.25  &  2.35 & \quart{46}{6}{48}{231} \bigstrut\\
        \hline
          5 &       SySeVR$^m$ &    27.14  &  2.94 & \quart{37}{8}{40}{231} \bigstrut\\
        \hline
          6 &        VulDeePecker$^1$ &    15.7  &  6.41 & \quart{1}{17}{10}{231} \bigstrut\\
          6 & Russel et. al. &    15.24  &  2.74 & \quart{3}{7}{8}{231} \bigstrut\\
          6 &        VulDeePecker$^m$ &    14.58  &  5.41 & \quart{0}{14}{7}{231} \bigstrut\\
        \hlineB{2}
    \end{tabular}
   
    \label{tab:full_comparison_verum}
\end{table}


\begin{table}[!htb]
    \centering
    \footnotesize
    \caption{Comparisons of all available baselines in \devigndata (F-1 score).}
    \begin{tabular}{l@{~~~}l@{~~~}r@{~~~}r@{~~~}c}
        \hlineB{2}
        \textbf{Rank} & \textbf{Treatment} & \textbf{Median} & \textbf{IQR} & \bigstrut\\
        \hlineB{2}
          1 &    Repr+GGNN &    64.42  &  1.33 & \quart{77}{2}{78}{154} \bigstrut\\
        \hline
          2 & Repr-wo-GGNN &    63.67  &  0.83 & \quart{75}{2}{76}{154} \bigstrut\\
        \hline
          3 &         GGNN &    62.59  &  4.64 & \quart{66}{10}{74}{154} \bigstrut\\
        \hline
          4 &     SySeVR$^1$ &    56.03  &  3.20 & \quart{55}{7}{60}{154} \bigstrut\\
        \hline
          5 &     SySeVR$^m$ &    46.82  &  4.44 & \quart{35}{9}{41}{154} \bigstrut\\
          5 & Russel et. al. &    45.62  &  1.33 & \quart{37}{3}{38}{154} \bigstrut\\
        \hline
          6 &      VulDeePecker$^1$ &    35.20  &  8.82 & \quart{7}{19}{16}{154} \bigstrut\\
          6 &      VulDeePecker$^m$ &    32.12  &  10.27 & \quart{0}{21}{9}{154} \bigstrut\\
        \hlineB{2}
    \end{tabular}
    \label{tab:full_comparison_devign}
\end{table}

==> Tables/slice_real_world.tex <==
\begin{table*}[!htb]
    \centering
    \caption{\small{\textbf{Performance of CNN+RF model to predict vulnerability of code slices extracted from real world datasets (accuracy/f1-score).}}}
    \footnotesize
    \begin{tabular}{l|cc|ccc||cc|ccc}
    \hline
    \multirow{3}{*}{\textbf{Dataset}} &   \multicolumn{5}{c||}{\textbf{API Call slice}} & \multicolumn{5}{c}{\textbf{Array Index slice}}  \\
    \cline{2-11}
    &  \multicolumn{2}{c|}{\textbf{Slice Granularity}}  &  \multicolumn{3}{c||}{\textbf{Function Granularity}} &  \multicolumn{2}{c|}{\textbf{Slice Granularity}}  &  \multicolumn{3}{c}{\textbf{Function Granularity}}\\
    \cline{2-11}
    & \textbf{Accuracy} & \textbf{F1} & \textbf{\%f*} & \textbf{Accuracy} & \textbf{F1} & \textbf{Accuracy} & \textbf{F1} & \textbf{\%f*} & \textbf{Accuracy} & \textbf{F1}\\
    \hline
    Devign & 47.75 & 36.19 & 90.90 & 50.53 & 57.53 & 48.68 & 42.44 & 43.43 & 51.28 & 55.38\\
    \hline
    \realdata & 81.49 & 5.88 & 74.22 & 84.37 & 19.94 & 68.75 & 12.95 & 30.70 & 75.15 & 25.55\\
    \hline
    \end{tabular}\\
    *\textbf{\%f} is the percentage of function from which at least one corresponding slice can be extracted and hence considered for prediction by respective model.
    \label{tab:slice_real_world}
\end{table*}

==> Tables/token_real_world.tex <==
% ! TEX root = ../RQ_details/rq1.tex

\begin{table}[!htb]
    \centering
    \caption{\small{\textbf{Existing approaches' performance on real world datasets (accuracy/f1-score).}}}
    \footnotesize
    \begin{tabular}{l|c|c|c|c}
    \toprule
    \textbf{Dataset}     &   \textbf{CNN+RF}  &   \textbf{CNN}   &\textbf{ BLSTM }  &   \textbf{BGRU}\\
    \midrule
    Devign &   55/45    &   56/39 & 56/34   &   55/38\\
    \midrule
    \realdata &   90/9    & 91/2 & 84/21 & 88/13 \\   
    \bottomrule
    \end{tabular}
    \label{tab:token_real_world}
\end{table}

==> Tables/token_size.tex <==
\begin{table}[!htpb]
\caption{\small \textbf{Average number of tokens per sample for each dataset.}}
\centering
\footnotesize
\label{tab:dataset}
\begin{tabular}{llr}
\toprule
&\textbf{Dataset} &  \textbf{Average \#Tokens} \\ 
\midrule 
\multirow{4}{*}{Pre-existing} & SATE IV Juliet \cite{okun2013report}   & 127.26 \\
& VulDeePecker    \cite{li2018vuldeepecker}   &  84.01  \\
& SySeVR    \cite{li2018sysevr}    & 233.31 \\
& Github + Debian   \cite{russell2018automated}   & 151.86 \\  
% \midrule
% {Curated Real-world} & Chromium + Debian & 5545.77\\%~\evan{check the numbers}\\
\bottomrule
\end{tabular}
\label{tab:avg_token}
\end{table}

==> backup/background_back.tex <==
\section{Methodology}
\label{sec:back}

Most recent Deep Learning based vulnerability detection (referred to as \vd hereafter) pipelines commonly consisted of the following three parts~\cite{goodfellow2016deep}: data preprocessing, model training, and model validation. An illustration for the pipeline is shown in Figure~\ref{fig:pipeline}. We give an overview for the components of the pipeline, and discuss recent research for each component when deep learning is applied to \vd on source code in a static analysis style.

\subsection{Data Collection}
\label{subsec:data_col}

\noindent Data collection procedure play a very important role in any \vp tool. Specially for the tools which rely on the static properties of the code~\cite{}. To collect data for training Deep Learning based \vp tool, there are two different direction of approaches \textemdash a. use of synthetic data, b. use of real data. In first approach, researchers often use vulnerable and good code examples that are used for exampling Common Vulnerability Enumerations (CVEs) or Common Weakness Enumerations (CWEs). For instance, SATE IV Juliet Test Suite consists of  synthetic code examples with vulnerabilities from 118 CWE classes. This dataset was originally
designed to explore the performance of static and dynamic analyzers. Li~\etal~\cite{li2018vuldeepecker, li2018sysevr} and Russel~\etal\cite{russell2018automated} evaluated their method on this dataset. 

\noindent In the latter approach, there is an effort of collecting data from real code from open source projects~\cite{russell2018automated, zhou2019devign}. In this case, code are collected from real world projects. Russel~\etal used different static analyzers to annotate code examples as vulnerable or non-vulnerable. Albeit simple, this method leads to a potential threat of letting the Deep Learning model learn whatever the static analyzers can annotate; seriously restricting the scope of \vp tool.

\begin{figure}[!htb]
    \centering
    \includegraphics[width=0.85\linewidth]{imgs/plane.pdf}
    \caption{Data Collection Procedure in \realdata.}
    \label{fig:data_collection}
\end{figure}

\noindent In contrast, similar to Zhou~\etal~\cite{zhou2019devign}, we collected and annotated vulnerability data from real world vulnerability fix commits from projects' issue tracking repository. Figure~\ref{fig:data_collection} shows the data collection procedure in \realdata. First, we filtered out 


\subsection{Data Preprossessing}

The success of DL lies in its capacity to extract high-level features from a vast quantity of data automatically~\cite{krizhevsky2012imagenet, simonyan2014very}. 
However, vast quantities of data, especially from real-world sources without expert labeling as often used in \vd, may contain a wide spectrum of noise. %~\cite{li2018vuldeepecker, li2018sysevr}. 
In theory, a good DL model should be able to tolerate some noise (\ie, features that are not related to the source of vulnerability) and identify meaningful signals (\ie features that are related to the source of vulnerability). However, since DL is a data-driven process, excessive noise in data forces (biases) the model to learn inaccurate hypotheses~\cite{goodfellow2016deep}. For instance, without proper human labeling of vulnerable code fragments, the model can be biased to learn inaccurate labeling --- \eg that buffer overflows are associated with if statements defined in the beginning of the function. %The granularity of code fragments can also be a source of bias for DL-based techniques, 
% Typically, people train their deep learning model on a large dataset in order to enjoy the benefits of deep learning, which are automatic feature extraction and an end-to-end training process. However, a large dataset would also include a wide spectrum of noise originated from different code lengths, program structures, naming conventions, positions of vulnerability and types of vulnerability.

To tackle this problem of noise in DL-based approaches to \vd, researchers should use one or more of several preprocessing techniques. Good preprocessing should remove most of the noise while retaining crucial information~\cite{li2018vuldeepecker, li2018sysevr} related to vulnerabilities. Some such techniques are described below. 
% Researchers need to determine how to properly pre-process datasets such that the noise can be filtered out without loss of much crucial information. There are multiple techniques that help with this, as we explain in the following.

\subsubsection*{Code Normalization }
Developers may use a wide variety of identifier names in their source code, chosen according to project policy, business requirements, \etc When analyzing source code with a diverse set of possible tokens representing identifiers, the occurrence of individual identifiers may be very sparse. Or, alternatively, the same identifiers might be used very frequently in similar contexts in the same codebase, perhaps implying unwarranted associations between those specific identifiers and vulnerabilities. Hence it can be very difficult for DL models to learn the correct hypotheses involving identifiers.  To solve this problem, researchers have proposed several techniques to normalize tokens and/or identifiers. This can be achieved in several ways, ranging from mapping tokens to corresponding type or generic names~\cite{russell2018automated}, \eg {\tt VARIABLE, FUNCTION}, to transformation of a large sparse identifier namespace to a dense space with pre-specified rules~\cite{li2018vuldeepecker, li2018sysevr}, such as symbolically tokenizing identifiers to {\tt VARIABLE\_1, FUNCTION\_2}. This kind of transformation can be learned as well~\cite{li2018vuldeepecker, li2018sysevr}. 

% Similar to what has been done in program analysis research \saikat{need citation}, to minimize the size of vocabulary in training, 
% user-named tokens can be mapped to generic tokens according to pre-specified rules, or lexers. According to different sets of rules, the vocabulary size can vary from hundreds to thousands --- which affects the learning power of the model. The larger the number of tokens in the generic set, the more information is retained in model training, but large numbers of tokens also hurts generalizability since the vocabulary may include tokens specific to the current dataset. 

\begin{figure*}[ht]
  %\includegraphics[width=\textwidth,height=5cm, keepaspectratio = true]{./imgs/flow_chart.pdf}
  \includegraphics[width=0.9\linewidth,keepaspectratio = true]{./imgs/Overview.pdf}
  \caption{\textbf{\small A Common Pipeline for Using Deep Learning in Vulnerability Detection.}}
  \label{fig:pipeline}
\end{figure*}

\subsubsection*{Code Segmentation }
In this context, segmentation means cutting off the parts of code not related to vulnerabilities by slicing~\cite{weiser1981program} or other methods.  For example, a single line of code can cause a security vulnerability (take misuse of \textit{strcpy} as an example). In such a case, if all the lines of the corresponding file are included, it will drop the performance or generalization of the model because of extraneous noise. Thus, \emph{segmenting} any known sources of vulnerability seems useful. However, it is non-trivial to collect a well-annotated dataset where only the vulnerable lines are annotated. To overcome this problem, some researchers use synthetic datasets where vulnerabilities are automatically or manually injected~\cite{dolan2016lava}. However, this approach may induce bad generalization, as we will discuss in later sections. Further,  there are complicated scenarios where multiple functions are involved in a single (known) vulnerability~\cite{lhee2003buffer}, but inter-procedural code segmentation is a non-trivial task~\cite{yamaguchi2014modeling}.  
% It may be tempting to include all the lines from every source file in the training data. But this might damage the quality of the training data since a single line of code can cause a security vulnerability (take misuse of \textit{strcpy} as an example), which further leads to drop in performance or generalization because of extraneous noise.
% Thus, \emph{segmenting} any known sources of vulnerability seems useful. In this context, segmenting means cutting off the unrelated parts of code by slicing~\cite{weiser1981program} or other methods.  The first difficulty in doing so is that it is not easy to collect a well-annotated dataset that is sufficient for a deep learning task, where in particular the vulnerable lines of code are marked as such. Some researchers use synthetic datasets in which vulnerabilities are automatically or manually injected to overcome this problem~\cite{dolan2016lava}. However, this approach may induce bad generalization, as we will discuss in later sections. The second difficulty is that there are complicated scenarios where multiple functions are involved in a single (known) vulnerability~\cite{cite}, but inter-procedural code segmentation is a non-trivial task~\cite{cite}.  

% \saikat{Move this section to a new section named "Machine Learning Models", How RNN, LSTM, CNN are used and what is the high level differenct between these.}

\subsection{Models for Vulnerability Detection}

%\subsubsection*{Different Types of Models Used in Deep Learning}
\subsubsection*{Types of DL models}
The DL literature has explored a variety of models for different tasks. Choice of DL model is highly task and data specific --- a different task may need a different kind of model~\cite{goodfellow2016deep}. In this paper, we focus on classification models for \vd research. Kinds of classification models used previously in this area include Feed-forward neural network~\cite{fan2017autoencoder, wang2016automatically}, Recurrent Neural Networks (RNNs)~\cite{hochreiter1997long, cho2014learning}, and Convolution Neural Networks (CNNs)~\cite{russell2018automated}.

At a high level, the goal of all these models is to take the input and transform it to the output space. Feed-forward networks consider a fixed-length input, typically a real-valued vector representing the data example at hand, features of source code in the \vd case. Converting an example to a real-valued vector is called \emph{feature extraction}. Oftentimes, it is not clear what features of the data are most important for the task, hence feature extraction is hard and may lead to sub-optimal solutions~\cite{hira2015review}. 

RNNs (and its variations LSTM, GRU, \etc), on the other hand, are sequential models that are effective when the input is of variable-length. For instance, in the case of classifying source code as vulnerable (or not), the input is a variable-length sequence of programming language and identifier tokens. While processing the sequential data, an RNN's hidden state captures the information of the sequential dependencies. One drawback of such a model is that it is not very effective in modeling the non-linear dependencies between parts of the input. There have been several improvements proposed over RNN (and also LSTM, GRU), such as bi-directional RNNs~\cite{schuster1997bidirectional, graves2013hybrid} that model data dependencies in both directions, tree-RNN~\cite{tai2015improved} to model tree-structured data representations, graph-NN~\cite{scarselli2009graph} to capture graph-structured data, \etc. However, each of these models is computationally more expensive than its predecessor.  

CNNs are highly effective for detecting higher-level features by extraction of spatial features through convolution filters, and are widely used in image processing and text processing. For vulnerability detection, CNNs are used by~\cite{russell2018automated} and achieved much better performance than static analyzers. It is able to convolute on the inputs, and empirically, it can learn and surpass the capacity of human designed filters \cite{krizhevsky2012imagenet}.


\subsubsection*{Data Representations}% for Vulnerability Detection}
Detecting vulnerabilities can be considered a classification task, where a model is trained with annotated data and then is used to predict vulnerable/not-vulnerable for un-labeled data. In such a way,  modeling source code and natural languages are somewhat similar\textemdash  both have a set of grammars and are sequential in nature. Source code further has structural information like abstract syntax trees (ASTs), control flow graphs (CFGs) and data flow graphs (DFGs) that can be leveraged during modeling. 

\saikat{However, this paper's focus is not on advancing model design for vulnerability detection; our attention is empirically evaluating performance of popular deep learning models, check this.}


\subsection{Model Validation}
Given a well-optimized model, how does anybody know whether it will work on previously unseen data? This is the \emph{generalization problem} that we focus on in this paper.  In theoretical machine learning, there have been recent advancements in analyzing generalization of two-layer neural networks~\cite{ma2018priori, arora2019fine}. However, state-of-the-art mathematical generalization analysis requires extremely wide networks (impossible to fit in memory) and are confined to shallow architectures (two or three layers), which makes them far from ideal for practical use.

Without perfect theoretical tools, researchers use a train/test split and cross-validation/k-fold validation to validate their models' performance~\cite{kohavi1995study}. The procedure is simply leaving part of the initial dataset aside, training on only a subset (the training set), then evaluating the model's performance at the end of training on this left-out set of data (the test or validation set). This is a simple yet powerful empirical trick and has been employed in much applied machine learning research. But this empirical technique does not guarantee that the model would perform at the same level under different scenarios than the left-out test set, and it is this paper's purpose to explore when, why and how a deep learning model will generalize well on unseen data for vulnerability detection. 

\subsection{Vulnerability Detection Model Deployment}
\label{subsec:model_deployment}

==> backup/methodology_backup.tex <==
\section{Methodology}
\label{sec:method}

In this section, we describe the overview of Deep Learning based \vp systems,the datasets that we studied in this research, relevant data collection procedure, the approaches that we studied, and analysis techniques that we used answering the research questions outlined in Section~\ref{sec:rq_summary}.

% \subsection{Overview}
% \label{subsec:overview}
% \begin{figure*}[!htb]
%   \includegraphics[width=0.9\linewidth,keepaspectratio = true]{./imgs/Overview.pdf}
%   \caption{\textbf{\small Overview of different sub-components of Deep Learning based Vulnerability Detection systems.}}
%   \label{fig:pipeline}
% \end{figure*}

Figure~\ref{fig:pipeline} shows an overview of Deep Learning based Vulnerability Detection system. First, in training phase, a large number of code (usually function) and corresponding vulnerability annotations are collected. Then code samples are preprocessed using appropriate tokenizer/parsers. Afer this step, samples are represented in appropriate format (\eg sequence of tokens, graph etc.). Then an appropriate model is trained. In deployment phase, the code sample that is being tested for vulnerability goes through the same preprocessing and abstracting technique in the training phase. The processed code sample that is being tested for vulnerability, are then passed the the pre-trained model to get a binary verdict.

\subsection{Datasets}
\label{sucsec:dataset}
We analyzed two types of datasets: 1) four open-source synthetic datasets that are studied in the past, 2) two real-world vulnerability datasets.

\input{Tables/dataset.tex}

\input{Tables/approaches}

\subsubsection{\textbf{Synthetic Datasets}}~
We conducted our study on four publicly available datasets: SATE IV Juliet~\cite{okun2013report} from the National Institute of Standards and Technology (NIST), VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, and Github+Debian~\cite{russell2018automated}  that are studied by previous research. VulDeePecker and SySeVR are further divided into sub-categories based on the vulnerability types. The details of each dataset are shown in Table \ref{tab:number_samples}.

{SATE IV Juliet}~\cite{okun2013report} was created for testing static analyzers by NIST; it contains 118 different CWEs and 64,099 test cases. Each test case has a few bad implementations that induce specific vulnerabilities and a few good implementations that fix the issue. {VulDeePecker}~\cite{li2018vuldeepecker} and {SySeVR}~\cite{li2018sysevr} are produced by slicing programs,
the code snippets are created from real-world programs and synthetic programs. {Github+Debian}~\cite{russell2018automated} was curated by running three static analyzers on public projects retrieved from Github and the Debian Linux kernel.  It also includes the SATE IV Juliet dataset. 

Detailed information of these datasets is shown in Table~\ref{tab:paper_sum}. Both VulDeePecker and SySeVR significantly re-use SATE IV Juliet dataset.  Note that, a majority of SATE IV Juliet samples are synthetic programs, which may not be representative of real-world vulnerabilities. In contrast, Github + Debian was collected from real-world software projects and a small part of synthetic data to avoid potential issues of a pure synthetic dataset. However, in this dataset, the vulnerabilities are annotated by static analysis; since static analyzers are known to have high false-positive rate~\cite{johnson2013don,smith2015questions}, a model trained with such labeled data would mimic the behavior of the static analyzers, and inherit all the false-positives that the static analyzers may have introduced.


\smallskip
\subsubsection{\textbf{Real World Datasets}}~
\label{sec:real_world}
A good dataset for vulnerability studies should cover a wide range of vulnerabilities that are representative of the real-world issues. Zhou~\etal~\cite{zhou2019devign} proposed Devign dataset, which consist of vulnerabilities from five open source projects. However, examples from two of those five projects are publicly available. 

To understand better about the real world vulnerabilities, we also curated such data\footnote{Our collected dataset is available in this anonymous directory \url{https://bit.ly/2IaPB18}} by tracking the past vulnerabilities from two open-source projects: Linux Debian Kernel and Chromium (open source project of Chrome). We select these projects because (i) these are two very popular and well-maintained public projects with large evolutionary history, (ii) the two projects represent two important program domains (OS and browsers) that have diverse security issues, and (iii) both the projects have plenty of publicly available bug reports.

% \begin{figure}[!htb]
%     \centering
%     \includegraphics[width=0.65\linewidth]{imgs/data_col.pdf}
%     \caption{Overview of our data collection procedure. The green shaded functions are labelled as non-vulnerable while the red shaded one is vulnerable.}
%     \label{fig:data_col}
% \end{figure}

For Chromium, we scraped its bug repository Bugzilla\footnote{\url{https://bugs.chromium.org/p/chromium/issues/list}}. First, we collected the fixed issues labeled with  ``security"  tag and then downloaded the corresponding bugfix patches from Google Git.  For Linux Debian Kernel, we downloaded the security-related bugfix patches from the Debian security tracker\footnote{\url{https://security-tracker.debian.org/tracker/}}.  Given a bugfix patch, the old version is annotated as buggy and the newer version as non-buggy.  Note that, some commits of Debian security issues are not always publicly linked to the patch.  In such cases, we only considered the issues where the corresponding patches are available. Figure~\ref{fig:data_col} shows a brief overview of our data collection procedure.

\begin{table}[!htb]
    \centering
    \footnotesize
    \caption{Details about the real world datasets.}
    \begin{tabular}{l l c}
    \toprule
    \textbf{Dataset} & \textbf{Projects} & \textbf{\# Examples} \\
    \midrule
    Devign~\cite{zhou2019devign}     &  Qemu, FFMpeg & 26036\\
    \realdata & Chromium, Debian & 22148\\
    \bottomrule
    \end{tabular}
    \label{tab:my_label}
\end{table}

For each patch, we extracted the corresponding vulnerable and fixed versions (\ie, old and new version) of {\tt C/C++} source and header files that are changed in the patch. We annotate all the functions that are changed in a vulnerable file; leaving rest of the functions as non-vulnerable. Annotating code in this way simulates real world \vp settings, where developer would want to know which function is vulnerable given all the functions in a file/project. In contrast, Zhou~\etal~\cite{zhou2019devign} only annotated the ``after'' version of a changed function as non-vulnerable, excluding all the other functions that are available in file from the dataset. While we emphasize of collecting a dataset that will train a model to discriminate vulnerable code from non-vulnerable code, Devign dataset implicitly will train a model to discriminate between the before and after version of a vulnerability fix commit. Albeit a very good artifact, Devign dataset is very much suitable for learning based automated program repair tools such as Codit~\cite{chakraborty2019codit}. Nevertheless, since the purpose of this paper is to investigate on the current status of the Deep Learning based approaches and figure out ``dos'' and ``don'ts'', we conducted experiments on both the \realdata and Devign data.

\subsection{Studied Approaches}
\label{subsec:background}

\begin{lstlisting}[caption = \small{\textbf{A piece of code in its original form, after symbolic tokenization and after abstract normalization.}}, basicstyle=\scriptsize\tt,captionpos=b, label = {lst:normalizer}]
/*Code in its original form*/
if (fgets(password, 100, stdin) == NULL) {
    printLine("fgets() failed");
    password[0] = '\0';
}

/*Code after abstract tokenization*/
if ( FUNCTION ( VARIABLE , INT , IDENT ) == NULL ) {
    FUNCTION ( STRING ) ;
    VARIABLE [ 0 ] = CHAR ;
}

/*Code after symbolic tokenization*/
if ( FUNCTION_1 ( VARIABLE_0 , INT , IDENT ) == NULL ) {
    FUNCTION_2 ( STRING ) ;
    VARIABLE_0 [ 0 ] = CHAR ;
}
\end{lstlisting}

\noindent\textbf{Token Abstraction}~ Like all deep learning based code modeling applications, Vocabulary explosion is also a very pressing problem in \vp task. The number of possible identifiers in a code can be virtually infinite making it very difficult to reason about the tokens. To overcome this problem, Russel~\etal~\cite{russell2018automated} used abstract token format, where they replaced all literals with literal types and identifiers with corresponding identifier type (\ie variable, function etc.). VulDeePecker~\cite{li2018vuldeepecker} and SySeVR~\cite{li2018sysevr} used symbolic token abstraction, where the tokens are replaced by the positions from the respective symbol table. Devign~\cite{zhou2019devign}, in contrast took a different route, where they trained a Word2Vec~\cite{rong2014word2vec} model for code token and used token embedding for Word2Vec tokens. To build the abstract and symbolic tokenizer, We built a Clang compiler{clang} based tokenizer. Listing~\ref{lst:normalizer} shows an example code in original form, in abstract tokenized form and in symbolic tokenized form. We built a Word2Vec model for using Gensim~\cite{rehurek_lrec}, which we trained based on code from Qemu, FFMpeg, Chromium and Debian projects. 

\noindent\textbf{Code Granularity}~ 
Zhou~\etal~\cite{zhou2019devign} and Russel~\etal~\cite{russell2018automated} assumed function granularity of code in their respective work. Given a function, both of those model predict whether it is vulnerable or not. VulDeePecker~\cite{li2018vuldeepecker} and SySeVR~\cite{li2018sysevr} in contrast extracted slices from some entry points in a respective function and classified those slices. While, VulDeePecker only considers backward slicing, SySeVR considers a combination of both the forward slice and the backward slice. Both of these approaches start from some pre-defined entry points inside a function (\eg API calls, array indexing etc.) and extract slices. We build a code slicer based using Joern code property graph generator~\cite{yamaguchi2014modeling}. VulDeePecker, SySeVR, and Russel~\etal represented the input code to their model as a sequence of tokens rendering their models as sequence based modeling. Devign~\cite{zhou2019devign}, on the other hand, extracted the code property graph using Joern and leveraged graph based modeling technique. 

\noindent\textbf{Studied Models}~ 
To have a better understanding, we studied four different token based Deep Learning model. The models are based on Convolutional Neural Network (CNN) based ~\cite{russell2018automated}, Bidirectional LSTM (BLSTM) based ~\cite{li2018vuldeepecker}, Bidirectional Gated Recurrent Unit (BGRU) based~\cite{li2018sysevr} models. Along with these three, we also studied the CNN + RandomForest model, proposed by Russel~\etal. For Devign~\cite{zhou2019devign}, we implemented the Gated Graph Neural Network~\cite{li2015gated} based classifier, since the implementation of Devign is not publicly available. Since improving the model is beyond the scope of this paper, we empirically validated all our research question using our simplified implementation of Devign. 

==> backup/rq_summary_backup.tex <==
\section{Research Questions}
\label{sec:rq_summary}

A vulnerability detection tool based on source code helps developer write and check code for potential vulnerability at a very early stage so that it can be fixed before the code goes to deployment. Since static analysis causes a lot of false positives~\cite{}, using static analyzer for vulnerability detection is often less solicited method among developers~\cite{}. On top of that, hand writing violation patterns for static analyzers are often gruesome for the developers. A Machine Learning based vulnerability detection tool should be able to discover those violation patterns from sufficient volume of data and should avoid the huge number of false positives. 

In this paper, we look into the different Deep Learning(DL) based techniques that are proposed in vulnerability detection literature and investigate in details about the applicability of those techniques, their pitfalls. We systematically investigate the reasons behind the pitfalls and propose some suggestions for overcoming such shortcomings.
\saikat{The above two paragraph may go to introduction}


Any ML based technique depends on the data that the technique is trained on. Success of a ML technique largely depends on both the power of the technique and quality of the data. 

Although recent DL based  techniques~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated} showed very high performance in detecting vulnerabilities, we are interested to investigate their proposed models' applicability in real world software development scenario. To simulate real world software development, we first investigate how each of these techniques generalize beyond the dataset each individual model is trained on. Hence, we ask the first research question,
% \RQ{1}{How well an existing DL based approach can be applicable in a plausible real world development scenario?}
\RQ{1}{How well a trained model perform to detect vulnerability on unseen data?}

Since all the DL based vulnerability detection technique require annotated data, we are simulating this scenario particularly considering that a developer may not have sufficient annotation. Hence they would want to rely on a pre-trained model on other dataset. Scarcity of annotated vulnerable code legitimize this use case scenario. 

To answer this question, we test each of the trained model on other test datasets. Here we use test examples from other dataset as a proxy of unknown dataset in the wild.

Details about the experimental setup are described in Section~\ref{sec:rq1-answer}. With detailed experiments, we find the answer, 
\RS{1}{The existing approaches does not work well when applied in a very plausible real world development scenario. A DL model for Vulnerability detection does not generalize beyond the dataset it is trained on.}


Now we are more interested on investigating the properties of the dataset that is keeping it from generalizing examples   

To answer this question, we use two different intuitive solutions. Firstly to test vulnerability from a particular dataset (Dataset-A), we deploy pre-trained model from other dataset and observe the performance. Secondly, we build an ensemble model~\cite{} trained on all the other datasets.  We use both \emph{Veto} and \emph{Majority Voting} ensemble method. In \emph{Veto} ensemble method, if one model says a piece of code is vulnerable, the we conclude that code is vulnerable. In case of \emph{Majority Voting}, we go with the decision of the majority models. 

We observe that, the techniques we investigated in above research question are all token based model \ie they consider code as a sequence of tokens. Having that in mind, we are curious to know what is keeping a model to be applicable in real world scenario. To that end, we take a closer look at both the models and the datasets they are trained on. Here we ask our next research question, 
\RQ{2}{Why existing token based approaches do not generalize in real world use case scenario?}

To answer this question, first we observe different properties of the datasets. In particular we investigate on the simplicity of those datasets. We build a simple SVM to measure. If an SVM can be fitted to a dataset with higher fitting accuracy and wider SVM margin is intuitively a very simple dataset. We call this bias \emph{Contextual Bias}. We also measure the degree for code repetitions inside a dataset. We call this \emph{Repetition Bias}. We also measure these biases on our real world dataset collected from Chromium and Debian. 

With our research finding showing that the datasets much simpler than real world scenario, we focus on what the models are actually learning. We investigate whatever the model is learning has anything to do with the vulnerability. We do a case study with extracting important feature that is learned by a model. This study shows us the contribution of different tokens for a prediction of vulnerability. The details of the experiments and case study are described in Section~\ref{sec:bias-and-case-study}. We summarize the findings as, 
\RS{2}{The existing synthetic datasets are so simple that an SVM based classifies is sufficient for vulnerability prediction. These dataset do not exhibit the complex property of vulnerability in real dataset. Furthermore, token based models based on these datasets learn irrelevant features and patterns.}

With the aforementioned research findings at hand, we hypothesize that any Deep Learning based model to be applicable in real world development scenario, needs to be trained on real world data. We focus on the performance of existing models on real world dataset. We ask, 
\RQ{3}{How well does existing models perform in real world dataset?}
To answer this question, we adopt 2 different approach. First one is proposed by Russel~\etal~\cite{russell2018automated}, where code for each function is considered as a standalone point for prediction. The second approach is proposed by Li~\etal~\cite{li2018vuldeepecker}, where instead of entire body of the functions, slices extracted from different interest points in the function (\eg API calls, array usage etc.) are considered for prediction. To have a fair comparison of these two approaches, if any of the slices extracted from a function is predicted as vulnerable by the latter approach, we consider the whole function as predicted vulnerable. Experimental details are described in Section~\ref{sec:existing-method-on-real-data}.
After rigorous experiment, we reach to the following research findings
\RS{3}{Token based DL techniques are \textbf{not} very effective in predicting vulnerability in real world scenario. Even static analyzer (through slice extraction) \textbf{does not} help as much to boost the performance of token based models.}









==> body/1_intro_back.tex <==
\section{Introduction}
\label{sec:intro}

Vulnerabilities in software are pervasive\needcitation. Automated detection of security vulnerabilities is a fundamental problem in systems security. A  vulnerability detection tool which can predict vulnerability in the source code can help developer patch that vulnerability at a very early stage of software development\needcitation. Traditional techniques for this task suffer from high false-positive/negative rates, thus developers tend to avoid such tools/techniques~\cite{johnson2013don}. For example, static analysis based \vp typically results in high false positives, \ie, detects non-vulnerable cases as vulnerable and dynamic analysis suffers from high false negatives, \ie, cannot detect many real vulnerabilities\needcitation. Such inadequacy of these tools creates enormous overhead for developers since they cannot fully rely on those tools~\cite{smith2015questions}.

Recent progress in Machine Learning (ML), especially in domains like computer vision and natural language processing, has sparked interest in using ML to detect security vulnerabilities automatically with high accuracy. According to Google scholar, 68 papers appeared in popular security and software engineering venues in 2018 alone that apply ML to detect different types of bugs\footnote{published in S\&P Oakland, CCS, USENIX Security, NDSS, ASE, FSE, ICSE, TSE, ISSTA, and ACSAC.}. In fact, several recent studies have demonstrated very promising results achieving high accuracy (up to $95\%$) at detecting vulnerabilities~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated, li2017large, maiorca2019digital, suarez2017droidsieve, zhou2019devign}. 

\input{tex/intro_fig}

Given such reported success of ML models at detecting vulnerabilities, it is natural to ask whether developers can effectively and reliably use such tools. It is of paramount importance to investigate whether these models are actually learning meaningful features and whether these will generalize to detect real-world vulnerabilities accurately. Lack of generalizability in ML models is a potentially serious problem in traditional ML for long time domains like computer vision~\cite{barreno2006can, torralba2011unbiased}. Implicit biases in the dataset might allow ML models to achieve high accuracy by learning highly idiosyncratic features specific to that dataset instead of generalizable features. For example, Yudkowsky et al.~\cite{yudkowsky2008artificial} described an instance where the US Army found out that a neural network for detecting camouflaged tanks did not generalize well because of dataset bias even though the model achieved very high accuracy in the testing data. Further investigation revealed that all the photos with the camouflaged tanks in the dataset were shot in cloudy days and the model trivially learned to classify lighter and darker images instead of detecting tanks. 

In our experiment, we find that there is a vast gap between the reported performance of existing techniques and their performance on real-world vulnerability data. We investigate the feature that the models in existing techniques are picking up from pre-existing datasets leveraging state-of-the-art explanation techniques ~\cite{springenberg2014striving,guo2018lemna}. To our surprise, models that exhibit outstanding performance in pre-existing datasets are picking up irrelevant features from those datasets. These features are not related to vulnerabilities in any way and are likely to be artifacts of those datasets. 

To that end, we propose a general framework to collect real-world vulnerability data, so that the user can create their own datasets. We also create a new vulnerability dataset (hereafter \realdata) from two large-scale popular real-world projects: Chromium and Debian to help us to understand the performance of different techniques in the real-world \vp. Having both the code and vulnerability annotation coming from the real-world, this is dataset is the most realistic data to our best knowledge. 

Further, we propose a novel graph-based representation learning technique for \vp. We base our representation learning on two key observations from the literature. First, reasoning about the semantics of code is the most important feature for effectively detecting vulnerability ~\cite{yamaguchi2014modeling, zhou2019devign}. For a model to learn about the semantics, it has to be presented with such. For instance, if a model considers only the AST of code, it cannot reason about the control flow or data flow. Second, if we can decouple an ML-based task to easier sub-tasks and deploy different sub-models for those sub-tasks, each individual model will learn to do easier sub-task better. A combination of such sub-models will eventually improve the performance in original tasks~\cite{russell2018automated, chakraborty2019codit}. Following these observations, we design a modularised framework for \vp namely \tool (\underline{\bf \textsc{Re}}presentation Learning for \underline{\bf \textsc{V}}uln\underline{\bf \textsc{e}}r\underline{\bf \textsc{a}}bi\underline{\bf \textsc{l}}ity Prediction). \tool divides the \vp task into three steps \textemdash~(a) learning about the semantics of the code, (b) balancing training data, and (c) learning to predict vulnerability with representation learning. 

Our experimental result shows that \tool achieves the best F1-score in real-world datasets in comparison with state-of-the-art techniques. \tool’s graph-based modeling technique results in 36.4\%, and 14.9\% improvement from the highest performing token-based model in two different real-world vulnerability datasets. \tool’s representation learning model also improves the F1-score by 38.09\%, and 12.66\% those datasets. 

In summary, our contributions in this paper are,
\begin{enumerate}
\item We systematically study existing approaches in \dlvp task with respective pros and cons. Our systematic study would help future researchers and practitioners in \vp to better understand unique aspects and components of \dlvp task. 
\item With thorough investigation and corresponding evaluation results, we show that existing datasets do not represent real-world vulnerabilities enough. To our best knowledge, we are the first to define a taxonomy of realism in \vp datasets.
\item With the detailed experiment, we point out and advocate for graph-based reasoning and graph-based modeling of \vp task. 
\item We propose an algorithm to collect real-world vulnerability data so that researchers/practitioners can create their own vulnerability dataset to train their model. We also collected \realdata, a real-world dataset from two open-source projects \textemdash Chromium and Debian following the algorithm we proposed. We release our dataset in this anonymous directory \url{https://bit.ly/3bX30ai}.
\item We propose a novel graph representation learning-based \vp technique \tool, which performs best in detecting real-world vulnerabilities compared to state-of-the-art techniques.
\item We also open source all our code and data we used in this study for broader dissemination. Our code and replication data are available in \url{https://git.io/Jf6IA}.
\end{enumerate}

% Vulnerabilities in software are pervasive. Automated detection of security vulnerabilities is a fundamental problem in systems security. Existing approaches suffer from high false positive/negative rates~\cite{johnson2013don, smith2015questions}. For example, static analysis typically results in high false positives, i.e., detects benign cases as buggy and dynamic analysis suffers from high false negatives, i.e., fails to detect many real vulnerabilities. Manually designing detection techniques that can achieve better balance between false positives and negatives has turned out to be very hard even after decades of effort.

% Recent progress in Machine Learning (ML) especially in domains like computer vision and natural language processing has sparked interest in using ML to automatically detect security vulnerabilities with high accuracy. According to Google scholar, $68$ papers appeared in popular security and software engineering venues in 2018 alone that apply ML to detect different types of bugs\footnote{published in S\&P Oakland, CCS, USENIX Security,  NDSS, ASE, FSE, ICSE, TSE, ISSTA, and ACSAC.}. In fact, several recent studies have demonstrated promising results achieving high accuracy (up to $95\%$) at detecting vulnerabilities~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated, li2017large, maiorca2019digital, suarez2017droidsieve, zhou2019devign}. 

% Given such reported success of ML models at detecting vulnerabilities, it is natural to ask whether these models are indeed learning meaningful features and whether they will generalize to detect real-world vulnerabilities in the wild accurately. Lack of generalizability in ML models have long been known as a potentially serious problem in traditional ML domains like computer vision~\cite{barreno2006can, torralba2011unbiased}. 

% Being a data driven approach, any machine learning models are as good as the data it is trained on\needcitation. To understand the usability of existing techniques, we intend to check whether existing datasets are robust enough to represent real world vulnerabilities. Implicit biases in the dataset might allow ML models to achieve high accuracy by learning highly idiosyncratic features specific to that dataset instead of generalizable features. For example, Yudkowsky et al.~\cite{yudkowsky2008artificial} described an instance where US Army found out that a neural network for detecting camouflaged tanks did not generalize well due to dataset bias even though the model achieved very high accuracy in the testing data. Further investigation revealed that all the photos with the camouflaged tanks in the dataset were shot in cloudy days and the model simply learned to classify lighter and darker images instead of detecting tanks. 

% % In this paper, we study different approaches in Deep Learning based \VP (will be referred to as \dlvp hereafter) that are proposed in recent few years. More specifically, our focus is investigating the applicability of those approaches in finding real world vulnerabilities. For this work, we primarily focus on the Deep Neural Network (DNN) models that take source code as input~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated}, not  binaries~\cite{yamaguchi2013chucky, yamaguchi2015automatic,li2017large, maiorca2019digital, suarez2017droidsieve}. As source code contains more information (i.e., richer features) than binary, we expect the source-code-based ML models to achieve better robustness than the ones learning from binary data.

% In our experiment, we find that there is a huge gap between the reported performance of existing techniques and their performance on real world vulnerability data indicating that those technique learning irrelevant features from respective datasets. We investigate the irrelevant feature that the models in existing techniques are picking up leveraging state-of-the-art explanation techniques ~\cite{springenberg2014striving,guo2018lemna}. Our experimental results show that, existing datasets are not representative of real world vulnerabilities -- either they are too simple to catch complex vulnerabilities in real world, or the ratio of vulnerable to non-vulnerable code is completely unrealistic. This observation led us to design \dlvp technique that learns from real world vulnerability data. 

% % To understand the quality of the datasets, we define a taxonomy of dataset classification based on the synthetic and realistic nature of the dataset. This categorization model would help future research in this domain to curate appropriate datasets for \dlvp task. 
% To that end, we propose an general framework to collect real world vulnerability data, so that user can create their own datasets. We also create a new vulnerability dataset (will be referred to as \realdata hereafter) from two large-scale popular  real-world  projects: Chromium and Debian to help us to understand the performance of different techniques in real world \vp. Having both the code and vulnerability annotation coming from real world, this is dataset is the most realistic data to our best knowledge. Along with the code and vulnerability annotation source, \realdata preserves the distribution of vulnerable and non-vulnerable code in a given file of projects. Unlike \devigndata, \realdata is more representative of real world vulnerability dataset in terms of the data distribution.


% % We further investigate on using different type of models and techniques that are used for \dlvp task. We investigate different pros and cons of each of the techniques. Our experimental results show that graph based modeling is necessary for learning vulnerability patterns. Our vanilla graph based model achieves good performance in predicting real-world vulnerabilities. We advocate on further investigation of graph based DL models in \vp, since such models show the ability to reason about syntax and semantics of the code through learning from the structure of the graph. Finally, we investigate on the realistic distribution of vulnerability data and its effect of \dlvp. We propose a training data balancing technique which which models are able to effectively learn from real world vulnerability data. 

% In summary, our contributions in this paper are,

% \begin{enumerate}
%     \item We systematically study existing approaches in \dlvp task with respective pros and cons. Our systematic study would help future researchers and practitioners in \vp to better understand different aspects of \dlvp task. 
%     \item With through investigation and corresponding evaluation results, we show that existing datasets do not represent real world vulnerabilities enough. To our best knowledge, we are the first to define a taxonomy of realism in \vp datasets.
%     \item With detailed experiment, we point out and advocate for graph based reasoning and graph based modeling of \vp task. 
%     \item We propose an algorithm to collect real world vulnerability data, so that researchers/practitioners can create their own vulnerability dataset to train their model. We also collected \realdata, a real world dataset from two open source projects -- Chromium and Debian following the algorithm we proposed. We release our dataset in this anonymous directory \url{https://bit.ly/3bX30ai}.
%     \item We also open source the all our code and data we used in this study for broader dissemination. Code, replication data are available in \url{https://git.io/Jf6IA}.
% \end{enumerate}

% % Next step is to use those model in real world software developers during the production phase. In order for doing that, it is very important to measure the performance of those models and techniques in real world. An approach producing a lot of false negatives while detecting vulnerability in production code might not be usable by the developers due to its ineffectiveness. On the other hand, with high false positives, developers have to manually check and verify each of the predicted vulnerability. Such an approach will lose interest among the developers due to its imprecision.  


% % These ML models can be used in software production is two different ways. While working in a relatively new project, developers typically transfer their knowledge working in other projects~\cite{}. Similarly, in case of \vp of those projects, developers would want to reuse models trained from other projects/vulnerability datasets. In contrast, for a project with a lot of fixed vulnerabilities in project history, developers would want to retrain those models on their past vulnerabilities, so that in future if those mistakes are made will be caught.

% % Recent advancements in Graph Based Deep Learning~\cite{li2015gated, allamanis2017learning, battaglia2018relational} unveils opportunity to learn from and reason about structure of the graph. Some initial approach~\cite{zhou2019devign} in \vp using such models show promises of overcoming the drawbacks of token based modeling. In these approaches, the whole graph of a program is presented to the model and model learns to reason about it. Since the whole graph, including all the nodes, the syntactic and semantic relationship between the nodes are individually available to the model, there is an opportunity for the model to learn reasoning about it. 



% % In our experiment, we find that there is a huge gap between the reported performance of existing techniques and their performance on our datasets indicating that those technique learning irrelevant features from respective datasets. We investigate the irrelevant feature that the models in existing techniques are picking up leveraging state-of-the-art explanation techniques ~\cite{springenberg2014striving,guo2018lemna}. Our experimental results show that, existing datasets are not representative of real world vulnerabilities -- either they are too simple to catch complex vulnerabilities in real world, or the ratio of vulnerable to non-vulnerable code is completely unrealistic. 




% % In the first use case scenario, it is important to assess how generalizable existing techniques are on detecting vulnerability real world production code.  We find that the vulnerability datasets used to train/test ML models are often re-purposed from existing code samples for other tasks. For instance, SARD dataset~\cite{SARD}, which is heavily used to train VulDeePecker and SySeVR, mostly contain synthetic and academic code. Albeit good artifact for testing other vulnerability detectors (mostly static analysis based), the code samples in this dataset are often very simple and do not truly reflect the complexity of real world vulnerabilities. Notable other approaches in collecting real world vulnerability dataset include the Draper dataset~\cite{russell2018automated}, the \devigndata dataset~\cite{zhou2019devign}. It is of utmost important to test whether models trained on these dataset actually perform in predicting real world vulnerabilities. If a model learns important patterns that are related to vulnerability, that model would certainly be a good fit for predicting vulnerability in real world. On the other hand, if a model fail to predict real world vulnerability effectively, it surely is learning some other features from the dataset that have nothing to do with the vulnerability. High performance of models in those dataset indicates that the models are doing the right thing for wrong reason. In such case, those datasets are not representative enough for real world vulnerabilities.

% % In second use case scenario, when developers have sufficient data train their vulnerability predictor, developers can follow the techniques proposed in literature and train their own models. However, before deploying the models into the \vp task, it is important to understand which technique should be adopted and pros and cons of every techniques. There are two genre of modeling code -- (a) as a sequence of tokens (often anatomized to prevent vocabulary explosion problem), (b) as a graph (often the semantic graph). Being a semantic reasoning problem~\cite{yamaguchi2014modeling}, \vp task demands reasoning about code semantics~\cite{yamaguchi2015automatic}. 

% % Code treated as plain sequence of tokens often loses the semantic information. To add some semantics into the code tokens sequence, some existing approaches extract slices before converting it to a token sequence. Although these slices contains semantic information, there are still a token sequence, and thus inherits the problems with token based models. One such problem is, if one extract slice from control dependency graph, the data dependencies are not there in the slice and vice versa. When slices are extracted from a combined control and data dependency graph and converted to a sequence to token, the relationship information between the tokens (whether they are control dependent or data dependent) are lost. 
% % for testing non-ML-based detectors and therefore had various biases built in them. For example, several popular datasets~\cite{li2018vuldeepecker, li2018sysevr} contain synthetic buggy code with non-standard function names/if conditions repurposed from datasets~\cite{okun2013report} designed to test static-analysis-based vulnerability detectors. Similarly, some datasets~\cite{russell2018automated} use static analysis for generating ground-truth labels and therefore suffer from biases caused by the false positives/negatives of the underlying analyzer. Albeit good artifacts for these

% % Lack of generalizability in ML models have long been known as a potentially serious problem in traditional ML domains like computer vision~\cite{barreno2006can, torralba2011unbiased}. 
% % There are two main issues that affect generalizability: (i) overfitting to training data and (ii) bias in the dataset. 
% % ML models, which overfit to training data, pick up features specific to the training data and thus do not generalize well to test data (i.e., testing accuracy tends to be significantly lower than training  accuracy). A common way to detect such cases is to compare the values of training loss and testing loss over different epochs~\cite{lever2016points}. Any large difference between these two curves (i.e., training and testing loss over increasing number of epochs) often indicates overfitting. 

% % The main factor hurting generalizability is different types of implicit biases present in the dataset~\cite{torralba2011unbiased, yudkowsky2008artificial}. Such biases are introduced during the dataset generation/curation/labeling process and therefore affect both the testing and training data equally (assuming that they are drawn from the same dataset). These biases tend to be more subtle and harder to detect 
% % % than overfitting 
% % as they allow ML models to achieve high accuracy in the test data by learning highly idiosyncratic features specific to that dataset instead of generalizable features. For example, Yudkowsky et al.~\cite{yudkowsky2008artificial} described an instance where US Army found out that a neural network for detecting camouflaged tanks did not generalize well due to dataset bias even though the model achieved very high accuracy in the testing data. Further investigation revealed that all the photos with the camouflaged tanks in the dataset were shot in cloudy days and the model simply learned to classify lighter and darker images instead of detecting tanks. 


% % For instance, some techniques consider implicitly learn to reason about code semantics by learning from the token sequences in the slices extracted from code. Other techniques treat the code as a holistic semantic graph and reason about it. A systematic study is very important to understand the capability of each individual model. 


% % In this paper, we systematically measure the generalizability of four state-of-the-art neural network architectures~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated} that have been reported to detect security vulnerabilities with high accuracy (upto $97\%$) in existing literature. For this work, we primarily focus on the Deep Neural Network (DNN) models that take source code as input~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated}, not  binaries~\cite{yamaguchi2013chucky, yamaguchi2015automatic,li2017large, maiorca2019digital, suarez2017droidsieve}. As source code contains more information (i.e., richer features) than binary, we expect the source-code-based ML models to achieve better generalizability than the ones learning from binary data.

% % In this paper, we systematically perform in-depth study of several recent Deep Learning(DL) based \vp techniques~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated}, that hat have been reported to detect security vulnerabilities with high accuracy (upto $95\%$). To understand the performance of these models in finding real world vulnerability, we create a new real world vulnerability dataset by crawling vulnerable and non-vulnerable code from two open source repository (\ie Chromium and Debian). For this work, we primarily focus on the Deep Neural Network (DNN) models that take source code as input~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated}, not  binaries~\cite{yamaguchi2013chucky, yamaguchi2015automatic,li2017large, maiorca2019digital, suarez2017droidsieve}. As source code contains more information (i.e., richer features) than binary, we expect the source-code-based ML models to achieve better robustness than the ones learning from binary data.

% % In our experiment, we find that there is a huge gap between the reported performance of existing techniques and their performance on our datasets indicating that those technique learning irrelevant features from respective datasets. 
% % generalize well to any other dataset except the one they were trained on. Next, we carefully measure and rule out overfitting as a potential cause as the gaps between testing and training loss over different epochs tend to be very small for all of the tested models. Therefore, we focus on dataset bias as another possible root cause. We define a taxonomy of different potential biases affecting the venerability datasets and provide measurement methodology to accurately estimate their effects. We use our methodology and demonstrate that all of popular vulnerability datasets that we tested suffer from multiple types of bias introduced either during the data generation or labeling process. 

% %  We further use state-of-the-art explanation techniques ~\cite{springenberg2014striving,guo2018lemna} to perform multiple case studies demonstrating the effect of dataset bias on the features learned by the neural network models. 
% % Figure~\ref{fig:example}~\cite{okun2013report} demonstrates one such example where the neural network picked up  uncommon variable/function names and if conditions (shown in red) completely unrelated to vulnerability as the strongest feature for predicting that vulnerability. We also found that some of those features were specifically introduced to test static analyzers which was the original use case of the dataset~\cite{juliet_user}. 

% % \begin{figure}[h]
% %     \centering
% %     \includegraphics[width=0.9\linewidth, keepaspectratio=True]{imgs/intro-example.pdf}
% %     \caption{\small{\textbf{A sample important feature (highlighted in red, green indicates lower importance) learned by one of our tested neural networks trained on SATE IV Juliet dataset~\cite{okun2013report}.} Note that the feature has nothing to do with the actual vulnerability and is simply an artifact of the dataset bias (i.e., uncommon variable/function names, if conditions, etc.). Some of these biases (i.e., uncommon if conditions) were introduced specifically for testing static analyzers, the original purpose of the dataset.}}
% %     \label{fig:example}
% % \end{figure}

% % Next,  We measured that the dataset, unlike the test sets used in the prior work, is balanced and does not suffer from any serious bias issues. We use this dataset to demonstrate that none of the existing models can achieve more thn 50\% test accuracy and thereby demonstrate a fundamental limitation of the models used in the literature. Therefore, we speculate that the tested models do not tend to have enough capacity to achieve reasonable performance  from balanced real-world datasets and finding models that can accurately detect vulnerabilities in such datasets is still an open problem. Our results demonstrate the importance of carefully designing balanced and unfair datasets for ML-based vulnerability detection. Besides our bias measurement methodology, we also provide a summary of best practices that we hope will help the ML-based vulnerability researchers to avoid such mistakes in the future.  

% % In summary, our paper makes the following contributions:
% % \begin{enumerate}
% %     \item We systematically measure the generalizability of four state-of-the-art neural network architectures that reported achieving high accuracy (up to $97\%$). Our results demonstrate that none of these networks generalize beyond the datasets they are trained on.
% %     \item 
% %       To the best of our knowledge, we are the first to define a taxonomy of different potential biases affecting venerability datasets and provide a measurement methodology to accurately estimate their effects. 
% %     \item 
% %     We use our bias measurement methodology to demonstrate that all of popular vulnerability datasets that we tested suffer from multiple types of bias introduced either during the data generation/labeling process which significantly hurt the generalization of the models trained on those datasets. 
% %     \item 
% %     We collected a real-world dataset from developer/user reported vulnerabilities from two popular real-world projects (\ie, Chromium and Debian) and demonstrate that none of the existing models can achieve high accuracy on this dataset. Therefore, we argue that ML-based vulnerability detection is still is very much an open problem potentially requiring new neural architectures.
% % %     We are currently working on making our bias measurement code, balanced datasets, and the corresponding models publicly available for community use. 
    
% % \end{enumerate}


% % To this end, we systematically study different datasets, and DL models to 


==> body/2_background_back.tex <==
% \begin{figure*}[bht]
%   \includegraphics[width=0.9\linewidth,keepaspectratio = true]{./imgs/Overview.pdf}
%   \caption{\textbf{\small Overview of different sub-components of Deep Learning based Vulnerability Detection systems.}}
%   \label{fig:pipeline}
% \end{figure*}
%\input{tex/dlvp_overview.tex}

%\section{Background and Theory}
%\section{Existing Approaches and Limitations}
\section{Background and Challenges}
\label{sec:background}

\dlvp methods aim to detect unknown vulnerabilities in target software by learning different vulnerability patterns from a training dataset. 
% In theory, DL based approaches for \vp can be applied in both static analysis~\cite{russell2018automated} and dynamic analysis scenario~\cite{she2019neuzz}. However, most recent and accentuating approaches in DL based \vp research addressed the problem in static analysis setting~\cite{larochelle2001statically}. In particular, most of the approaches proposed in recent few years predict vulnerability in a given piece of code by reasoning about the code and associated static properties of code (\ie control/data flow graph~\cite{zhou2019devign}, static slices from the graph~\cite{li2018sysevr, li2018vuldeepecker} etc.). 
% \begin{algorithm}[!htpb]
% \SetAlgoLined
%  $\mathscr{D} \leftarrow Collect\_Data\_For\_Training()$\;
%  $\mathscr{M} \leftarrow Choose\_Model()$\;
%  $\mathscr{D}' \leftarrow Preprocess\_Data(\mathscr{M}, \mathscr{D})$\;
%  $Train(\mathscr{M}, \mathscr{D}')$\;
%  $\mathscr{D}_t \leftarrow preprocessed\_evaluation\_data()$\;
%  $Evaluate(\mathscr{M}, \mathscr{D}_t)$\;
%  \caption{Overview of DL-based \vp Approach}
%  \label{alg:overview}
% \end{algorithm}
Most popular \dlvp approaches consist of three steps: data collection, model building, and evaluation. 
%follow the generic steps as outlined in~\Cref{fig:overview}. 
First, data is collected for training, and an appropriate model is chosen as per design goal and resource constraints.
The training data is preprocessed according to the format preferred by the chosen model. 
Then the model is trained to minimize the loss function. 
The trained model is intended to be used in the real world. 
To assess the effectiveness of the model, researchers accumulate unseen test examples, preprocess them, %using the same technique used prior to training. Then, 
ans then evaluate the performance on those test examples.

\bray{move this para to related work} Although, such approaches can be applied in both static- ~\cite{russell2018automated} and dynamic-analysis scenario~\cite{she2019neuzz}, most recent and prominent work addressed the problem in static analysis setting~\cite{larochelle2001statically}, where vulnerabilities are predicted using static code properties (\eg control/data flow graph~\cite{zhou2019devign}, static slices from the graph~\cite{li2018sysevr, li2018vuldeepecker} etc.). 

% In general, most \dlvp approaches consist of the following  steps.
% %follow the generic steps as outlined in~\Cref{fig:overview}. 
% First, data is collected for training, and an appropriate model is chosen as per design goal and resource constraints.
% Next, the training data is preprocessed according to the format preferred by the chosen model. Then the model is trained to minimize the loss function. The trained model is now ready to be used in the real world. 
% To assess the effectiveness of the model, researchers accumulate unseen test examples and preprocess those examples using the same technique used prior to training. Then, the performance of the model is evaluated on those test examples.

 
%Most DL based \vp systems follow the generic framework outline in \ref{alg:overview}. First, data are collected for training. Next, appropriate model is chosen according to different design goal and resource constraints and training data is pre-processed according to the format of the chosen model. Then the model is trained to minimize loss function. When a model is completely trained, it is ready to be used in the real world. To understand the effectiveness of the model, researchers accumulate unseen test examples and preprocess those examples using the same technique used before training. Then, performance of the model is evaluated on those test examples.

The rest this section describes the theory of DL-based \vp approaches (\S\ref{subsec:overview_models}), their different steps (\S\ref{subsec:background_overview}), and challenges that limits the applicability of the existing approaches (\S\ref{sect:challenges}). 

%\subsection{Theory behing DL-based Vulnerability Prediction}
\subsection{\dlvp Theory}
\label{subsec:overview_models}

% In a DL based \vp system, vulnerability of code elements are learned from set of vulnerable and non-vulnerable code elements (training data, $D$). Depending on the representation, code elements can be sequence of tokens, graphs etc. Given a set of set of code element and corresponding vulnerability labels represented as $(x, y)$, the goal of the model is to learn features that maximizes the probability $p(y|x)$. Formally, a model learns the optimal parameter settings ($\theta^*$) such that,

DL-based vulnerability predictors learn the vulnerable code patterns from a training data ($D_{train}$) set where code elements are labeled as vulnerable or non-vulnerable.  Given a code element $(x)$ and corresponding vulnerable/non-vulnerable label $(y)$, the goal of the model is to learn features that maximize the probability $p(y|x)$ with respect to the model parameters ($\theta$). Formally, training a model is learning the optimal parameter settings ($\theta^*$) such that,

\begin{equation}
    \theta^* = argmax_\theta{\prod\limits_{(x,y) \in D_{train}}p(y|x, \theta})
    \label{eqn:prob}
\end{equation}

First, a code element ($x^i$) is transformed to a real valued vector ($h^i \in \mathbb{R}^n$), which is a compact representation of $x^i$. How a model transforms $x^i$ to $h^i$ depends on the specifics of the model. This $h^i$ is transformed to a vector $h_f^i \in \mathbb{R}^2$. The 2 elements in $h_f^i$ denote the probability of code element $x^i$ being non-vulnerable and vulnerable respectively. More formally, $h_f^i[0] = p(y^i = 0|x^i)$ and $h_f^i[1] = p(y^i = 1|x^i)$ and $h_f^i[0] + h_f^i[1] = 1.0$. In general, this transformation and probability calculation is achieved through a feed forward layer and a softmax~\cite{bridle1990probabilistic} layer in the model. Typically, for binary classification task like \vp, optimal model parameters are learned by minimizing the cross-entropy loss~\cite{suter1990multilayer}. Cross-entropy loss indicates the distance between what the model's predicted probability distribution and the actual probability of a code being vulnerable~\cite{plunkett1997exercises}. However, other loss functions can be used depending on the focus of the task~\cite{zellner1986bayesian, allwein2000reducing}. 


%  An optimal $\theta^*$ lets the model learn the most influential features to predict vulnerability with the hope that the optimal model should be able to predict vulnerability for unseen code elements. 

%First a code element ($x^i$) is transformed to a real valued vector ($h^i \in \mathbb{R}^n$). This $h^i$ is the compact representation of the code element in consideration. How a model transforms a $x^i$ to $h^i$ depends on the specifics of the model. This $h^i$ is transformed to a vector $h_f^i \in \mathbb{R}^2$. The 2 elements in $h_f^i$ denote the probability of code element $x^i$ being non-vulnerable and vulnerable respectively. More formally, $h_f^i[0] = p(y^i = 0|x^i)$ and $h_f^i[1] = p(y^i = 1|x^i)$ and $h_f^i[0] + h_f^i[0] = 1.0$. This transformation and probability calculation is achieved through a feedforward layer and a softmax~\cite{bridle1990probabilistic} layer in the model. 

% An optimal $\theta^*$ lets the model learn most influential features to predict vulnerability. This optimal model should predict vulnerability for unseen code elements. 


%\subsection{Components in DL based \vp}
\subsection{\dlvp pipeline}
\label{subsec:background_overview}

\dlvp mainly contains three steps: (i) data collection, (ii) modeling, and (iii) evaluation, as we discuss below. 

\begin{figure}[!htb]
    \centering
    \includegraphics[width=\linewidth]{imgs/realism.pdf}
    \caption{\small Different \dlvp dataset and their synthetic/realistic nature.}
    \label{fig:realism_axis}
\end{figure}

\noindent
\textbf{(i) Data Collection.}
%\subsubsection{Data Collection}
To train a \vp model, we need a set of annotated code with annotation as vulnerable or benign. The number of vulnerable code should be large enough to let the model learn from it. Researchers used a wide spectrum of data sources to collect data for \dlvp (see~\Cref{fig:realism_axis}). On one end of this spectrum there is synthetic data where the vulnerable code along with the corresponding  annotations are artificially created. On the other end, there is real data, where vulnerable code are collected from real-world code repositories. Other datasets lie between synthetic and real datasets where real code is either modified or its annotations are \emph{not} derived from real sources. \Cref{tab:dataset_purpose} shows a summary of the dataset used so far in different approaches. 

Among the synthetic datasets, the code and annotation are synthesized based on predefined patterns. For instance, SATE IV Juliet dataset~\cite{okun2013report}, which was originally synthesized for testing static analyzers, is used by Russel~\etal~\cite{russell2018automated} to train their \dlvp model. Other synthetic data include SARD~\cite{SARD}, which consists of synthetic and academic code, is heavily used by VulDeePecker~\cite{li2018vuldeepecker} and SySeVR~\cite{li2018sysevr}. 

In some other datasets, vulnerable code are isolated from its context and often modified in a way to demonstrate the vulnerability. Even though those code are taken from real world, modification and/or isolation make them lose some of the complexities of real world. National Vulnerability Database (NVD ~\cite{booth2013national}) is one such dataset.
%that contains vulnerable code from real world projects, but often modified and in isolation. 

Russel~\etal~\cite{russell2018automated} collected the Draper dataset, where they collected code from real world open source repositories. However, the annotation of these code examples are made using several static analyzers. These code snippets, being part of the real world code base, are complex enough to represent code in the wild. However, since they are annotated by a static analyzer, any model trained on these dataset will inherit any potential drawbacks from the annotation tools. 

Other approaches to collect real-world vulnerabilities extract vulnerable/non-vulnerable annotations from code metadata (\eg commit message, bug report, issue report, etc.), which are easily available from code repositories~\cite{zhou2019devign, zhou2017automated} like GitHub, Bitbucket, etc. For instance, Zhou~\etal's~\cite{zhou2019devign} introduced a dataset from the closed bug reports of four open-source projects, where the bugs are already patched. The corresponding buggy code version is annotated as ``vulnerable'', and the patched version is annotated as ``benign''. 
%They collected data from four open source projects (Linux Kernel, Qemu, FFMpeg, Wireshark), two of which (FFMpeg and Qemu) are publicly available. 
Such an annotation scheme often requires the classification of code metadata and often requires human intervention. Due to the relatively fewer number of vulnerable code and their metadata, the dataset collected in this fashion is often quite small. 


% \smallskip
% \noindent \textbf{Semi-Synthetic Datasets.}~
% To address the complexity of real-world code, Draper dataset proposed by Russel~\etal~\cite{russell2018automated} collected functions from open source repositories and annotated those using a collection of static analyzers. Some examples in SARD~\cite{SARD} dataset are also taken from production code; however, they are isolated from their code context. Although these datasets are more complex than synthetic ones, they do not fully capture the complex nature of the real-world vulnerabilities to the full extent due to artificial annotations or out-of-context nature, respectively. For example, \dlvp trained on Draper dataset will be biased by the patterns annotated by static analyzers, which often result in false positives. Moreover, without the context SARD patterns become relatively simple.  


%Further approaches to collect real world vulnerability include extraction of annotation from analyzing the code metadata (\eg commit message, bug report, issue report, etc.) that are abundant with established code repositories~\cite{zhou2019devign, zhou2017automated}. For instance, Zhou~\etal's~\cite{zhou2019devign} proposed a dataset consisting of four real world projects. To create the dataset, they considered bug/issue reports that are already patched. The code version before the issue is fixed is annotated as ``vulnerable'' and the version after the fix is annotated as ``benign''. They collected data from four open source projects (Linux Kernel, Qemu, FFMpeg, Wireshark), two of which (FFMpeg and Qemu) are publicly available. This annotation scheme often require classification of code metadata and often require human intervention. And due to the relatively fewer number of code metadata related to the vulnerability, dataset collected in this fashion are often quite small. 

% This data collection is non-trivial,~\saikat{is data scarcity the only issue? this is my speculation, there is no specific mention in any paper about the reson. } 
% since vulnerable code is very scarce in practice than the benign code. To address such scarcity, different approaches used a wide spectrum of data sources (see~\Cref{fig:realism_axis}). On one end of this spectrum there is synthetic data where the vulnerable code are artificially created. On the other end, there is real data, where vulnerable code are collected from real world code repositories
% \saikat{this sentence is not connected with data imbalance issue----why real/synthesis will address data imbalance.}.
% Figure~\ref{tab:dataset_purpose} shows a summary of the dataset used so far in different approaches. 

% To circumvent this problem, 
% Several synthetic datasets are proposed in the literature for other tasks -- \eg testing static analyzer, demonstration of vulnerability, etc.
%  \saikat{what is other task?}. 
% For example, SATE IV Juliet dataset~\cite{okun2013report}, originally designed to test static analyzers, contains sets of synthesized vulnerable and non-vulnerable code corresponding to different CWEs. Russel~\etal~\cite{russell2018automated} evaluated their hypotheses based on this dataset. SARD~\cite{SARD} and NVD~\cite{booth2013national} are two datasets used by VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}. SARD dataset, originally designed for evaluating \vp tools, consists of Synthetic, Production and Academic code examples of different known vulnerabilities. Examples in SARD are illustration of those known vulnerabilities in isolation. NVD dataset, in contrast, constitutes of real world vulnerable code (often in isolation). Both in VulDeePecker and SySeVR dataset, synthetic SARD data consist of 90\% of their respective datasets.
% Any model trained on such synthetically generated datasets will have limited applicability in practice, since the seed pattern is known at the first place. Often examples generated in this approach are too simple to match the complexity of real world data. 

% To capture the complex nature of the real world data, another approach is to collect \emph{Semi-real data} where code examples from collected from real world data and annotated with other tools (often from static analyzers). 






\smallskip
\noindent\textbf{(ii) Model Selection and Data Preprocessing.}~
Model selection depends mainly on the information that one wants to incorporate. Token-based models are the most popular choice where code is considered as a sequence of tokens. These models, in general,  do not consider semantic dependencies and thus cannot reason about code semantics. Other popular options, Graph-based models, consider code as graphs, and incorporate different semantic dependencies. Based on the chosen model, the code is preprocessed to match the expected model input~\cite{li2018vuldeepecker, russell2018automated, zhou2019devign}. 


Existing token-based models used different Neural Network architectures. For instance, Li~\etal~\cite{li2018vuldeepecker} proposed a Bidirectional Long Short Term Memory (BSLTM) based model, Russel~\etal~\cite{russell2018automated} proposed a Convolutional Neural Network (CNN) and Radom Forest-based model and compared against Recurrent Neural Network (RNN) and CNN based baseline models for \vp. For such relatively simple token-based models, token sequence length is an important factor to impact performance as it is difficult for the models to reason about long sequences. To address this problem, VulDeePecker~\cite{li2018vuldeepecker} and SySeVR~\cite{li2018sysevr} extract code slices. The motivation behind slicing is that not every line in the code is equally important for \vp. Therefore, instead of considering the whole code fragment, slices extracted from ``interesting points'' in code (\eg API calls, array indexing, pointer usage, etc.) are considered for vulnerability prediction and other lines are omitted. 

\begin{figure}[!htpb]
\centering
\includegraphics[width=0.87\linewidth]{imgs/flow_graph.pdf}
\caption{\small Example of CWE-761, where a buffer is freed not at the start of the buffer but somewhere in the middle of the buffer. This can cause the application to crash, or in some cases, modify critical program variables or execute code. This example shows the importance of long distance data dependency to reason about the vulnerability.\protect\footnotemark
}
\label{code:token_vuln}
\end{figure}
\footnotetext{Details of this vulnerability in \url{https://cwe.mitre.org/data/definitions/761.html}}

Token based models assume that tokens are linearly dependent on each other, and thus, only lexical dependencies between the tokens are present, while the semantic dependencies are lost.  To incorporate some semantic information, VulDeePecker~\cite{li2018vuldeepecker} and SySeVR~\cite{li2018sysevr} extracted program slices of a potentially interesting point. For example, consider the code in Figure~\ref{code:token_vuln}. A slice \wrt {\tt free} function call at line 10 gives us all the lines except lines 6 and 7. The token sequence of the slice are: {\tt void action ( char * data ) const \{ for ( data ; * data != `$\backslash$0' ; \textbf{data ++} ) \{ foo ( data ) ; bar ( data ) ; if ( * data == SEARCH\_CHAR ) \{ \textbf{free ( data )} ;}. In this examples, while the two main components for this code being vulnerable, \ie~{\tt \textbf{data ++}} (line 2) ~and {\tt \textbf{free ( data )}} (line 10) are present in the token sequence, 
they are far apart from each other without explicitly maintaining any  dependencies. 


To incorporate semantic dependencies, graph-based models can be a potential option. A code graph $\mathcal{G}$ is represented by a tuple $(\mathcal{V}, \mathcal{E})$, where $\mathcal{V}$ is the set of nodes, and $\mathcal{E}$ is the set of edges. Each node $v_i \in \mathcal{V}$ is represented by a node type $t_{v_i}$, and a label $l_{v_i}$. Each edge $e^k_{i,j} \in \mathcal{E}$ is a directed edge from node $v_i$ to and $v_j$ represented by an edge type $k$. The edge type represents the type of the edge (\ie control flow edge, data flow edge, AST edge, etc.). Two nodes can be connected by multiple edges of different types. For loops and back-edges, the source and the destination can be the same. Such a graph is usually constructed by augmenting different dependency edges (\ie control flow, data flow, def-use, etc.) to the Abstract Syntax Tree (AST)  representation of the code.~\cite{zhou2019devign}. 


As for the example shown in~\Cref{code:token_vuln}, when we consider the data dependency edges (\red{red} edge), we see that there is a direct edge between those lines making those lines closer to each other making it easier for the model to reason about that connection. Note that this is a simple CWE example (CWE 761), which requires only the data dependency graph to reason about. Real-world vulnerabilities are much more complex and require reasoning about control flow, data flow, dominance relationship, and other kinds of dependencies between code elements~\cite{yamaguchi2014modeling}.

Both graph and token-based models have to deal with {\em vocabulary explosion} problem\textemdash  the number of possible identifiers (variable, function name, constants) in code can be virtually infinite, and the models have to reason about such identifiers.  A common way to address this issue is to replace the tokens with abstract names~\cite{li2018vuldeepecker, li2018sysevr}. For instance, VulDeePecker~\cite{li2018vuldeepecker} replaces most of the variable and function names with symbolic names ({\tt VAR1, VAR2, FUNC1, FUNC2} etc.).

%There are several choices for token based models. Such models are used and compared against (as respective baselines) in different approaches. For instance, Li~\etal~\cite{li2018vuldeepecker} proposed a Bidirectional Long Short Term Memory(BSLTM) based model, Russel~\etal~\cite{russell2018automated} proposed a Convolutional Neural Network(CNN) and Radom Forest based model and compared against Recurrent Neural Network(RNN) and CNN based baseline models. As all token based models classifies sequence of tokens, number of tokens (\ie sequence length) is an important factor that impacts the performance. It is difficult for the models to reason about long sequences. To overcome this problem, VulDeePecker~\cite{li2018vuldeepecker} and SySeVR~\cite{li2018sysevr} extracts slices from the code. The motivation behind this technique is that not every line in the code are equally important for \vp. Instead of considering the whole code fragment, slices extracted from ``interesting points'' in code (\eg API calls, array indexing, pointer usage etc.) are considered for vulnerability prediction. In such way, when predicting vulnerability in an ``interesting point'', lines irrelevant to the that are omitted.  

% Graph based models considers code as a graph and learns to reason about both the nodes in the graph and structure of the graph. To retain both syntactic and semantic information of the code, code graph is constructed by augmenting different edges (\ie control flow, data flow, def-use etc.) to the AST of the code. Zhou~\etal~\cite{zhou2019devign} proposed a graph model based approach where the model learned to reason about syntactic and semantic graph (AST with control flow and data flow edges) and compared %against syntax only graph (AST) and CFG and DFG. 

% How each approach tackle the curse of dimensionality problem
%The number of possible identifiers (variable, function name, constants) in code can be virtually infinite. This huge number of possible tokens make it very difficult to reason about the code. In natural language processing, this problem is known as vocabulary explosion problem. Both the token based and graph based model suffers from this problem. To overcome this problem, one way is to replace the tokens with abstract names~\cite{li2018vuldeepecker, li2018sysevr}. For instance, VulDeePecker~\cite{li2018vuldeepecker} replaces most of  variable and function names with symbolic names ({\tt VAR1, VAR2, FUNC1, FUNC2} etc.). 

% There are several ways to convert tokens to real values vectors\saikat{suddenly introduced vector, say something like the models take embedded inputs etc.}. 
Expected input for all the models are real valued vectors commonly known as embeddings. There are several ways to embed tokens to vectors. One such way is to use an embedding layer~\cite{turian2010word} that is jointly trained with the \vp task~\cite{russell2018automated}. Another option is to use external word embedding tool(\eg \emph{Word2Vec}~\cite{rong2014word2vec}) to create vector representation of every token. VulDeePecker~\cite{li2018vuldeepecker} and SySeVR~\cite{li2018sysevr} uses \emph{Word2Vec} to transform their symbolic tokens into vectors. Devign~\cite{zhou2019devign}, in contrast, uses \emph{Word2Vec} to transform the concrete code tokens to real vectors. 

Once a model is chosen and appropriate preprocessing is done on the training dataset, the model is ready to be trained by minimizing a loss function. Most of the existing approaches optimize the model by minimizing some variation of cross-entropy loss. For instance, Russel~\etal~\cite{russell2018automated} optimized their model using cross-entropy loss, Zhou~\etal~\cite{zhou2019devign} used regularized cross entropy loss. However, as described in~\cref{subsec:overview_models}, minimizing cross-entropy loss lets the model learn the probability distribution without putting much emphasis on physically separating the positive and negative examples in latent feature space. 
% The optimal model is one which satisfies the optimality constraint in Equation~\ref{eqn:prob}. Usually, this is achieved by minimizing a loss function. For example, 

%%%%%%%%%%%%%%%%%%%% From Section 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%
% Most of the vulnerabilities in code are exhibited by the semantics of the code. For example, consider a code where a {\tt buffer} is initialized with size {\tt n}. After initialization, if that buffer is accessed with any index ``{\tt i > n}'', %(0 based indexing assumed), 
% that will make the code vulnerable to ``Buffer Overflow''. However, a simple check on $i$ before accessing the array will make the code non-vulnerable. A data-dependency analysis is the most common way to figure out such vulnerability~\cite{clang, cppcheck, newsome2005dynamic, godefroid2008grammar}. 
% Thus, a good \dlvp should incorporate such semantics in their analysis. 
% Here we discuss different ways semantics of the code are modeled in existing literature.  
% % \smallskip\noindent\textbf{Token-based Modeling.}~As discussed in~\Cref{subsec:background_overview}, the popular models for \dlvp are token-based models~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated}. These 
% \smallskip
% \noindent\textbf{Graph-based Modeling.}~
% First, to understand how the node types $t_{n_i}$ and $l_{n_i}$ influence vulnerability detection, we use traditional ML algorithms (\ie SVM, Logistic regression, K Nearest Neighbor, etc.) on top of the $d$-dimensional feature vectors ($f_{n_i} \in \mathbb{R}^d$) extracted from nodes.  
% Next, we use a graph neural network~\cite{li2015gated} (GNN) that learns the whole structure of a graph through a message-passing network. The architecture is similar to the routing protocols of computer networks, where each node (router/host) passes its current information (typically routing table) to the immediate neighbors. Every node, after receiving information from all the neighbors, updates its own information. After a certain period of time, every node eventually has information about the whole graph topology. For GNN, the message passed by a node $n_i$ is its feature vector $f_{n_i}$.  Zhou \etal~\cite{zhou2019devign} use a similar approach on \devigndata dataset and report promising results for \vp task. 
% We will compare the impact of different model choices in~\Cref{sect:rq2}.
%%%%%%%%%%%%%%%%%%%% From Section 3 %%%%%%%%%%%%%%%%%%%%%%%%%%%%



\smallskip
\noindent\textbf{(iii) Evaluation.}~
To understand the applicability of a trained model for detecting vulnerability in the wild, it must be evaluated first. In most cases, a trained model is evaluated on held out test set. Test examples go through the same pre-processing technique as the training and then the model predicts the vulnerability of those pre-processed test examples. This evaluation approach gives a pseudo estimate of how the model will perform when it will be used to detect vulnerabilities in the wild. 

\subsection{Challenges with Existing Approaches}
\label{sect:challenges}
 
Application of DL in \vp creates new opportunity to learn from complex nature of the real-world vulnerabilities, as DL can learn important features without explicitly mentioning them and also tend to ignore noises. However, the existing approaches proposed over last few years come with their respective challenges (see~\Cref{tab:existing_approach_design_choices} for the design choices of existing approaches). As the empirical results show (\S\ref{sec:results}), these challenges pose major threat to the applicability of these models to predict vulnerabilities in real world code. We divide the problems into three broad categories -- i. challenges with Data source, ii. challenges with modeling and training
, iii. challenges with evaluation. 

\smallskip
\noindent\textbf{{i. Challenges with Data.}}~ 
The problems with the dataset lie on how realistic the data source is and  how they are annotated (see~\Cref{fig:realism_axis}).  For instance, most of the vulnerability examples in NVD and SARD\footnote{Used by VulDeePecker, and SySeVR} datasets are synthetic and quite simple. Thus, a model trained on this dataset will be limited to the simple patterns offered by this dataset. 

\begin{figure}[!htpb]
\begin{lstlisting}
void action(char *data) const {
    /* FLAW: We are incrementing the pointer in
    the loop - this will cause us to free the *
    memory block not at the start of the buffer */
    for (; *data != '\0'; data++){
        if (*data == SEARCH_CHAR){
            printLine("We have a match!");
            break;
        }
    }
    free(data);
}
\end{lstlisting}
\caption{\small Example Vulnerable implementation of (slightly modified) {\tt action} function in CWE761, Taken from VulDeePecker data repository \url{https://bit.ly/2VnBaxP}.}
\label{code:simple_synthetic_code}
\end{figure}

\begin{figure}[!htpb]
\begin{lstlisting}
static int read_request_line(
        request_rec *r, apr_bucket_brigade *bb){
    ...
/* FLAW: proto_num and protocol are not properly initialized. This could lead to a denial of service attack.*/
    if (APR_STATUS_IS_ENOSPC(rv)) {
        r->status    = HTTP_REQUEST_URI_TOO_LARGE;
@\red{\textbf{-}}@      @\red{\textbf{r->proto\_num = HTTP\_VERSION(1,0);}}@
@\red{\textbf{-}}@      @\red{\textbf{r->protocol  = apr\_pstrdup(r->pool, "HTTP/1.0");}}@
    }
    else if (APR_STATUS_IS_TIMEUP(rv)) {
        r->status = HTTP_REQUEST_TIME_OUT;
    }
    else if (APR_STATUS_IS_EINVAL(rv)) {
        r->status = HTTP_BAD_REQUEST;
    }
@\green{\textbf{+}}@    @\green{\textbf{r->proto\_num = HTTP\_VERSION(1,0);}}@
@\green{\textbf{+}}@    @\green{\textbf{r->protocol  = apr\_pstrdup(r->pool, "HTTP/1.0");}}@
    return 0;
    ...
}
\end{lstlisting}
\caption{\small CVE-2015-0253 - An instance of Null Pointer Dereferencing vulnerability in Apache HTTP Server 2.4.12. The {\tt read\_request\_line} function in server/protocol.c does not initialize the protocol structure member, which allows remote attackers to cause a denial of service (NULL pointer dereference and process crash).\protect\footnotemark}
\label{code:real_linux_code}
\end{figure}
\footnotetext{https://nvd.nist.gov/vuln/detail/CVE-2015-0253}

For instance,~\Cref{code:simple_synthetic_code} shows an example of \emph{buffer overflow} vulnerability from the combined dataset that VulDeePecker is trained on. Albeit a very good example for demonstration purpose, real world vulnerabilities are not as simple and isolated as it is. Figure~\ref{code:real_linux_code} shows an example of buffer overflow vulnerability patch from linux kernel. Though the fix is very simple, finding the vulnerability itself require in depth reasoning on semantics of the code. If a model is trained to reason about simpler examples shown in Figure~\ref{code:simple_synthetic_code}, it will not learn to reason about Figure~\ref{code:real_linux_code} code.
 
There are some effort to collect more realistic data by Russel~\etal~\cite{russell2018automated} and Zhou~\etal~\cite{zhou2019devign}. 
However, these data are tainted with either simplistic annotations or  unrealistic vulnerability distributions. 
%Although, these datasets are better than synthetic datasets, there are challenges with these datasets. 
For example, Github and Debian dataset proposed by Russel~\etal~\cite{russell2018automated} is annotated by static analyzers. Hence, a model trained on this dataset will be limited by the  static analyzer's ability to detect vulnerability, which often reports a lot of  false positives~\cite{johnson2013don, smith2015questions}. 
\devigndata~\cite{zhou2019devign} dataset is the most realistic data so far. However, the ratio of vulnerable and non-vulnerable examples in their dataset is approximately 45\%-55\%, which does not reflect the real world distribution of vulnerable code. 

\smallskip
\noindent\textbf{{ii. Challenges with Modeling and Training.}}~ 
Token-based models cannot reason about the syntactic and semantic relationship of the code tokens, which often play important roles in \vp~\cite{clang, cppcheck, flawfiner}. Hence, it is more logical to use graph-based models. However,  graph-based models are much more expensive than their token-based counterparts and do not perform well in a resource-constrained environment. While all the existing techniques train models to learn to discriminate vulnerable and non-vulnerable code samples, the training paradigm does not explicitly focus on the maximal separation between the vulnerable and non-vulnerable examples. Better training strategy of more robust learning objective could be a potential solution to this problem. 

The proportion of vulnerable examples in comparison to the non-vulnerable one in real world dataset is extremely low~\cite{russell2018automated} making the dataset extremely imbalanced. When a model is trained  on such imbalanced dataset, models tend to be biased by the non-vulnerable example. The challenges of learning from imbalanced dataset~\cite{wu2003class} extend to \vp task when learning vulnerability patterns from real world data. 
%Token based models perform very poor to reason about the syntactic and semantic relationship of the code token, which should play an important role in \vp. Any static analysis based tool for finding vulnerability reasons on the semantic graph of the code~\cite{clang, cppcheck, flawfiner}. Hence, it is more logical to use graph based models to predict vulnerability in real world. The only  reason someone would want to use token based model is if there is any resource constraints, since graph based models are much more expensive that their token based counterparts. However, as we will see in our experiment, in real world projects, if we use simple machine learning models on top of the code graphs work better than that of a token based model.  

\smallskip
% VulDeePecker did do a 10 fold cross validation, so we can assume that SySeVR does the same. 

\noindent\textbf{{iii. Challenges with Evaluation.}}~ 
Although all the existing approaches report their performances using their own evaluation dataset, it does not give a comprehensive overview of the applicability of the model in the real-world. All we can learn from such intra-dataset evaluation is how good an approach is to fit their own dataset. 
Although there are some limited case studies on such models finding vulnerabilities in real-world projects, those case studies do not shed light on the false positives and false negatives~\cite{johnson2013don}. 
The number of false positives and false negatives are directly correlated to the developer effort in \vp~\cite{aggarwal2006integrating} and too much of any would hold the developer from using the model~\cite{heckman2011systematic, muske2016survey}.
%Although all the existing approaches show performance evaluation within respective dataset, it does not give a comprehensive overview of the applicability of the model in real world. All we learn from the intra-dataset evaluation is how good an approach is to fit and generalize the dataset. A simple cross dataset generalization test would give us an estimate of how applicable an approach is in the real world. Although, there are some limited case study on such models finding vulnerability in real world projects, those case studies do not shed light on the false positives and false negatives while doing those case study. The number of false positives and false negatives are directly correlated to the developer effort in \vp~\cite{aggarwal2006integrating} and too much of any would hold the developer a from leveraging the model~\cite{heckman2011systematic, muske2016survey}.

==> body/5_datasets_investigation.tex <==
\section{Closer look into the existing datasets}
\label{sec:closer_look}

\textbf{RQ1:} \textit{What are the limitations of existing datasets?}

\begin{figure}[!htb]
    \input{Tables/lemna_example_1_integer_overflow}
    \vspace{5mm}
    \input{Tables/lemna_example_2_memory_overflow}
    \vspace{5mm}
    \input{Tables/lemna_example_3_draper_G_D}
    \vspace{5mm}
    \caption{\small \textbf{Code examples visualization with Lemna~\cite{guo2018lemna}. All of these code examples are predicted as vulnerable by respective models. \cref{fig:lemna_int_overflow} and \cref{fig:lemna_memory_overflow} are code slices from NVD+SARD dataset and SySeVR predicted those as vulnerable. \cref{fig:lemna_draper} is also predicted as vulnerable by Russel~\etal's CNN+RF~\cite{russell2018automated} model. \lone{Red} colored tokens contributed the most in respective predictions. \lfive{Green} colored tokens contributed the least.}}
    \label{fig:lemna_examples}
\end{figure}

% \noindent\textbf{}

By now, an obvious question arises in readers' mind about the need of real world data, when we have much larger dataset proposed by different previous approaches readily available. To answer to that, let us closely investigate the limitations of existing (semi-)synthetic datasets. Our in-depth investigation reveals that these datasets are too simple and homogeneous to be representative of the intricacies of real-world vulnerabilities. Essentially, the existing models trained on the synthetic datasets are learning trivial and shallow features that are not related to the core logic of the vulnerabilities.

VulDeePecker~\cite{li2016vulpecker} and SySeVR~\cite{li2018sysevr} offer vulnerability prediction models trained on a mixture of vulnerable examples from NVD~\cite{booth2013national} and SARD~\cite{SARD} datasets; Russell~\etal~\cite{russell2018automated} offers a vulnerability prediction model trained on GitHub+Debian data which are annotated with a static-analysis tool (see~\tab{existing_approach_design_choices}). We used these approaches since they train their models on datasets (NVD, SARD, and GitHub+Debian) containing source code examples and annotations obtained from the real world.

To understand the difference between baseline performance of VulDeePecker, SySeVR, and Russell~\etal and the reported performance in respective paper, we inspect what features are learned by the different approaches. To do this, we use Lemna~\cite{guo2018lemna} which is popular explainability framework for deep learning models. Lemna~\cite{guo2018lemna} attempts to explain black-box (\ie, non-explainable) deep learning models by estimating the local decision boundary around a data point using a white-box (\ie, explainable) linear model. 

Specifically, given an example data point $(x_i,\;y_i),\;i\in \{1,\ldots,N\}$ where $x_i$ is the input and $y_i$ is the corresponding label, Lemna draws samples around $x_i$ to obtain $L$ synthetic input sequences $z_{i,j},\;j\in \{1,\ldots,L\}$ and its prediction labels $w_{i,j},\;j\in \{1,\ldots,L\}$. Lemna then learns a linear regression model from the original data point along with the sampled data points. Each of the token $x_i^t$ is assigned a value $\omega_i^t$ representing the contribution of that token for prediction. Higher value of $\omega_i^t$ would indicate larger contribution of token $x_i^t$ in predicting $y_i$~\footnote{For a detailed discussion, see~\cite{guo2018lemna}}. 


We use a heatmap to visualize the contribution of different tokens in an input code snippet for predicting the existence of vulnerability. ~\Cref{fig:lemna_examples} shows three examples of vulnerable code snippets.~\Cref{fig:lemna_int_overflow}, and~\Cref{fig:lemna_memory_overflow} are from NVD and SARD datasets and used by VulDeePecker~\cite{li2018vuldeepecker}, and SySeVR~\cite{li2018sysevr} to train their models repectively. Thus both of those code snippets show code slices extracted from the program.~\Cref{fig:lemna_draper} shows a function from Github + Debian~\cite{russell2018automated}, which Russel~\etal~\cite{russell2018automated} used to train their model. Note that, while we show the actual code tokens for analysis purpose, for training we used approach specific tokenization.

Each token in~\fig{lemna_examples} is highlighted with a color corresponding to the token's contribution to the prediction. Most important tokens are highlighted in \lone{red} and the least important tokens are colored \lfive{green}. We make the following observations:

\smallskip
\noindent\textbf{NVD + SARD dataset.}~\Cref{fig:lemna_int_overflow} and \Cref{fig:lemna_memory_overflow} show two code slices extracted by SySeVR from NVD and SARD datasets. Although these examples are predicted correctly by SySeVR, the most important token sequences used for the prediction are not related to the tokens pertaining to the actual vulnerability. 


~\Cref{fig:lemna_int_overflow} demonstrates an integer overflow vulnerability (CWE-190) where multiplying two integers (or a floating point variable) might result in an overflow. The actual vulnerability in this case lies in line 7, however \lone{\tt \textbf{void}} \lone{\tt CWE190\_Integer\_Overflow\_Unsigned\_int...()} contributes the most to SySeVR's Deep Learning model followed by \ltwo{\tt \textbf{unsigned int} data} and \ltwo{data = 0;}. 


\Cref{fig:lemna_memory_overflow} shows a similar example for Uncontrolled Memory Vulnerability (CWE-789), where size of the memory allocated comes from a user input or the output of an API call. Without explicit sanitization, it can cause an uncontrolled memory allocation leading to a crash. Even though the main reason for the vulnerability in this example lies in lines 5, 9, and 10, however \lone{\tt \textbf{void} CWE789\_Uncontrolled\_Mem\_Alloc... ()} contributes the most in SySeVR's Prediction, followed by \ltwo{\tt \textbf{size\_t} data ;} and \ltwo{\tt data = 0;}.

\smallskip
\noindent\textbf{Github + Debian dataset.}~\Cref{fig:lemna_draper} shows an example from Github + Debian dataset. The plausible reason for this code to be vulnerable is the use of {\tt sprintf} function in line 6, 8, and 10. The length of {\tt buf} is not checked before writing to it through the {\tt sprintf} function. The CNN+RF model proposed by Russel~\etal~\cite{russell2018automated} picked up \lone{\small \tt \textbf{struct} port\_attribute} \lone{\tt *unused, \textbf{char} * buf)\{ \textbf{switch}} as the highest contributing token sequence. Similar to previous two examples, neither highest, nor the second highest contributing token sequences are related to the vulnerability.

We note that dataset used to train VulDeePecker and SySeVR\footnote{NVD + SARD dataset, mostly examples from SARD} were not originally intended to be used for vulnerability prediction task. These datasets were designed to elicit false negatives/false positives in static analyzers and also for human reference (in the form of CWEs). Therefore, they offer a simplified representation of the real vulnerability. Unlike these datasets, the GitHub + Debian dataset was collected by Russell~\etal~\cite{russell2018automated} from the real world projects on GitHub and some examples from the Debian distribution. However, the annotations for GitHub + Debian were made using a collection of static analyzers, therefore, it is difficult to know how noisy the dataset is \ie how many of these annotated vulnerabilities are False Positives. The simplicity and the noise in the datasets are forcing models to learn irrelevant features from the datasets. 


% \noindent\textbf{Approach.}~
To further understand \Cref{fig:lemna_examples}, we inspect the (semi-)synthetic datasets that were used by VulDeePecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr} and GitHub+Debian~\cite{russell2018automated}). To analyze the characteristics of those datasets, we investigate repetitiveness  of the data. Repetitiveness is introduced by the preprocessing technique used by the DLVP method; this informs us of how much of the training and testing samples are exactly the same after the code has been preprocessed. 

\begin{table}[!tb]
    \centering
    \footnotesize
    \caption{\small Percentage of duplicate samples in datasets. Draper data provide specific train, dev, and test split of the dataset. 94.93\% examples are unique to dev and test set from the corresponding train set. We found 97.02\% unique examples when we combine all the examples together.}
    \begin{tabular}{c|c|c}
        \hlineB{2}
        \textbf{Dataset} &\textbf{Technique} & \textbf{\% of duplicates}\bigstrut\\
        \hlineB{2}
         Juliet & Russell~\etal & 68.63 \bigstrut\\
         \hlineB{1}
         \multirow{2}{*}{NVD + SARD} & VulDeePecker &  67.33 \bigstrut\\
         & SySeVR &  61.991 \bigstrut\\
         \hlineB{1}
         Github+Debian & Russell~\etal & 6.07 / 2.99 \bigstrut\\
         \hlineB{2}
    \end{tabular}
    \label{tab:duplicate}
\end{table}


Table~\ref{tab:duplicate} shows the percentage of duplicate samples generated by different DLVP methods. For NVD and SARD datasets, the preprocessing technique from VulDeePecker results in $\mathbf{\sim75\%}$ duplicate examples (leaving only $\sim$25\% unique examples). $\mathbf{\sim50\%}$ of the examples are duplicated for NVD and SARD datasets when preprocessing technique from SySeVR is used. In Juliet and Github+Debian datasets, Russell~\etal.'s method produces $57\%$ and $2.98\%$ duplicate examples, respectively. 

Ideally, a DL based model should be trained and tested on a dataset where 100\% of the examples are unique.  Duplication tends to artificially increase the overall performance of the method~\cite{allamanis2019adverse} (as reported in Baseline row of~\tab{rq1_real_world_prediction}).



==> pycodes/alogorithms.tex <==
\renewcommand\thesubfigure{\alph{subfigure}}
\begin{figure*}[ht!]
\centering
\begin{minipage}{.45\linewidth}
\begin{subfigure}[t]{\linewidth}

\vspace{-1.8em}
\caption{The overall framework of \tool}
\label{fig:general_framework}    
\end{subfigure}
\end{minipage}
\begin{minipage}{.45\linewidth}
\begin{subfigure}[t]{\linewidth}

\vspace{-1.8em}
\caption{Method for extracting feature from a given code.}
\label{fig:extract_feature}    
\end{subfigure}%~
\end{minipage}
\begin{minipage}{.45\linewidth}
\begin{subfigure}{\linewidth}

\vspace{-2em}
\caption{Method to calculating \tool loss.}
\label{fig:calculate_loss}    
\end{subfigure}
\end{minipage}
\caption{{\small Pseudo-code of \tool.}}
\label{fig:pseudo}
\end{figure*}

==> pycodes/codes.tex <==
\renewcommand\thesubfigure{\alph{subfigure}}
\begin{figure*}[ht!]
\centering
\begin{minipage}{.45\linewidth}
\begin{subfigure}[t]{\linewidth}
\inputminted[bgcolor=white, numbersep=5pt, linenos=true, fontsize=\scriptsize]{python}{pycodes/framework.py}
\vspace{-1.8em}
\caption{The overall framework of \tool}
\label{fig:general_framework}    
\end{subfigure}
\end{minipage}
\begin{minipage}{.45\linewidth}
\begin{subfigure}[t]{\linewidth}
\inputminted[bgcolor=white, numbersep=5pt, linenos=true, fontsize=\scriptsize]{python}{pycodes/extract_feature.py}
\vspace{-1.8em}
\caption{Method for extracting feature from a given code.}
\label{fig:extract_feature}    
\end{subfigure}%~
\end{minipage}
\begin{minipage}{.45\linewidth}
\begin{subfigure}{\linewidth}
\inputminted[bgcolor=white, numbersep=5pt, linenos=true, fontsize=\scriptsize]{python}{pycodes/calculate_loss.py}
\vspace{-2em}
\caption{Method to calculating \tool loss.}
\label{fig:calculate_loss}    
\end{subfigure}
\end{minipage}
\caption{{\small Pseudo-code of \tool.}}
\label{fig:pseudo}
\end{figure*}

==> rq_summary.tex <==
\section{Research Questions}
\label{sec:rq_summary}

% A vulnerability detection tool based on source code helps developer write and check code for potential vulnerability at a very early stage so that it can be fixed before the code goes to deployment. Since static analysis causes a lot of false positives~\cite{}, using static analyzer for vulnerability detection is often less solicited method among developers~\cite{}. On top of that, hand writing violation patterns for static analyzers are often gruesome for the developers. A Machine Learning based vulnerability detection tool should be able to discover those violation patterns from sufficient volume of data and should avoid the huge number of false positives. 

% In this paper, we look into the different Deep Learning(DL) based techniques that are proposed in vulnerability detection literature and investigate in details about the applicability of those techniques, their pitfalls. We systematically investigate the reasons behind the pitfalls and propose some suggestions for overcoming such shortcomings.
% \saikat{The above two paragraph may go to introduction}


% Any ML based technique depends on the data that the technique is trained on. Success of a ML technique largely depends on both the power of the technique and quality of the data. 

% Although recent DL based  techniques~\cite{li2018vuldeepecker, li2018sysevr, russell2018automated} showed very high performance in detecting vulnerabilities, we are interested to investigate their proposed models' applicability in real world software development scenario. To simulate real world software development, we first investigate how each of these techniques generalize beyond the dataset each individual model is trained on. Hence, we ask the first research question,
% \RQ{1}{How well an existing DL based approach can be applicable in a plausible real world development scenario?}

\noindent\textbf{RQ1: How well do state-of-the-art vulnerability prediction models work in a real-world situations?}\\
\motivation
Most vulnerability prediction models are intended to be used predict vulnerabilities in real-world situations. However, there have so far been very limited results on real-world validation. Thus, in the first research question we ask how effective state-of-the-art vulnerability prediction models are under real-world circumstances.
% Since all the DL based vulnerability detection technique require annotated data, we are simulating this scenario particularly considering that a developer may not have sufficient annotation. Hence they would want to rely on a pre-trained model on other dataset. Scarcity of annotated vulnerable code legitimize this use case scenario. 

\approach To answer this question, we evaluate situations where a developer may have a scarcity of annotated data and thus chooses to use a pre-trained model. Here, we assess the performance of 4 state-of-the-art vulnerability prediction models namely, CNN, CNN+RF, BGRU, and BLSTM pre-trained on a 5 \vp datasets namely, Juliet~\cite{okun2013report}, VulDeepPecker~\cite{li2018vuldeepecker}, SySeVR~\cite{li2018sysevr}, Github + Debian~\cite{russell2018automated}. In addition, we also evaluate the 4 vulnerability prediction models on two additional real-world datasets, \ie, Devign dataset (consisting real world vulnerabilities from Qemu and FFMpeg)~\cite{zhou2019devign} and vulnerabilities from Chrome and Debian. 
We evaluate the performance of pre-trained models on each of the available datasets in a round-robin fashion. 
We find:

% and (b)~situations where training data comes from a real-world projects.
% To answer this question, we test each of the trained model on other test datasets. Here we use test examples from other dataset as a proxy of unknown dataset in the wild. One obvious question may rise with this approach that what is we learn from all existing dataset. To test the existing approaches' effectiveness, we design an ensemble model on all the existing dataset except the dataset in test. Details about the experimental setup are described in Section~\ref{sec:rq1-answer}. With detailed experiments, we find the answer, 

\begin{result}
The existing vulnerability prediction models do not work well when applied in a real-world setting. We notice a significant drop in both accuracy (by XX times in some cases) and F-1 score (by XX times in some cases).
\end{result}

% \rayb{Saikat says: I still want to put ensemble as a part of this RQ? Because, in my mind, ensemble goes before the next RQ, because in next RQ, we are proving that the datasets are very simple (all synthetic), hence there is no point of trying ensemble after that.}

\noindent\textbf{RQ2. Why do current vulnerability prediction models fail in real-world situations?}\\

\motivation~In this RQ, we investigate the reasons why existing vulnerability prediction models do not work well when applied in a real-world setting. 

\approach~We identify two possible reasons: (a) Inadequate data, and (b) Inadequate models. We break this research question into two sub-questions:  

\noindent\textit{\textbf{RQ2-A What are the challenges with the available data?}}
We analyze the vulnerability prediction dataset for any anomalous patterns that may affect its usability. We find that,
\begin{result}
Each of the 5 synthetic \vp datasets exhibit extensive repetition bias, \ie, there number of code clones are too high. For instance, \textit{Juliet}~\cite{okun2013report} and \textit{DRAPER}~\cite{russell2018automated} has less than 50\% were unique code samples. Further, models trained on synthetic \vp datasets were found to mostly used spurious (noisy) features to make predictions.% compared to real-world \vp datasets.   
\end{result}

\noindent\textit{\textbf{RQ2-B What are the challenges with the available models?}}
We inspect the frequently used machine learning framework for \vp in terms of code pre-processing method, code abstraction methods, and the underlying machine learning algorithm. We find that:
\begin{result}
We find that existing methods, \ie, CNN~\cite{russell2018automated}, BLSTM~\cite{li2018vuldeepecker}, BGRU~\cite{li2018sysevr}, fail to work in real-world setting because they (a)~Do not incorporate concrete token names, and (b)~Don not account for structural and semantic information. 
\end{result}


\noindent\textbf{RQ3. How to improve real world \vp?}

The previous two research questions demonstrate that current \vp approaches do not generalize to real-world applications because: (a)~; and (b)~.  we hypothesize that any Deep Learning based model to be applicable in real world development scenario, needs to be trained on real world data. We focus on the performance of existing models on real world dataset. We ask,

% To answer this question, first we observe different properties of the datasets. In particular we investigate the degree for code repetitions inside a dataset. We call this \emph{Repetition Bias}. This bias is causing the models to pick of irrelevant signals for vulnerability prediction. Then we compare such properties from real world dataset. The details of the experiments and case study are described in Section~\ref{sec:bias-and-case-study}. We summarize the findings as, 

% \begin{result}
% % The existing datasets are so simple that an SVM based classifies is sufficient for vulnerability prediction. These dataset do not exhibit the complex property of vulnerability in real dataset. 
% The existing datasets are very repetitive in nature. This repetition forces the models to pick up wrong signals.
% % Furthermore, token based models based on these datasets learn irrelevant features and patterns.
% \end{result}


%%%%%%%%%%%% This following paragraph might be used if we chose to include explainability of the features %%%%%%%%%%%%%%%%
% With our research finding showing that the datasets much simpler than real world scenario, we focus on what the models are actually learning. We investigate whatever the model is learning has anything to do with the vulnerability. We do a case study with extracting important feature that is learned by a model. This study shows us the contribution of different tokens for a prediction of vulnerability. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

%%%%%%%%%%%%%%%%%%%%% This paragraph describe the ensemble model %%%%%%%%%%%%%%%%%%%%%
% To answer this question, we use two different intuitive solutions. Firstly to test vulnerability from a particular dataset (Dataset-A), we deploy pre-trained model from other dataset and observe the performance. Secondly, we build an ensemble model~\cite{} trained on all the other datasets.  We use both \emph{Veto} and \emph{Majority Voting} ensemble method. In \emph{Veto} ensemble method, if one model says a piece of code is vulnerable, the we conclude that code is vulnerable. In case of \emph{Majority Voting}, we go with the decision of the majority models. 
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

% We observe that, the techniques we investigated in above research question are all token based model \ie they consider code as a sequence of tokens. Having that in mind, we are curious to know what is keeping a model to be applicable in real world scenario. To that end, we take a closer look at both the models and the datasets they are trained on. Here we ask our next research question, 


 
% \RQ{3}{How well does existing models perform in real world dataset?}
% To answer this question, we adopt 2 different approach. First one is proposed by Russel~\etal~\cite{russell2018automated}, where code for each function is considered as a standalone point for prediction. The second approach is proposed by Li~\etal~\cite{li2018vuldeepecker}, where instead of entire body of the functions, slices extracted from different interest points in the function (\eg API calls, array usage etc.) are considered for prediction. To have a fair comparison of these two approaches, if any of the slices extracted from a function is predicted as vulnerable by the latter approach, we consider the whole function as predicted vulnerable. Experimental details are described in Section~\ref{sec:existing-method-on-real-data}.
% After rigorous experiment, we reach to the following research findings
% \RS{3}{Token based DL techniques are \textbf{not} very effective in predicting vulnerability in real world scenario. Even static analyzer (through slice extraction) \textbf{does not} help as much to boost the performance of token based models.}

% We observe that, the techniques we investigated in above research question are all token based model \ie they consider code as a sequence of tokens. We hypothesize that to let any model understand the semantic relationships between code elements, any vulnerability detection tool should consider the control and data dependency in the code. We ask the following research question,

% \RQ{4}{Does semantic information in code help improve the performance of Vulnerability Detection model?}

% We build a Gated Graph Neural Network~\cite{} based vulnerability detection tool. Similar method is proposed by Zhou~\etal~\cite{zhou2019devign}. We tested this model on the (partial)dataset (Devign dataset) that Zhou~\etal released and also on our collected dataset. We summarize our finding as 
% \RS{4}{Graph based models are better suitable for capturing semantic information, hence perform better that token based counterpart.}

% In the previous research question, We observe that the the performance of graph based model Zhou~\etal~\cite{zhou2019devign} is relatively better than that of our dataset. We observe that the ratio between vulnerable code and non-vulnerable code in their dataset and in our dataset are different. Their dataset is highly balance (with 55\% non-vulnerable examples and 45\% vulnerable examples). 

% Then we ask, 
% \RQ{5}{Does imbalance in dataset has any influence on the performance?}

% To test our hypothesis, we created artificial imbalance on Devign data. Since in real world, developers are free to do whatever they want with the training data, in this experiment, we keep the train data in Devign as it is. We created artificial imbalance in the test data only to see this performance has any adverse effect on the performance. The result we found, 

% \RS{5}{High imbalance of non-vulnerable and vulnerable examples adversely effect the performance of vulnerability detection tool.}

% We observe that the dataset we collected has 90\% of non-vulnerable and 10\% vulnerable examples. An ML model trained directly on such imbalance data will be biased towards the class with majority examples~\cite{}. With that problem in mind, we ask
% \RQ{6}{How do we fix a training process so that bias towards majority class is avoided?}

% To answer this question, we balance the training data. We use random undersampling and oversampling techniques to balance the training data. We do not modify the imbalance ratio in test data. We experiment on various degree of undersampling and oversampling and a various degree of combination of these two techniques. We summarize the result,
% \RS{6}{Balancing out the training data does improve performance in imbalanced test set. We also observe that with higher oversampling precious increases and with higher undersampling recall increases. A combination of both results in the optimal performance in the test data.}

% In summary, our findings in this paper can be summarized as. 
% \begin{enumerate}
%     \item Models trained on synthetic data is not suitable for finding vulnerability in the wild.
%     \item Token based models fail to capture semantic information in the code that is necessary to detect vulnerability. 
%     \item Vulnerabilities are naturally scarce. Any dataset evaluation of vulnerability should reflect the (close to) natural distribution of vulnerability. 
%     \item Balancing in data should only be performed in the training data to help model learn better. Different balancing technique is suitable for different performance goal. 
%     \item Even sophisticated graph based models do not achieve high performance in vulnerability detection. Hence, ML-based vulnerability detection is still is very much an open problem.
% \end{enumerate}











==> tex/dlvp_overview.tex <==
% \begin{figure}[!t]
% \centering
% \includegraphics[width=\linewidth]{imgs/dlvp_pseudo_small.pdf}
% \bray{I do not think the definitions are necessary}
% \caption{\small Overview of DL-based \vp approach, also write it in listing so that we can play with it.
% \bray{fonts need to be increased. What does 1, 2, 3, 4 mean---confusing!!}
% }
% \label{fig:overview}
% \end{figure}

% \begin{algorithm}[!t]
%     \footnotesize
%     \SetAlgoLined
%     \SetKwInOut{Input}{Input}
%     \SetKwInOut{Output}{Output}
%     \SetKwFunction{DLVP}{}
%     \SetKwProg{Fn}{Function}{:}{}
%     \Input{Code Corpus ($\mathrm{C}$).}
%     \Output{$\mathcal{P}$: Prediction Performance.}
%         training\_corpus $\leftarrow$ collect\_training\_data$(\mathrm{C})$
%         testing\_corpus $\leftarrow$ collect\_testing\_data$(\mathrm{C})$
%     \caption{\textbf{\small Graph Embedding}}
%     \label{alg:feature_extraction}
% \end{algorithm}

% \begin{algorithm}[!htpb]
% \SetAlgoLined
%  ${D}_{train} \leftarrow Collect\_Data\_For\_Training()$\;
%  ${M} \leftarrow Choose\_Model()$\;
%  ${D}'_{train} \leftarrow Preprocess\_Data({D})$\;
%  $Train({M}, {D}'_{train})$\;
%  ${D}_{test} \leftarrow Evaluation\_Data()$\;
%  ${D}'_{test} \leftarrow preprocessed\_evaluation\_data({D}_{test})$\;
%  $Evaluate({M}, {D}'_{test})$\;
%  \caption{\small Overview of DL-based \vp approach}
%  \label{alg:overview}
% \end{algorithm}

==> tex/t-sne.tex <==
\begin{figure}[h!]
    \centering
    \begin{subfigure}{0.45\linewidth}
        \centering
    \includegraphics[width=0.98\linewidth]{imgs/before-training.pdf}
    \caption{}
    \label{a}
    \end{subfigure}~\begin{subfigure}{0.45\linewidth}
        \centering
        \includegraphics[width=\linewidth]{imgs/triplet.pdf}
    \caption{}
    \end{subfigure}
    \label{b}
    \caption{t-SNE~\cite{maaten2008visualizing} plots of features with and without representation learning (during training).}
    \label{fig:t-sne-train-plots}
    % \bray{we do not need this figure here, move all t-SNE plots in the same place}
\end{figure}

==> todo.tex <==
% All the todos will go here. 
% This file is included after the conclusion section from main.tex, will be commented out for submission. 

\section*{TODO}

